A Unified Linear Speedup Analysis of Federated Averaging and Nesterov FedAvg

Federated learning (FL) learns a model jointly from a set of participating devices without sharing each other's privately held data. The characteristics of non-i.i.d. data across the network, low device participation, high communication costs, and the mandate that data remain private bring challenges in understanding the convergence of FL algorithms, particularly regarding how convergence scales with the number of participating devices. In this paper, we focus on Federated Averaging (FedAvg), one of the most popular and effective FL algorithms in use today, as well as its Nesterov accelerated variant, and conduct a systematic study of how their convergence scale with the number of participating devices under non-i.i.d. data and partial participation in convex settings. We provide a unified analysis that establishes convergence guarantees for FedAvg under strongly convex, convex, and overparameterized strongly convex problems. We show that FedAvg enjoys linear speedup in each case, although with different convergence rates and communication efficiencies. For strongly convex and convex problems, we also characterize the corresponding convergence rates for the Nesterov accelerated FedAvg algorithm, which are the first linear speedup guarantees for momentum variants of FedAvg in convex settings. Empirical studies of the algorithms in various settings have supported our theoretical results.

==> app_overparameterized_theorem7.tex <==
% !TEX ROOT=./supp-main.tex

\subsection{Geometric Convergence of FedMaSS for Overparameterized Linear Regression}

\begin{thm}
For the overparamterized linear regression problem, FedMaSS with communication every $E$ iterations and constant
step sizes $\overline{\eta}_1=\mathcal{O}(\frac{1}{E}\frac{N}{l\nu_{\max}+\mu(N-\nu_{\min})}),\overline{\eta}_{2}=\frac{\overline{\eta}_{1}(1-\frac{1}{\tilde{\kappa}})}{1+\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}},\overline{\gamma}=\frac{1-\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}}{1+\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}}$
has geometric convergence:
\begin{align*}
\mathbb{E}F(\overline{\mathbf{w}}_{T}) & \leq\mathcal{O}\left(L\exp(-\frac{NT}{E(\nu_{\max}\sqrt{\kappa_{1}\tilde{\kappa}}+(N-\nu_{\min}))})\|\mathbf{w}_{0}-\mathbf{w}^{\ast}\|^{2}\right).
\end{align*}
\end{thm}
\begin{proof}
	
	The proof is based on results in~\cite{liu2018accelerating} which originally proposed the MaSS algorithm. Note that the update can equivalently be written as 
	\begin{align*}
	\mathbf{v}_{t+1}^{k} & =(1-\alpha^{k})\mathbf{v}_{t}^{k}+\alpha^{k}\mathbf{u}_{t}^{k}-\delta^{k}\vg_{t,k}\\
	\mathbf{w}_{t+1}^{k} & =\begin{cases}
	\mathbf{u}_{t}^{k}-\eta^{k}\vg_{t,k} & \text{if }t+1\notin\mathcal{I}_{E}\\
	\sum_{k=1}^{N}p_{k}\left[\mathbf{u}_{t}^{k}-\eta^{k}\vg_{t,k}\right] & \text{if }t+1\in\mathcal{I}_{E}
	\end{cases}\\
	\mathbf{u}_{t+1}^{k} & =\frac{\alpha^{k}}{1+\alpha^{k}}\mathbf{v}_{t+1}^{k}+\frac{1}{1+\alpha^{k}}\mathbf{w}_{t+1}^{k}
	\end{align*}
	where there is a bijection between the parameters $\frac{1-\alpha^{k}}{1+\alpha^{k}}=\gamma^{k},\eta^{k}=\eta_{1}^{k},\frac{\eta^{k}-\alpha^{k}\delta^{k}}{1+\alpha^{k}}=\eta_{2}^{k}$,
	and we further introduce an auxiliary parameter $\mathbf{v}_{t}^{k}$,
	which is initialized at $\mathbf{v}_{0}^{k}$. We also note that when
	$\delta^{k}=\frac{\eta^{k}}{\alpha^{k}}$, the update reduces to the
	Nesterov accelerated SGD. This version of the FedAvg algorithm with
	local MaSS updates is used for analyzing the geometric convergence. 
	
	As before, define the virtual sequences $\overline{\mathbf{w}}_{t}=\sum_{k=1}^{N}p_{k}\mathbf{w}_{t}^{k}$,
	$\overline{\mathbf{v}}_{t}=\sum_{k=1}^{N}p_{k}\mathbf{v}_{t}^{k}$,
	$\overline{\mathbf{u}}_{t}=\sum_{k=1}^{N}p_{k}\mathbf{u}_{t}^{k}$,
	and $\ov{g}_{t}=\sum_{k=1}^{N}p_{k}\mathbb{E}\vg_{t,k}$. We have
	$\mathbb{E}\vg_{t}=\ov{g}_{t}$ and $\overline{\mathbf{w}}_{t+1}=\overline{\mathbf{u}}_{t}-\eta_{t}\vg_{t}$,
	$\overline{\mathbf{v}}_{t+1}=(1-\alpha^{k})\overline{\mathbf{v}}_{t}+\alpha^{k}\overline{\mathbf{w}}_{t}-\delta^{k}\vg_{t}$,
	and $\overline{\mathbf{u}}_{t+1}=\frac{\alpha^{k}}{1+\alpha^{k}}\overline{\mathbf{v}}_{t+1}+\frac{1}{1+\alpha^{k}}\overline{\mathbf{w}}_{t+1}$.
	
	We first prove the theorem with $E=2$ and $t-1$ being a communication
	round. We have 
	\begin{align*}
	& \|\overline{\mathbf{v}}_{t+1}-\mathbf{w}^{\ast}\|_{\vH^{-1}}^{2}\\
	& =\|(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\delta\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\vu_{t}^{k}-\vw^{\ast})-\vw^{\ast}\|_{\vH^{-1}}^{2}\\
	& =\|(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\vu_{t}^{k}-\vw^{\ast})\|_{\vH^{-1}}^{2}\\
	& -2\delta\langle\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\vu_{t}^{k}-\vw^{\ast}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}\\
	& \leq\underset{A}{\underbrace{\|(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}}}+\underset{B}{\underbrace{2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vw^{\ast})\|_{\vH^{-1}}^{2}}}+2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}\\
	& \underset{C}{\underbrace{-2\delta\langle\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vw^{\ast}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}}}\\
	& -2\delta\langle\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\vu_{t}^{k}-\ov{u}_{t}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}
	\end{align*}
	Following the proof in~\cite{liu2018accelerating}, 
	\begin{align*}
	\mathbb{E}A & \leq\mathbb{E}(1-\alpha)\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\alpha\|\ov{u}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}\\
	& \leq\mathbb{E}(1-\alpha)\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\frac{\alpha}{\mu}\|\ov{u}_{t}-\vw^{\ast}\|^{2}
	\end{align*}
	using the convexity of the norm $\|\cdot\|_{\vH^{-1}}$ and that $\mu$
	is the smallest non-zero eigenvalue of $H$. 
	
	Now 
	\begin{align*}
	\mathbb{E}B & \leq2\delta^{2}(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})\|(\ov{u}_{t}-\vw^{\ast})\|_{H}^{2}
	\end{align*}
	using the folowing bound: 
	\begin{align*}
	\mathbb{E}\left(\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\right)\vH^{-1}\left(\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\right) & =\mathbb{E}\sum_{k}p_{k}^{2}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\sum_{k\neq j}p_{k}p_{j}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{j}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\sum_{k\neq j}p_{k}p_{j}\vH^{k}\vH^{-1}\vH^{j}\\
	& =\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\sum_{k,j}p_{k}p_{j}\vH^{k}\vH^{-1}\vH^{j}-\sum_{k}p_{k}^{2}\vH^{k}\vH^{-1}\vH^{k}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\vH-\frac{1}{N}\nu_{\min}\sum_{k}p_{k}\vH^{k}\vH^{-1}\vH^{k}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\vH-\frac{1}{N}\nu_{\min}(\sum_{k}p_{k}\vH^{k})\vH^{-1}(\sum_{k}p_{k}\vH^{k})\\
	& =\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}+\frac{N-\nu_{\min}}{N}\vH\\
	& \preceq\nu_{\max}\frac{1}{N}\tilde{\kappa}\vH+\frac{N-\nu_{\min}}{N}\vH
	\end{align*}
	where we have used $\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\vH^{-1}\tilde{\vH}_{t}^{k}\leq\tilde{\kappa}\vH$
	by definition of $\tilde{\kappa}$ and the operator convexity of the
	mapping $W\rightarrow W\vH^{-1}W$.
	
	Finally, 
	\begin{align*}
	\mathbb{E}C & =-\mathbb{E}2\delta\langle\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vw^{\ast}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}\\
	& =-2\delta\langle\sum_{k}p_{k}\vH^{k}(\ov{u}_{t}-\vw^{\ast}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}\\
	& =-2\delta\langle(\ov{u}_{t}-\vw^{\ast}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle\\
	& =-2\delta\langle(\ov{u}_{t}-\vw^{\ast}),\ov{u}_{t}-\vw^{\ast}+\frac{1-\alpha}{\alpha}(\ov{u}_{t}-\ov{w}_{t})\rangle\\
	& =-2\delta\|\ov{u}_{t}-\vw^{\ast}\|^{2}+\frac{1-\alpha}{\alpha}\delta(\|\ov{w}_{t}-\vw^{\ast}\|^{2}-\|\ov{u}_{t}-\vw^{\ast}\|^{2}-\|\ov{w}_{t}-\ov{u}_{t}\|^{2})\\
	& \leq\frac{1-\alpha}{\alpha}\delta\|\ov{w}_{t}-\vw^{\ast}\|^{2}-\frac{1-\alpha}{\alpha}\delta\|\ov{u}_{t}-\vw^{\ast}\|^{2}
	\end{align*}
	where we have used 
	\begin{align*}
	& (1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}\\
	& =(1-\alpha)((1+\alpha)\ov{u}_{t}-\ov{w}_{t})/\alpha+\alpha\ov{u}_{t}\\
	& =\frac{1}{\alpha}\ov{u}_{t}-\frac{1-\alpha}{\alpha}\ov{w}_{t}
	\end{align*}
	and the identity that $-2\langle \va,\vb\rangle=\|\va\|^{2}+\|\vb\|^{2}-\|\va+\vb\|^{2}$. 
	
	It follows that 
	\begin{align*}
	& \mathbb{E}\|\ov{v}_{t+1}-\vw^{\ast}\|_{\vH^{-1}}^{2}\\
	& \leq(1-\alpha)\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\frac{1-\alpha}{\alpha}\delta\|\ov{w}_{t}-\vw^{\ast}\|^{2}\\
	& +(\frac{\alpha}{\mu}-\frac{1-\alpha}{\alpha}\delta)\|\ov{u}_{t}-\vw^{\ast}\|^{2}+2\delta^{2}(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})\|(\ov{u}_{t}-\vw^{\ast})\|_{H}^{2}\\
	& +2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}\\
	& -2\delta\langle\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\vu_{t}^{k}-\ov{u}_{t}),(1-\alpha)\ov{v}_{t}+\alpha\ov{u}_{t}-\vw^{\ast}\rangle_{\vH^{-1}}
	\end{align*}
	
	On the other hand, 
	\begin{align*}
	\mathbb{E}\|\ov{w}_{t+1}-\vw^{\ast}\|^{2} & =\mathbb{E}\|\ov{u}_{t}-\vw^{\ast}-\eta\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vw^{\ast})\|^{2}\\
	& =\mathbb{E}\|\ov{u}_{t}-\vw^{\ast}\|^{2}-2\eta\|\ov{u}_{t}-\vw^{\ast}\|_{H}^{2}+\eta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vw^{\ast})\|^{2}\\
	& \leq\mathbb{E}\|\ov{u}_{t}-\vw^{\ast}\|^{2}-2\eta\|\ov{u}_{t}-\vw^{\ast}\|_{H}^{2}+\eta^{2}(\nu_{\max}\frac{1}{N}\ell+L\frac{N-\nu_{\min}}{N})\|\ov{u}_{t}-\vw^{\ast}\|^{2}
	\end{align*}
	where we use the following bound: 
	\begin{align*}
	& \mathbb{E}\left(\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\right)\left(\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\right)\\
	& =\mathbb{E}\sum_{k}p_{k}^{2}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\sum_{k\neq j}p_{k}p_{j}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{j}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\sum_{k\neq j}p_{k}p_{j}\vH^{k}\vH^{j}\\
	& =\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\sum_{k,j}p_{k}p_{j}\vH^{k}\vH^{j}-\sum_{k}p_{k}^{2}\vH^{k}\vH^{k}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\vH^{2}-\frac{1}{N}\nu_{\min}\sum_{k}p_{k}\vH^{k}\vH^{k}\\
	& \preceq\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\vH^{2}-\frac{1}{N}\nu_{\min}(\sum_{k}p_{k}\vH^{k})(\sum_{k}p_{k}\vH^{k})\\
	& =\nu_{\max}\frac{1}{N}\mathbb{E}\sum_{k}p_{k}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}+\frac{N-\nu_{\min}}{N}\vH^{2}\\
	& \preceq\nu_{\max}\frac{1}{N}l\vH+L\frac{N-\nu_{\min}}{N}\vH
	\end{align*}
	again using that $W\rightarrow W^{2}$ is operator convex and that
	$\mathbb{E}\tilde{\vH}_{t}^{k}\tilde{\vH}_{t}^{k}\preceq l\vH^{k}$ by definition
	of $l$. 
	
	Combining the bounds for $\mathbb{E}\|\ov{w}_{t+1}-\vw^{\ast}\|^{2}$
	and $\mathbb{E}\|\ov{v}_{t+1}-\vw^{\ast}\|_{\vH^{-1}}^{2}$, 
	\begin{align*}
	& \mathbb{E}\frac{\delta}{\alpha}\|\ov{w}_{t+1}-\vw^{\ast}\|^{2}+\|\ov{v}_{t+1}-\vw^{\ast}\|_{\vH^{-1}}^{2}\\
	& \leq(1-\alpha)\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\frac{1-\alpha}{\alpha}\delta\|\ov{w}_{t}-\vw^{\ast}\|^{2}+(\frac{\alpha}{\mu}-\delta)\|\ov{u}_{t}-\vw^{\ast}\|^{2}\\
	& +(2\delta^{2}(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})-2\eta\delta/\alpha+\eta^{2}\delta(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})/\alpha)\|\ov{u}_{t}-\vw^{\ast}\|^{2}\\
	& +2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}\\
	& +\delta L\sum_{k}p_{k}\|(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}
	\end{align*}
	
	Following~\cite{liu2018accelerating} if we choose step sizes so that 
	\begin{align*}
	\frac{\alpha}{\mu}-\delta & \leq0\\
	2\delta^{2}(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})-2\eta\delta/\alpha+\eta^{2}\delta(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})/\alpha & \leq0
	\end{align*}
	or equivalently 
	\begin{align*}
	\alpha/\delta & \leq\mu\\
	2\alpha\delta(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})+\eta(\eta(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})-2) & \leq0
	\end{align*}
	the second and third terms are negative. To optimize the step sizes,
	note that the two inequalities imply 
	\begin{align*}
	\alpha^{2} & \leq\eta(2-\eta(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N}))\mu/2(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})
	\end{align*}
	and maximizing the right hand side with respect to $\eta$, which
	is quadratic, we see that $\eta\equiv1/(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})$
	maximizes the right hand side, with 
	\begin{align*}
	\alpha & \equiv\frac{1}{\sqrt{2(\nu_{\max}\frac{1}{N}\kappa_{1}+\kappa\frac{N-\nu_{\min}}{N})(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})}}\\
	\delta & \equiv\frac{\alpha}{\mu}=\frac{\eta}{\alpha(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})}
	\end{align*}
	
	Note that $\alpha=\frac{1}{\sqrt{2(\nu_{\max}\frac{1}{N}\kappa_{1}+\kappa\frac{N-\nu_{\min}}{N})(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})}}=O(\frac{N}{\sqrt{\kappa_{1}\tilde{\kappa}}})$
	when $N=O(\min\{\tilde{\kappa},\kappa_{1}/\kappa\})$. Finally, to
	deal with the terms $2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}+\delta L\sum_{k}p_{k}\|(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}$,
	we can use Jensen
	\begin{align*}
	&2\delta^{2}\|\sum_{k}p_{k}\tilde{\vH}_{t}^{k}(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2}+\delta L\sum_{k}p_{k}\|(\ov{u}_{t}-\vu_{t}^{k})\|_{\vH^{-1}}^{2} \\
	& \leq(2\delta^{2}l^{2}+\delta L)\sum_{k}p_{k}\|\ov{u}_{t}-\vu_{t}^{k}\|_{\vH^{-1}}^{2}\\
	& =(2\delta^{2}l^{2}+\delta L)\sum_{k}p_{k}\|\frac{\alpha}{1+\alpha}\ov{v}_{t}+\frac{1}{1+\alpha}\ov{w}_{t}-(\frac{\alpha}{1+\alpha}v_{t}^{k}+\frac{1}{1+\alpha}w_{t}^{k})\|_{\vH^{-1}}^{2}\\
	& \leq(2\delta^{2}l^{2}+\delta L)(2(\frac{\alpha}{1+\alpha})^{2}\delta^{2}+2(\frac{1}{1+\alpha})^{2}\eta^{2})\sum_{k}p_{k}\|\tilde{\vH}_{t-1}^{k}(\ov{u}_{t-1}-\vw^{\ast})\|^{2}\\
	& \leq(2\delta^{2}l^{2}+\delta L)(2(\frac{\alpha}{1+\alpha})^{2}\delta^{2}+2(\frac{1}{1+\alpha})^{2}\eta^{2})l^{2}\|(\ov{u}_{t-1}-\vw^{\ast})\|^{2}
	\end{align*}
	which can be combined with the terms with $\|(\ov{u}_{t-1}-\vw^{\ast})\|^{2}$
	in the recursive expansion of $\mathbb{E}\frac{\delta}{\alpha}\|\ov{w}_{t}-\vw^{\ast}\|^{2}+\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}$:
	\begin{align*}
	& \mathbb{E}\frac{\delta}{\alpha}\|\ov{w}_{t}-\vw^{\ast}\|^{2}+\|\ov{v}_{t}-\vw^{\ast}\|_{\vH^{-1}}^{2}\\
	& \leq(1-\alpha)\|\ov{v}_{t-1}-\vw^{\ast}\|_{\vH^{-1}}^{2}+\frac{1-\alpha}{\alpha}\delta\|\ov{w}_{t-1}-\vw^{\ast}\|^{2}+(\frac{\alpha}{\mu}-\delta)\|\ov{u}_{t-1}-\vw^{\ast}\|^{2}\\
	& +(2\delta^{2}(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})-2\eta\delta/\alpha+\eta^{2}\delta(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})/\alpha)\|\ov{u}_{t-1}-\vw^{\ast}\|^{2}
	\end{align*}
	and the step sizes can be chosen so that the resulting coefficients
	are negative. Therefore, we have shown that 
	\begin{align*}
	\mathbb{E}\|\ov{w}_{t+1}-\vw^{\ast}\|^{2} & \leq(1-\alpha)^{2}\|\ov{w}_{t-1}-\vw^{\ast}\|^{2}
	\end{align*}
	where $\alpha=\frac{1}{\sqrt{2(\nu_{\max}\frac{1}{N}\kappa_{1}+\kappa\frac{N-\nu_{\min}}{N})(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})}}=O(\frac{N}{\nu_{\max}\sqrt{\kappa_{1}\tilde{\kappa}}+N-\nu_{\min}})$
	when $N=O(\min\{\tilde{\kappa},\kappa_{1}/\kappa\})$.
	
	For general $E>1$, choosing $\eta=c/E(\nu_{\max}\frac{1}{N}l+L\frac{N-\nu_{\min}}{N})$
	for some small constant $c$ results in $\alpha=O(\frac{1}{E\sqrt{(\nu_{\max}\frac{1}{N}\kappa_{1}+\kappa\frac{N-\nu_{\min}}{N})(\nu_{\max}\frac{1}{N}\tilde{\kappa}+\frac{N-\nu_{\min}}{N})}})$
	and this guarantees that 
	\begin{align*}
	\mathbb{E}\|\ov{w}_{t}-\vw^{\ast}\|^{2} & \leq(1-\alpha)^{t}\|\vw_{0}-\vw^{\ast}\|^{2}
	\end{align*}
	for all $t$. 
	
	
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

\def\cO{{\mathcal{O}}}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec_acceleratedFL.tex <==
% !TEX ROOT=./main.tex


\section{Accelerated Federated Learning}

\subsection{Literature review}

\cite{felbab2019optimization} applies various accleration method
into federated learning and empirically compare the performance, 
while they did not provide any theoretical analysis of convergence.
\cite{liu2019accelerating} discuss momentum gradient descent
in the context of federated learning. They provide
convergence rate $\cO(\frac{1}{T})$ 
for strongly convex, $L$-smooth under gradient
descent algorithm. 
\cite{huo2020faster} provide convergence rate of momentum accelerated 
stochastic gradient descent for non-convex functions. 


\subsection{Framework summarization}

\begin{assumption}
The expected squared norm of stochastic subgradients is uniformly bounded. i.e.,
$\mathbb{E}\|\vg_{t,k}\|^2  \leq G_k^{2}$, for all $k = 1,..., N$ and $t=0, \dots, T-1$.  This also implies $\left\| \mathbb{E}\vg_{t,k}\right\|^2  \leq \mathbb{E}\|\vg_{t,k}\|^2 \leq G_k^2$.
\label{ass:subgrad2}
\end{assumption}

\begin{assumption}[Lipschitz continuous]
	The local function $F_k$ is lipschitz continuous. 
	\label{ass:lipcont}
\end{assumption}

\begin{assumption}[L-smooth]
$F_{1}, \cdots, F_{N}$ are all $L$-smooth: for all  $\mathbf{v}$  and $\mathbf{w}$, $F_{k}(\mathbf{v}) \leq F_{k}(\mathbf{w})+(\mathbf{v}- \\ \mathbf{w})^{T} \nabla F_{k}(\mathbf{w})+\frac{L}{2}\|\mathbf{v}-\mathbf{w}\|_{2}^{2}$.
\label{ass:lsmooth}
\end{assumption}

\begin{assumption}[Polyak-Lojasiewicz (PL)] The global objective functions $f($ ) is differentiable and satisfy the Polyak-Lojasiewicz condition with constant $\mu,$ i.e., $\frac{1}{2}\|\nabla f(\boldsymbol{w})\|_{2}^{2} \geq \mu\left(f(\boldsymbol{w})-f\left(\boldsymbol{w}^{*}\right)\right)$ holds $\forall \boldsymbol{w} \in \mathbb{R}^{d}$ with
$\boldsymbol{w}^{*}$ being the optimal solution of global objective.
\label{ass:pl}
\end{assumption}

\begin{assumption}[Strongly-convex]
$	F_{1}, \cdots, F_{N} \text { are all } \mu \text { -strongly convex: for all v and } \mathbf{w}, F_{k}(\mathbf{v}) \geq F_{k}(\mathbf{w})+(\mathbf{v}-\mathbf{w})^{T} \nabla F_{k}(\mathbf{w})+\frac{\mu}{2}\|\mathbf{v}-\mathbf{w}\|_{2}^{2}$
\label{ass:stroncvx}
\end{assumption}

\begin{assumption}[Bounded Variance]
Let $\xi_{t}^{k}$ be sampled from the k-th device's local data uniformly at random. The variance of stochastic gradients in each device is bounded:
$\mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)-\nabla F_{k}\left(\mathbf{w}_{t}^{k}\right)\right\|^{2} \leq \sigma_{k}^{2}$, for $k = 1,..., N$.
\label{ass:lgradvar}
\end{assumption}

\begin{assumption}[Expected square norm of gradient]
The expected squared norm of stochastic gradients is uniformly bounded. i.e.,
$\mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)\right\|^{2} \leq G^{2}$, for all $k = 1,..., N$ and $t=0, \dots, T-1$.
\label{ass:squaregrad}
\end{assumption}

\begin{assumption}[loss function f]
	Loss function $F$ has lower bound $F_{\inf}$. This assumption is assumed for all the works.  The existence of $F^*$. We didn't add this 
	in the table.
	\label{ass:flb}
\end{assumption}

\begin{assumption}[Bounded Weighted Gradient Diversity]
	The weighted gradient diversity among local objectives is defined as:
$$
\Lambda(\boldsymbol{w}, \boldsymbol{q}) \triangleq \frac{\sum_{k=1}^{N} p_{k}\left\|\nabla f_{k}(\boldsymbol{w})\right\|_{2}^{2}}{\left\|\sum_{k=1}^{N} p_{k} \nabla f_{k}(\boldsymbol{w})\right\|_{2}^{2}} \leq \lambda
$$
\label{ass:bgd}
\end{assumption}

\begin{table}[h!]
\centering
\small
	\begin{tabular}{|c|c|c|c|c|}\hline
		paper         & Noncvx & Cvx & Strongly Cvx\\ \hline
	Accelerated	SGD   & \cite{huo2020faster} A\ref{ass:lsmooth},\ref{ass:lgradvar} &          &             \\\hline
	Accelerated GD    &        &       &     \cite{liu2019accelerating}A\ref{ass:lipcont},\ref{ass:lsmooth}        \\\hline
	SGD    &   \cite{haddadpour2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},(\ref{ass:pl},\ref{ass:bgd}) ; \cite{huo2020faster}A\ref{ass:lsmooth},\ref{ass:lgradvar}  & A\ref{ass:subgrad2}  &   \cite{haddadpour2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},(\ref{ass:bgd}); \cite{li2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},\ref{ass:squaregrad}     \\\hline
	GD     &   \cite{haddadpour2019convergence}A\ref{ass:lsmooth},(\ref{ass:pl},\ref{ass:bgd})    & \cite{khaled2019first} A\ref{ass:lsmooth} &        \cite{haddadpour2019convergence}A\ref{ass:lsmooth},(\ref{ass:pl},\ref{ass:bgd})    \\\hline
	\end{tabular}
	\caption{Summarize of assumptions on federated learning, heterogeneous data. $(\cdot)$ means that the assumption is not necessary.}
	\label{tb:ass2}
\end{table}

\begin{table}[h!]
\centering
\small
	\begin{tabular}{|c|c|c|c|c|}\hline
		paper         & Noncvx & Cvx and Non-smth & Cvx and L-smth & Strongly Cvx and L-smth\\ \hline
	Accelerated	SGD   & \cite{huo2020faster} A\ref{ass:lsmooth},\ref{ass:lgradvar} &    &      &             \\\hline
	Accelerated GD    &        &    &   &     \cite{liu2019accelerating}A\ref{ass:lipcont},\ref{ass:lsmooth}        \\\hline
	SGD    &   \cite{haddadpour2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},(\ref{ass:pl},\ref{ass:bgd}) ; \cite{huo2020faster}A\ref{ass:lsmooth},\ref{ass:lgradvar}  & A\ref{ass:subgrad2}  &  &   \cite{haddadpour2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},(\ref{ass:bgd}); \cite{li2019convergence} A\ref{ass:lsmooth},\ref{ass:lgradvar},\ref{ass:squaregrad}     \\\hline
	GD     &   \cite{haddadpour2019convergence}A\ref{ass:lsmooth},(\ref{ass:pl},\ref{ass:bgd})     &  & \cite{khaled2019first} A\ref{ass:lsmooth} &        \cite{haddadpour2019convergence}A\ref{ass:lsmooth},(\ref{ass:pl},\ref{ass:bgd})    \\\hline
	\end{tabular}
	\caption{Summarize of assumptions on federated learning, heterogeneous data. $(\cdot)$ means that the assumption is not necessary.}
	\label{tb:ass}
\end{table}
\vspace{-1em}
\begin{table}[h!]
\centering
\small
	\begin{tabular}{|c|c|c|c|c|}\hline
		paper         & Noncvx & Cvx and Non-smth & Cvx and L-smth & Strongly Cvx and L-smth\\ \hline
	Accelerated	SGD   & \cite{huo2020faster} &        &    &             \\\hline
	Accelerated GD    &        &    &    &    \cite{liu2019accelerating}        \\\hline
	SGD    &   \cite{haddadpour2019convergence,huo2020faster}    & Ours &     &    \cite{li2019convergence}       \\\hline
	GD     &   \cite{haddadpour2019convergence}     &  & \cite{khaled2019first}     &         \\\hline
	\end{tabular}
	\caption{Summarize of relatedwork on federated learning, heterogeneous data.}
\end{table}


Note for table~\ref{tb:ass}:
\begin{itemize}
	\item \textbf{GD}: \cite{haddadpour2019convergence} the proof of Noncvx can be used directly for Strongly cvx and L-smooth.
	\item \textbf{SGD}: necessary assumption: Bounded gradient variance assumption. 
	\item \textbf{Non Cvx}: necessary assumption:  L-smooth.
	\item \textbf{Convex}:
\end{itemize}


\textbf{GD}
The proof of convergence rate of local GD in~\cite{haddadpour2019convergence} 
is based A~\ref{ass:lsmooth} and A~\ref{ass:pl}, note that PL is a generalization of $\mu$-strongly convexity. $\mu$-strongly convexity
indicates A~\ref{ass:pl} is satisfied. Therefore, the same proof in~\cite{haddadpour2019convergence} for non-convex function 
can be adapted for strongly convex and $L$-smooth function. 




\begin{itemize}
	\item Online Meta learning~\cite{finn2019online} strongly convex case convergence rate~\cite{lin2020collaborative}. 
	\item FL + bandit? 
	\item FL + TD convergence rate.
\end{itemize}

==> sec_conclude.tex <==
% !TEX ROOT=./main.tex

\section{Conclusions}
\begin{comment}
This paper provides a comprehensive and unified analysis of the convergence rate of FedAvg
and its accelerated variants in a general federated learning problem with heterogeneous local data and partial participation. We show that both Nesterov accelerated FedAvg and FedAvg
can achieve {\small{$\cO(\frac{1}{\sqrt{NT}})$}} linear speedup convergence for convex smooth problems and {\small{$\cO(\frac{1}{NT})$}} convergence for strongly 
convex smooth problems. In addition, we show that the local steps for stronlgy convex and convex smooth problems can be as large as {\small{$\cO(\sqrt{\frac{T}{N}})$}}, which can substantially save communication cost comparing to prior results. 
Furthermore, this work also makes algorithmic contributions. We not only prove that FedAvg can achieve exponential convergence for overparameterized strongly convex smooth problems, but also propose the MaSS accelerated Fedavg algorithm, which has provable speedup in convergence rate over FedAvg on quadratic problems. Last but not least, we empirically
verify the linear speedup of FedAvg and Nesterov accelerated FedAvg for strongly convex, convex smooth, and linear regression problems. The empirical results are well-aligned with our theories.		
\end{comment}

This paper provides a comprehensive and unified analysis of the convergence of FedAvg
and its accelerated variants in a general federated learning problem with heterogeneous local data and partial participation. 
We show that both Nesterov accelerated FedAvg and FedAvg can achieve linear speedup convergence for convex smooth problems and strongly 
convex smooth problems. We further prove that FedAvg can achieve geometric convergence for overparameterized strongly convex smooth problems. We also propose a new variant of FedAvg with momentum updates (FedMaSS), which has provable speedup in geometric convergence rate over FedAvg on quadratic problems. Last but not least, extensive empirical 
evaluations demonstrate the linear speedup of FedAvg and accelerated FedAvg under various settings.	



==> sec_convexsmoothsgd.tex <==
% !TEX ROOT=./main.tex

Stochastic gradient of device $k$ at time step $t$, at point $\vw_t^k$: 
	$\vg_{t,k} \coloneqq \vg_{t,k}(w_t^k)$,
	$ \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}, \xi_{t}^{k}\right) $,
	$\EE \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}\right)$.
One-step stochastic gradient of all devices:
$\vg_{t}=\sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) $, $\EE \vg_{t}= \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) \coloneqq \sum_{k=1}^{N} p_{k} \EE \vg_{t, k} = \ov{g}_t$.

\begin{lemma}
Under Assumption~\ref{ass:subgrad2}, we have the following bound
\begin{align}
	 \|\EE \vg_{t,k}\|^2 & \leq G_k^2	\label{eq:g3} \\
	\|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 & \leq  G_k^2 \label{eq:g2} \\
   \EE\| \vg_{t} \|^{2} &  \leq  \sum_{k=1}^N p_k G_k^2  \label{eq:g1}
\end{align}
\label{lma:gradient}
\end{lemma}
The first two inequalities directly follows from Assumption~\ref{ass:subgrad2} and the inequality
can be obtained by applying the convexity of the l2 norm and Jensen's inequality. 

\begin{lemma}
	With unbiased device sampling scheme, we have the following bound: 
	$$ \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \leq \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 $$
\label{lma:wdistance}
\end{lemma}
\begin{proof}
\begin{align*}
& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \\
=& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1} + \overline{\vv}_{t+1} - \vw^*\|^2\\
=& \EE_{\cS_{t+1}, \xi_{t}} \left[\|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \|\overline{\vv}_{t+1} - \vw^*\|^2\right] + 2\EE_{\xi_{t}} \left<\EE_{\cS_{t+1}} \overline{\vw}_{t+1} - \overline{\vv}_{t+1},   \overline{\vv}_{t+1} - \vw^*\right> \\
=& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 \\
\leq&  \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 %\label{eq:sgdcvxsmth1}
\end{align*}
where in the second line we use $\EE_{\cS_{t+1}} \overline{\vw}_{t+1}  = \overline{\vv}_{t+1}$. 
The first term can be bounded by consider different sampling scheme as in \eq{\ref{eq:partialsample}}.
\end{proof}

\begin{lemma}[Lemma 3~\cite{li2019convergence}]
Let $\eta_t$ and $E$ satisfy $\eta_0 \leq 2 \eta_t$ for all $t- t_0 \leq E - 1$, we have
$$\mathbb{E}\left[\sum_{k=1}^{N} p_{k}\left\|\overline{\mathbf{w}}_{t}-\mathbf{w}_{k}^{t}\right\|^{2}\right] \leq \sum_{k=1}^N p_k4 \eta_{t}^{2}(E-1)^{2} G_k^{2}$$
\label{lma:l3iclr}
\end{lemma}

\begin{theorem}
Let Assumption~\ref{ass:subgrad2} and Assumption~\ref{ass:lsmooth} hold, suppose we have a bound 
on our starting distance, i.e., $\|\vw_{0} - \vw^*\|^2 \leq \Delta_0$, set learning rate $\eta_t =  \left(\frac{\Delta_0}{ T [G^2( 4L(E-1)^2 + 1) + C]}\right)^{1/2}$, we have,
$$\EE[ F_t^*] - F^*  \leq \left(\frac{ \Delta_0 [G^2( 4L(E-1)^2 + 1) + C] }{T}\right)^{1/2}$$
where we denote $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$.
% \label{th:sgdcvxsmth}
\end{theorem}
\begin{proof}
With Lemma~\ref{lma:wdistance}, 
\begin{align}
	\EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \leq \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2\label{eq:sgdcvxsmth1}
\end{align}
and according to the definition of $\overline{\vv}_{t+1}$ in \eq{\ref{eq:vbar}}, we can expand the second term in \eq{\ref{eq:sgdcvxsmth1}} as follows:
\begin{align*}
\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2 
 &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*}\right\|^2 \\
 &=\left\|\ov{w}_{t}-\vw^{*}\right\|^{2}-2 \eta_{t} \left< \vg_{t}, \ov{w}_{t}-\vw^{*} \right>+\eta_{t}^{2}\left\|\vg_{t}\right\|^{2} 
\end{align*}
We take the expectation condition on $\vw_t$ over $\xi_t$, i.e., random samples at all devices:
\begin{align}
\EE\left[\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\ov{w}_{t}-\vw^{*}\|^{2}-2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*} \right> +\eta_{t}^{2} \EE\| \vg_{t} \|^{2}
\label{eq:expandsgd}
\end{align}

Now we focus on bounding $-2 \eta_{t} \left< \EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right>$ in \eq{\ref{eq:expandsgd}}: 

\begin{align*}
	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right> \\
 =  & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t}, \vw^{k}_t - \vw^{*}\right>\\
 \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\\
 \leq &\sum_{k=1}^N p_k \left[2 \eta_{t} (F_k(\vw^{k}_t) - F_k(\ov{w}_t) + \frac{L}{2} \|\ov{w}_t - \vw^{k}_t\|^2 ) + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\right]\\
 = & \sum_{k=1}^N p_k \eta_t L \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t))\\
 = &  \eta_t L \sum_{k=1}^N p_k \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - F(\ov{w}_t))
\end{align*}
Plug in this upper bound into \eq{\ref{eq:expandsgd}}, \eq{\ref{eq:sgdcvxsmth1}} and take totoal expectation over all samples at all iterations, we have
\begin{align}
\EE\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2 &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \vg_{t} \|^{2} + \eta_t L \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_t^2 C\\
&\leq\EE \|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  4L\eta_t^3(E-1)^2 G^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_t^2 C\\
&\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} G^2 +  4L\eta_t^3(E-1)^2 G^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t))+\eta_t^2 C \label{eq:cvxsgd1}
\end{align}
where in the second line and third line we use Lemma~\ref{lma:gradient}.

Sum two sides of \eq{\ref{eq:cvxsgd1}}, we require $\eta_t < 1$ and set $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$, 
\begin{align*}
	\sum_{t=0}^{T-1} 2\eta_t (\EE[F(\ov{w}_t)] - F^* ) & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} - \EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 + \sum_{t=0}^{T-1} (\eta_t^3 4LG^2(E-1)^2 + \eta_t^2 G^2+ \eta_t^2 C)\\ 
    & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} - \EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 + \sum_{t=0}^{T-1} (\eta_t^3 4LG^2(E-1)^2 + \eta_t^2 G^2+ \eta_t^2 C)\\ 
    & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2\left[ G^2 ( 4L(E-1)^2 + 1) + C\right]\\
    \sum_{t=0}^{T-1} 2\eta_t (\EE[F^*_t] - F^* ) & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2\left[ G^2 ( 4L(E-1)^2 + 1) + C\right]\\
\EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{\left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t }
\end{align*}
It will converge under the following conditions: $ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t = \infty$, 
$ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t^2 < \infty$. 
\begin{align*}
	\EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{\left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t } \\
	\EE[ F_t^*] - F^*  & \leq \frac{\Delta_0 + \left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2 }{2 \sum_{t=0}^{T-1} \eta_t }\\
	& \leq \left(\frac{ \Delta_0 [G^2( 4L(E-1)^2 + 1) + C] }{T}\right)^{1/2}
\end{align*}
where in the last line we set the learning rate satisfying $\eta_t =  \left(\frac{\Delta_0}{ T [G^2( 4L(E-1)^2 + 1) + C]}\right)^{1/2}$.
\end{proof}

==> sec_convexsmoothsgd_note.tex <==
% !TEX ROOT=./main.tex

Stochastic gradient of device $k$ at time step $t$, at point $\vw_t^k$: 
	$\vg_{t,k} \coloneqq \vg_{t,k}(w_t^k)$,
	$ \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}, \xi_{t}^{k}\right) $,
	$\EE \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}\right)$.
One-step stochastic gradient of all devices:
$\vg_{t}=\sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) $, $\EE \vg_{t}= \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) \coloneqq \sum_{k=1}^{N} p_{k} \EE \vg_{t, k} = \ov{g}_t$.

\begin{lemma}
Under Assumption~\ref{ass:subgrad2}, we have the following bound
\begin{equation}
	\eta_t^2 \|\EE \vg_{t,k}\|^2 \leq  \eta_t^2 G_k^2
	\label{eq:g3}
\end{equation}
\begin{equation}
	\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 \leq  \eta_t^2 G_k^2
	\label{eq:g2}
\end{equation}
\begin{align}
	  \eta_{t}^{2} \EE\| \vg_{t} \|^{2} 
	\leq   \eta_{t}^{2} \EE\| \sum_{k=1}^N p_k g_{t,k} \|^{2} 
	\leq   \eta_{t}^{2} \sum_{k=1}^N p_k \EE\| g_{t,k} \|^{2} 
	\leq   \eta_{t}^{2} \sum_{k=1}^N p_k G_k^2  \label{eq:g1}
\end{align}
\label{lma:gradient}
\end{lemma}


% Now the only term left in $C_1$ is $\eta_{t}^{2} \EE\| \vg_{t} \|^{2} $, follow the proof in Lemma 2~\cite{li2019convergence}:
% where in the third inequality we use the convexity of the l2 norm.

\begin{theorem}
Let Assumption~\ref{ass:subgrad2} and Assumption~\ref{ass:lsmooth} hold, suppose we have a bound 
on our starting distance, i.e., $\|\vw_{0} - \vw^*\|^2 \leq \Delta_0$, set learning rate $\eta_t =  \left(\frac{\Delta_0}{ T [G^2( 4L(E-1)^2 + 1) + C]}\right)^{1/2}$, we have,
$$\EE[ F_t^*] - F^*  \leq \left(\frac{ \Delta_0 [G^2( 4L(E-1)^2 + 1) + C] }{T}\right)^{1/2}$$
where we denote $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$.
% \label{th:sgdcvxsmth}
\end{theorem}

\begin{proof}
	

\begin{align}
\EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 &= \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1} + \overline{\vv}_{t+1} - \vw^*\|^2\\
&= \EE_{\cS_{t+1}, \xi_{t}} \left[\|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \|\overline{\vv}_{t+1} - \vw^*\|^2\right] \\
& \hspace{3em}+ 2\EE_{\xi_{t}} \left<\EE_{\cS_{t+1}} \overline{\vw}_{t+1} - \overline{\vv}_{t+1},   \overline{\vv}_{t+1} - \vw^*\right> \\
& = \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 \\
& \leq  \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 \label{eq:sgdcvxsmth1}
\end{align}
where in the second line we use $\EE_{\cS_{t+1}} \overline{\vw}_{t+1}  = \overline{\vv}_{t+1}$. 
The first term can be bounded by consider different sampling scheme. 
According to the definition of $\overline{\vv}_{t+1}$ in \eq{\ref{eq:vbar}}, we can expand the second term in \eq{\ref{eq:sgdcvxsmth1}} as follows:

\begin{align*}
\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2 
 &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*}\right\|^2 \\
 &=\left\|\ov{w}_{t}-\vw^{*}\right\|^{2}-2 \eta_{t} \left< \vg_{t}, \ov{w}_{t}-\vw^{*} \right>+\eta_{t}^{2}\left\|\vg_{t}\right\|^{2} 
\end{align*}
% \begin{align*}
% \left\|\ov{v}_{t+1}-\vw^{*}\right\|^2 
%  &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*}\right\|^2 \\
%  &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*} - \eta_t \ov{g}_t + \eta_t \ov{g}_t\right\|^2 
% \\
% & = \left\|\ov{w}_{t}- \eta_t \ov{g}_t  -\vw^{*} + \eta_t \ov{g}_t - \eta_{t} \vg_{t}\right\|^2 \\
% & = \left\|\ov{w}_{t}- \eta_t \ov{g}_t  -\vw^{*}\right\|^2  + 2\eta_t \left<\vw_t - \vw^* - \eta_t \ov{g}_t, \ov{g}_t - \vg_{t} \right> + \left\|\eta_t \ov{g}_t - \eta_{t} \vg_{t}\right\|^2 \\
%  &=\left\|\ov{w}_{t}-\vw^{*}\right\|^{2}-2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*} \right>+\eta_{t}^{2}\left\|\ov{g}_{t}\right\|^{2}  + \underbrace{2\eta_t \left<\vw_t - \vw^* - \eta_t \ov{g}_t, \ov{g}_t - \vg_{t} \right>}_{A_1} + \eta_{t}^2\left\| \ov{g}_t -  \vg_{t}\right\|^2
% \end{align*}

We take the expectation condition on $\vw_t$ over $\xi_t$, i.e., random samples at all devices:
\begin{align}
\EE\left[\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\ov{w}_{t}-\vw^{*}\|^{2}-2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*} \right> +\eta_{t}^{2} \EE\| \vg_{t} \|^{2}
\label{eq:expandsgd}
\end{align}

Now we focus on bounding $-2 \eta_{t} \left< \EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right>$ in \eq{\ref{eq:expandsgd}}: 

\begin{align*}
	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right> \\
 =  & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t}, \vw^{k}_t - \vw^{*}\right>\\
 \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\\
 \leq &\sum_{k=1}^N p_k \left[2 \eta_{t} (F_k(\vw^{k}_t) - F_k(\ov{w}_t) + \frac{L}{2} \|\ov{w}_t - \vw^{k}_t\|^2 ) + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\right]\\
 = & \sum_{k=1}^N p_k \eta_t L \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t))\\
 = &  \eta_t L \sum_{k=1}^N p_k \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - F(\ov{w}_t))
\end{align*}
Plug in this upper bound into \eq{\ref{eq:expandsgd}}, \eq{\ref{eq:sgdcvxsmth1}} and take totoal expectation over all samples at all iterations, we have
\begin{align}
\EE\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2 &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \vg_{t} \|^{2} + \eta_t L \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_t^2 C\\
&\leq\EE \|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  4L\eta_t^3(E-1)^2 G^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_t^2 C\\
&\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} G^2 +  4L\eta_t^3(E-1)^2 G^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t))+\eta_t^2 C \label{eq:cvxsgd1}
\end{align}

Sum two sides of \eq{\ref{eq:cvxsgd1}}, we require $\eta_t < 1$ and set $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$, 
\begin{align*}
	\sum_{t=0}^{T-1} 2\eta_t (\EE[F(\ov{w}_t)] - F^* ) & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} - \EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 + \sum_{t=0}^{T-1} (\eta_t^3 4LG^2(E-1)^2 + \eta_t^2 G^2+ \eta_t^2 C)\\ 
    & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} - \EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 + \sum_{t=0}^{T-1} (\eta_t^3 4LG^2(E-1)^2 + \eta_t^2 G^2+ \eta_t^2 C)\\ 
    & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2\left[ G^2 ( 4L(E-1)^2 + 1) + C\right]\\
    \sum_{t=0}^{T-1} 2\eta_t (\EE[F^*_t] - F^* ) & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2\left[ G^2 ( 4L(E-1)^2 + 1) + C\right]\\
\EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{\left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t }
\end{align*}
It will converge under the following conditions: $ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t = \infty$, 
$ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t^2 < \infty$. 
\begin{align*}
	\EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{\left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t } \\
	\EE[ F_t^*] - F^*  & \leq \frac{\Delta_0 + \left[G^2( 4L(E-1)^2 + 1) + C\right] \sum_{t=0}^{T-1} \eta_t^2 }{2 \sum_{t=0}^{T-1} \eta_t }\\
	& \leq \left(\frac{ \Delta_0 [G^2( 4L(E-1)^2 + 1) + C] }{T}\right)^{1/2}
\end{align*}
where in the last line we set the learning rate satisfying $\eta_t =  \left(\frac{\Delta_0}{ T [G^2( 4L(E-1)^2 + 1) + C]}\right)^{1/2}$.
\end{proof}

==> sec_convexsmoothsgdwthvariance.tex <==
% !TEX ROOT=./main.tex
Stochastic gradient of device $k$ at time step $t$, at point $\vw_t^k$: 
	$\vg_{t,k} \coloneqq \vg_{t,k}(w_t^k)$,
	$ \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}, \xi_{t}^{k}\right) $,
	$\EE \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}\right)$.
One-step stochastic gradient of all devices:
$\vg_{t}=\sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) $, $\EE \vg_{t}= \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) \coloneqq \sum_{k=1}^{N} p_{k} \EE \vg_{t, k} = \ov{g}_t$.
We further denote the following constants $\nu_{max}:=N\cdot\max_{k}p_{k}$ and $\nu_{min}:=N\cdot\min_{k}p_{k}$. 

% Let $\widetilde{F}_{k}(\mathbf{w})=p_{k} N F_{k}(\mathbf{w})$, Then the global objective change to the 
% average of all scaled local objectives. 
% $F(\mathbf{w})=\sum_{k=1}^{N} p_{k} F_{k}(\mathbf{w})=\frac{1}{N} \sum_{k=1}^{N} \widetilde{F}_{k}(\mathbf{w})$
% The constants were replaced as follows:
% $\widetilde{L} \triangleq \nu L, \widetilde{\mu} \triangleq_{S \mu,} \widetilde{\sigma}_{k}=\sqrt{\nu} \sigma,$ and $\widetilde{G}=\sqrt{\nu} G$, where $\nu=N \cdot \max _{k} p_{k}$ and $s=N \cdot \min _{k} p_{k}$

\begin{lemma}
Under Assumption~\ref{ass:subgrad2}, we have the following bound
\begin{align}
	 \|\EE \vg_{t,k}\|^2 & \leq G_k^2	\label{eq:g3} \\
	\|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 & \leq  G_k^2 \label{eq:g2} \\
   \EE\| \vg_{t} \|^{2} &  \leq  \sum_{k=1}^N p_k G_k^2  \label{eq:g1}
\end{align}
\label{lma:gradient}
\end{lemma}
The first two inequalities directly follows from Assumption~\ref{ass:subgrad2} and the inequality
can be obtained by applying the convexity of the l2 norm and Jensen's inequality. 

\begin{lemma}
	With unbiased device sampling scheme, we have the following bound: 
	$$ \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \leq \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 $$
\label{lma:wdistance}
\end{lemma}

\begin{proof}
\begin{align*}
& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \\
=& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1} + \overline{\vv}_{t+1} - \vw^*\|^2\\
=& \EE_{\cS_{t+1}, \xi_{t}} \left[\|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \|\overline{\vv}_{t+1} - \vw^*\|^2\right] + 2\EE_{\xi_{t}} \left<\EE_{\cS_{t+1}} \overline{\vw}_{t+1} - \overline{\vv}_{t+1},   \overline{\vv}_{t+1} - \vw^*\right> \\
=& \EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \overline{\vv}_{t+1}\|^2 + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 \\
\leq&  \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2 %\label{eq:sgdcvxsmth1}
\end{align*}
where in the second line we use $\EE_{\cS_{t+1}} \overline{\vw}_{t+1}  = \overline{\vv}_{t+1}$. 
The first term can be bounded by consider different sampling scheme as in \eq{\ref{eq:partialsample}}.
\end{proof}

\begin{lemma}[Lemma 3~\cite{li2019convergence}]
Let $\eta_t$ and $E$ satisfy $\eta_0 \leq 2 \eta_t$ for all $t- t_0 \leq E - 1$, we have
$$\mathbb{E}\left[\sum_{k=1}^{N} p_{k}\left\|\overline{\mathbf{w}}_{t}-\mathbf{w}_{k}^{t}\right\|^{2}\right] \leq \sum_{k=1}^N p_k4 \eta_{t}^{2}(E-1)^{2} G_k^{2}$$
\label{lma:l3iclr}
\end{lemma}

\begin{lemma}[Lemma 2~\cite{li2019convergence}]
$\mathbb{E}\left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} \leq \sum_{k=1}^{N} p_{k}^{2}\sigma_k^2 \leq \frac{1}{N}\nu_{\max}^2\sigma^2$
\label{lma:iclrvar}
\end{lemma}
\begin{proof}
	\begin{align} 
\mathbb{E}\left\|\mathbf{g}_{t}-\overline{\mathbf{g}}_{t}\right\|^{2} &=\mathbb{E}\left\|\sum_{k=1}^{N} p_{k}\left(\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)-\nabla F_{k}\left(\mathbf{w}_{t}^{k}\right)\right)\right\|^{2} \\ &=\sum_{k=1}^{N} p_{k}^{2} \mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)-\nabla F_{k}\left(\mathbf{w}_{t}^{k}\right)\right\|^{2} \\ & \leq \sum_{k=1}^{N} p_{k}^{2} \sigma_{k}^{2} \end{align}
\end{proof}

\begin{lemma}
Under Assumption~\ref{ass:lsmooth}, we have the following bound on the 
optimality gap.
$$\eta_t \sum_{k=1}^{N}p_{k}\left[F_{k}(w^{\ast})-F_{k}(\overline{w}_{t})\right] \leq-\eta_{t}^{2}\|\overline{g}_{t}\|^{2}+\eta_{t}^{2}L^{2}\sum_{k}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\eta_{t}^{3}L\mathbb{E}\|g_{t}\|^{2} $$
where $\eta_t$ denotes learning rate.
\label{lma:optgap}
\end{lemma}
\begin{proof}
Note that the expectation in here is taken w.r.t. $\xi_{t+1}^k$ for all $k$.
	\begin{align*}
	2\eta_{t}\EE\sum_{k=1}^{N}p_{k}\left[F_{k}(\vw^{\ast})-F_{k}(\overline{\vw}_{t})\right] & \leq 
	2\eta_{t}\EE \left[F(\overline{\vw}_{t+1})-F(\overline{\vw}_{t})\right]\\
	& \leq2\eta_{t}\mathbb{E}\langle\nabla F(\overline{\vw}_{t}),\overline{\vw}_{t+1}-\overline{\vw}_{t}\rangle+\eta_{t}L\mathbb{E}\|\overline{\vw}_{t+1}-\overline{\vw}_{t}\|^{2}\\
	% & =-2\eta_{t}^{2}\mathbb{E}\langle\nabla F(\overline{\vw}_{t}),\vg_{t}\rangle+\eta_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& =-2\eta_{t}^{2}\mathbb{E}\langle\nabla F(\overline{\vw}_{t}),\overline{\vg}_{t}\rangle+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}\\
	& =-\eta_{t}^{2}\left[\|\nabla F(\overline{\vw}_{t})\|^{2}+\|\overline{\vg}_{t}\|^{2}-\|\nabla F(\overline{\vw}_{t}) - \overline{\vg}_{t}\|^{2}\right]+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}\\
	& =-\eta_{t}^{2}\left[\|\nabla F(\overline{\vw}_{t})\|^{2}+\|\overline{\vg}_{t}\|^{2}-\|\nabla F(\overline{\vw}_{t})-\sum_{k}p_{k}\nabla F(\vw_{t}^{k})\|^{2}\right]+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}\\
	& \leq-\eta_{t}^{2}\left[\|\nabla F(\overline{\vw}_{t})\|^{2}+\|\overline{\vg}_{t}\|^{2}-\sum_{k}p_{k}\|\nabla F(\overline{\vw}_{t})-\nabla F(\vw_{t}^{k})\|^{2}\right]+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}\\
	& \leq-\eta_{t}^{2}\left[\|\nabla F(\overline{\vw}_{t})\|^{2}+\|\overline{\vg}_{t}\|^{2}-L^{2}\sum_{k}p_{k}\|\overline{\vw}_{t}-\vw_{t}^{k}\|^{2}\right]+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}\\
	& \leq-\eta_{t}^{2}\|\overline{\vg}_{t}\|^{2}+\eta_{t}^{2}L^{2}\sum_{k}p_{k}\|\overline{\vw}_{t}-\vw_{t}^{k}\|^{2}+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2}
	\end{align*}
\end{proof}

\begin{theorem}
Let Assumption~\ref{ass:subgrad2} and Assumption~\ref{ass:lsmooth} hold, suppose we have a bound 
on our starting distance, i.e., $\|\vw_{0} - \vw^*\|^2 \leq \Delta_0$, set learning rate $\eta_t =  \left(\frac{\Delta_0}{ T [G^2( 4L(E-1)^2 + 1) + C]}\right)^{1/2}$, we have,
$$\EE[ F_t^*] - F^*  \leq \left(\frac{ \Delta_0 [G^2( 4L(E-1)^2 + 1) + C] }{T}\right)^{1/2}$$
where we denote $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$.
% \label{th:sgdcvxsmth}
\end{theorem}

\begin{proof}
	

With Lemma~\ref{lma:wdistance}, 
\begin{align}
	\EE_{\cS_{t+1}, \xi_{t}} \|\overline{\vw}_{t+1} - \vw^*\|^2 \leq \eta_t^2 C + \EE_{\xi_t} \|\overline{\vv}_{t+1} - \vw^*\|^2\label{eq:sgdcvxsmth1}
\end{align}
and according to the definition of $\overline{\vv}_{t+1}$ in \eq{\ref{eq:vbar}}, we can expand the second term in \eq{\ref{eq:sgdcvxsmth1}} as follows:
\begin{align*}
\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2 
 &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*}\right\|^2 \\
 &=\left\|\ov{w}_{t}-\eta_{t} \vg_{t}-\vw^{*} - \eta_t \ov{g}_t + \eta_t \ov{g}_t\right\|^2 
\\
& = \left\|\ov{w}_{t}- \eta_t \ov{g}_t  -\vw^{*} + \eta_t \ov{g}_t - \eta_{t} \vg_{t}\right\|^2 \\
& = \left\|\ov{w}_{t}- \eta_t \ov{g}_t  -\vw^{*}\right\|^2  + 2\eta_t \left<\vw_t - \vw^* - \eta_t \ov{g}_t, \ov{g}_t - \vg_{t} \right> + \left\|\eta_t \ov{g}_t - \eta_{t} \vg_{t}\right\|^2 \\
 &=\left\|\ov{w}_{t}-\vw^{*}\right\|^{2}-2 \eta_{t} \left<\ov{g}_t, \ov{w}_{t}-\vw^{*} \right>+\eta_{t}^{2}\left\|\ov{g}_{t}\right\|^{2}  + \underbrace{2\eta_t \left<\vw_t - \vw^* - \eta_t \ov{g}_t, \ov{g}_t - \vg_{t} \right>}_{A_1} + \eta_{t}^2\left\| \ov{g}_t -  \vg_{t}\right\|^2
\end{align*}

We take the expectation condition on $\vw_t$ over $\xi_t$, i.e., random samples at all devices and
note that $\EE A_1 = 0$:
\begin{align}
\EE\left[\left\|\ov{v}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\ov{w}_{t}-\vw^{*}\|^{2}-2 \eta_{t} \left<\ov{g}_t, \ov{w}_{t}-\vw^{*} \right> +\eta_{t}^{2} \| \ov{g}_{t} \|^{2} + \EE \eta_{t}^2\left\| \ov{g}_t -  \vg_{t}\right\|^2
\label{eq:expandsgd}
\end{align}

Now we focus on bounding $-2 \eta_{t} \left< \EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right>$ in \eq{\ref{eq:expandsgd}}: 

\begin{align*}
	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}-\vw^{*}\right> \\
 =  & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t}, \vw^{k}_t - \vw^{*}\right>\\
 \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t}- \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\\
 \leq &\sum_{k=1}^N p_k \left[2 \eta_{t} (F_k(\vw^{k}_t) - F_k(\ov{w}_t) + \frac{L}{2} \|\ov{w}_t - \vw^{k}_t\|^2 ) + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\right]\\
 = & \sum_{k=1}^N p_k \eta_t L \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t))\\
 = &  \eta_t L \sum_{k=1}^N p_k \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - F(\ov{w}_t))
\end{align*}
Plug in this upper bound into \eq{\ref{eq:expandsgd}}, \eq{\ref{eq:sgdcvxsmth1}} and take totoal expectation over all samples at all iterations, we have
\begin{align}
\EE\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2 &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \ov{g}_{t} \|^{2} + \eta_t L \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2 \nonumber \\
& + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_{t}^2\EE\left\| \ov{g}_t -  \vg_{t}\right\|^2+ \eta_t^2 C\\
&\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2} + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_{t}^{2} G^2 +4 L \eta_{t}^{3}E^{2} G^{2} + \eta_{t}^{2}\sum_{k=1}^{N} p_{k}^{2}\sigma_k^2 + \eta_t^2 C\\
&\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2} + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \underbrace{\eta_{t}^{2} G^2 +4 L \eta_{t}^{2}E^{2} G^{2} + \eta_{t}^{2}\sum_{k=1}^{N} p_{k}^{2}\sigma_k^2 + \eta_t^2 C}_{\eta_t^2 A}
\label{eq:cvxsgd1}
\end{align}
where we use Lemma~\ref{lma:l3iclr}, Lemma~\ref{lma:iclrvar} and $\eta_t < 1$

Sum two sides of \eq{\ref{eq:cvxsgd1}}, and set constant learning rate $\eta_t = \eta$ and $F^*_t = \min_{t \in [0, T-1]} F(\ov{w}_t)$.
\begin{align*}
    \sum_{t=0}^{T-1} 2\eta_t (\EE[F^*_t] - F^* ) & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2 A\\
\EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{A \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t }
\end{align*}
where $A = (1 +4 L E^{2})G^{2} + \sum_{k=1}^{N} p_{k}^{2}\sigma_k^2 + C$.
It will converge under the following conditions: $ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t = \infty$, 
$ \lim_{T \rightarrow \infty }\sum_{t=0}^{T-1} \eta_t^2 < \infty$. 
\begin{align*}
	% \EE[ F_t^*] - F^*  & \leq \frac{\|\ov{w}_{0}-\vw^{*}\|^{2}}{2 \sum_{t=0}^{T-1} \eta_t } + \frac{A \sum_{t=0}^{T-1} \eta_t^2}{2 \sum_{t=0}^{T-1} \eta_t } \\
	\EE[ F_t^*] - F^*  & \leq \frac{\Delta_0 + A \sum_{t=0}^{T-1} \eta_t^2 }{2 \sum_{t=0}^{T-1} \eta_t }\\
	& \leq \left(\frac{ \Delta_0 A }{T}\right)^{1/2}
\end{align*}
where in the last line we set the learning rate satisfying $\eta_t =  \left(\frac{\Delta_0}{ TA }\right)^{1/2}$.
\end{proof}




% \begin{align}
% 	\EE\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2 &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \ov{g}_{t} \|^{2} + \eta_t L \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2 + 2 \eta_{t} (F^* - \EE F(\ov{w}_t)) + \eta_{t}^2\EE\left\| \ov{g}_t -  \vg_{t}\right\|^2+ \eta_t^2 C\\
% &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2}+\eta_{t}^{2} \EE\| \ov{g}_t \|^{2} + \eta_t L \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2  \nonumber\\
%  & - \eta_{t}^{2}\EE\|\overline{\vg}_{t}\|^{2}+\eta_{t}^{2}L^{2}\sum_{k}p_{k}\EE\|\overline{\vw}_{t}-\vw_{t}^{k}\|^{2}+\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2} + \eta_{t}^2\EE\left\| \ov{g}_t -  \vg_{t}\right\|^2 +\eta_t^2 C \\
%  &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2} + (\eta_t L + \eta_{t}^{2}L^{2}) \sum_{k=1}^N p_k \EE \|\ov{w}_t - \vw^{k}_t\|^2  +\eta_{t}^{3}L\mathbb{E}\|\vg_{t}\|^{2} + \eta_{t}^2\EE\left\| \ov{g}_t -  \vg_{t}\right\|^2+\eta_t^2 C \\
%   &\leq \EE\|\ov{w}_{t}-\vw^{*}\|^{2} + \underbrace{4(1 + \eta_{t}L)\eta_t^3LE^2G^2  +\eta_{t}^{3}LG^2 + \frac{1}{N}\eta_{t}^2\nu_{\max}^2\sigma^2 +\eta_t^2 C }_{A}
% \end{align}

% \begin{align}
% 		\EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2}  + TA\\ 
%     & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} - \EE\left\|\ov{w}_{T}-\vw^{*}\right\|^2 + \sum_{t=0}^{T-1} (\eta_t^3 4LG^2(E-1)^2 + \eta_t^2 G^2+ \eta_t^2 C)\\ 
%     & \leq \EE \|\ov{w}_{0}-\vw^{*}\|^{2} + \sum_{t=0}^{T-1}\eta_t^2\left[ G^2 ( 4L(E-1)^2 + 1) + C\right]\\
% \end{align}

==> sec_cvxnonsm.tex <==
% !TEX ROOT=./main.tex


% \textbf{Full Device Participation}

% \begin{itemize}
% 	\item Stochastic Subgradient of device $k$ at time step $t$, at point $w_{t,k}$: 
% 	$$\vg_{t,k} \coloneqq \vg_{t,k}(w_t^k)$$
% 	$$ \vg_{t, k} \in \partial F_{k}\left(w_{t}^{k}, \xi_{t}^{k}\right) $$
% 	$$\EE \vg_{t, k} \in \partial F_{k}\left(w_{t}^{k}\right)$$
% \item  One-step stochastic subgradient of all devices.
% $$\vg_{t}=\sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) $$
% \begin{align}
% 	\EE \vg_{t}= \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) \coloneqq \sum_{k=1}^{N} p_{k} \EE \vg_{t, k}
% 	\label{eq:egt}
% \end{align}
% \end{itemize}

\begin{theorem}
	Let Assumption~\ref{ass:subgrad2} hold, 
	then the FedAvg with partial device participation satisfies
	\begin{align}
		 \EE[F^*_t] - F^* &\leq  \left(\frac{\Delta_0[C+ G^2 \left(3 + 4(E-1)^2\right)]}{T}\right)^{1/2}
	\end{align}
	where $\eta_t = \eta_t  = \sqrt{ \frac{\Delta_0}{T[C+ G^2 \left(3 + 4(E-1)^2\right)]}}$,
	$F^*_t \coloneqq \min_{t \in [0, T-1]} F(\overline{\vw}_t)$.
	% $R = \sqrt{ \frac{\Delta_0}{L}},$
	% $L=\sum_{k=1}^N \left( G^2 \left(3 + 4(E-1)^2\right)\right).$
	% \label{th:cvxnonsmoth}
\end{theorem}
\begin{proof}
% In full device active setting, we have $\overline{\vw}_{t+1}=\overline{\vv}_{t+1}$,
Follow the same reasoning in the proof of Theorem~\ref{th:sgdcvxsmth} \eq{\ref{eq:expandsgd}}, we have
\begin{align}
\EE\left[\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\bar{\vw}_{t}-\vw^{*}\|^{2}-2 \eta_{t} \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)+\eta_{t}^{2} \EE\| \vg_{t} \|^{2}	
\label{eq:expand}
\end{align}
Note that since $\EE \vg_t = \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(\vw_{t}^{k}\right) \neq \EE \sum_{k=1}^Np_k \vg_{t,k}(\overline{\vw}_t)$, therefore $\EE \vg_t \notin \partial F(\overline{\vw}_t)$, we cannot directly use the convex definition to
upper bound $- \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)$ in \eq{\ref{eq:expand}}, as classic SGD proof did. 

Now we focus on bounding $-2 \eta_{t} \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)$ in \eq{\ref{eq:expand}}: 
\begin{align}
	& -2 \eta_{t} \left<\EE \vg_{t}, \bar{\vw}_{t}-\vw^{*} \right>\\
  = & 2 \eta_{t} \sum_{k=1}^N p_k \left(-\left<\EE \vg_{t,k}, \bar{\vw}_{t}-\vw^{*} \right> \right) \\
  \leq& 2 \eta_{t} \sum_{k=1}^N p_k  \left(\frac{1}{2\eta_t} \|\overline{\vw}_t - \vw_t^k\|^2 + \frac{\eta_t}{2} \|\EE \vg_{t,k}\|^2 - (F_k(\vw_t^k) - F_k(\vw^*) \right) \\
  =& \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 
  - 2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F_k(\vw^*)) \\
  =& \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 
  - 2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*) \label{eq:exp4}
\end{align}
where in the third line we use the following derivation:
\begin{align}
	& -\left<\EE \vg_{t,k}, \bar{\vw}_{t} - \vw^{*} \right>\\
=& - \left<\EE \vg_{t,k}, \bar{\vw}_{t} - \vw_t^k +  \vw_t^k - \vw^{*} \right>\\
=& - \left<\EE \vg_{t,k}, \bar{\vw}_{t} - \vw_t^k\right> - \left<\EE \vg_{t,k}, \vw_t^k - \vw^{*} \right>\\
\leq & - \left<\EE \vg_{t,k}, \bar{\vw}_{t} - \vw_t^k\right> - (F_k(\vw_t^k) - F_k(\vw^*)) \label{eq:3}\\
\leq & \frac{1}{2\eta_t} \|\bar{\vw}_t - \vw_t^k\|^2 + \frac{\eta_t}{2} \|\EE \vg_{t,k}\|^2
- (F_k(\vw_t^k) - F_k(\vw^*)) \label{eq:4}
\end{align}
where in \eq{\ref{eq:3}} we use the definition of convexity and in \eq{\ref{eq:4}} we use Cauchy-Schwarz inequality and AM-GM inequality $-\langle\va, \vb\rangle=\langle\va,-\vb\rangle \leqslant|\va||\vb| \leqslant \frac{1}{2}\left(|\va|^{2}+|\vb|^{2}\right)$.


Now we plug in \eq{\ref{eq:exp4}} into \eq{\ref{eq:expand}}:
\begin{align}
	\Delta_{t+1} \leq& \|\bar{\vw}_{t}-\vw^{*}\|^{2} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2}  + \eta_t^2 C \\
	& + \underbrace{\sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2}_{A_1} +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2
  - 2\eta_t\underbrace{\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*)}_{A_2} \label{eq:cvxmain2}
\end{align}

$A_1$ can be bounded by Lemma 3 in~\cite{li2019convergence}, 


Now we bound $A_2$:
\begin{align}
	& \sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*) \\
 = & \sum_{k=1}^N p_k (F_k(\vw_t^k) - F_k(\overline{w}_t) + F_k(\overline{w}_t) - F^*) \\
 = & \sum_{k=1}^N p_k (F_k(\vw_t^k) - F_k(\overline{w}_t) ) + (F(\overline{w}_t) - F^*)\\ 
 \geq & \sum_{k=1}^{N} P_{k}\left<\EE g_{t k}\left(\overline{\vw}_{t}\right), \vw_{t}^k-\overline{\vw}_{t}\right> + (F(\overline{w}_t) - F^*)\\
 \geq& -\frac{1}{2} \sum_{k=1}^{N} P_{k} (\eta_t \|\EE \vg_{t,k}(\overline{\vw}_t) \|^2 + \frac{1}{\eta_t} \|\vw_t^k - \overline{\vw}_t\|^2) + (F(\overline{w}_t) - F^*) \label{eq:cvxa24}
\end{align}
where in fourth line we use Cauchy-Schwarz inequality and AM-GM inequality. 


Now we plug in \eq{\ref{eq:cvxa24}} into \eq{\ref{eq:cvxmain2}}:
\begin{align}
	\Delta_{t+1} & \leq \Delta_t + 
	\eta_{t}^{2} \EE\| \vg_{t} \|^{2} + \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 + \eta_t^2 C \\
	 &- 2 \eta_t \left(-\frac{1}{2} \sum_{k=1}^{N} P_{k} (\eta_t \|\EE \vg_{t,k}(\overline{\vw}_t) \|^2 + \frac{1}{\eta_t} \|\vw_t^k - \overline{\vw}_t\|^2) + (F(\overline{w}_t) - F^*) \right)  + \eta_t^2 C \\
	& \leq \Delta_t + 
	\eta_{t}^{2} \EE\| \vg_{t} \|^{2} + \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2  + \eta_t^2 C  \\
	& +\sum_{k=1}^{N} P_{k} (\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t) \|^2 + \|\vw_t^k - \overline{\vw}_t\|^2) - 2\eta_t (F(\overline{w}_t) - F^*) \\
	& = \Delta_t + \underbrace{\eta_{t}^{2} \EE\| \vg_{t} \|^{2} +\sum_{k=1}^N p_k  ( 2\|\overline{\vw}_t - \vw_t^k\|^2  +  \eta_t^2 \|\EE \vg_{t,k}\|^2 + \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t) \|^2 ) + \eta_t^2 C }_{\eta_t^2C_1}  - 2\eta_t (F(\overline{w}_t) - F^*) \label{eq:main3}
\end{align}
Apply Lemma~\ref{lma:gradient} and Lemma~\ref{lma:l3iclr} in the last line, we can bound $C_1$ as follows:
\begin{align}
\eta_t^2 C_1  = \eta_t^2 [\sum_{k=1}^N p_k G_k^2 \left(3 + 4(E-1)^2\right) + C]  = \eta_t^2 [C+ G^2 \left(3 + 4(E-1)^2\right)]
\end{align}
Rearrange the last inequality:
\begin{align}
	2\eta_t (\EE[F(\overline{w}_t)] - F^*) \leq \Delta_t - \Delta_{t+1} + \eta_t^2 C_1 
\end{align}
Sum over two sides from $t=0$ to $t = T- 1$ and define $F^*_t \coloneqq \min_{t \in [0, T-1]} F(\overline{\vw}_t)$
\begin{align}
	\sum_{t=0}^{T-1} 2\eta_t(\EE[F(\overline{w}_t)] - F^*) & \leq \Delta_0 - \Delta_T + \sum_{t=0}^{T-1} \eta_t^2 C_1 \\
	\sum_{t=0}^{T-1} 2\eta_t(\EE[F(\overline{w}_t)]- F^*) & \leq \Delta_0 + \sum_{t=0}^{T-1} \eta_t^2 C_1 \\
    \EE[F^*_t] - F^* &\leq \frac{\Delta_0 + \sum_{t=0}^{T-1} \eta_t^2C_1 }{ \sum_{t=0}^{T-1}  2 \eta_t}\\
    \EE[F^*_t] - F^* &\leq  \left(\frac{\Delta_0[C+ G^2 \left(3 + 4(E-1)^2\right)]}{T}\right)^{1/2}
\end{align}
where in last line we let $\eta_t  = \sqrt{ \frac{\Delta_0}{T[C+ G^2 \left(3 + 4(E-1)^2\right)]}}$.

% Now we discuss how to bound the term $C_1$ in \eq{\ref{eq:main3}}
% Assume Assumption~\ref{ass:subgrad2}, $\eta_t$ is non-increasing, and $\eta_t \leq 2\eta_{t+E}$ for all $t\geq 0$, according to Lemma 3 in~\cite{li2019convergence}, we have


% \begin{equation}
% \mathbb{E}\left[\sum_{k=1}^{N} p_{k}\left\|\overline{\mathbf{w}}_{t}-\mathbf{w}_{k}^{t}\right\|^{2}\right] \leq \sum_{k=1}^N p_k4 \eta_{t}^{2}(E-1)^{2} G_k^{2}
% 	\label{eq:g4}
% \end{equation}


% Assume Assumption~\ref{ass:subgrad2}, we have 
% \begin{equation}
% 	\eta_t^2 \|\EE \vg_{t,k}\|^2 \leq  \eta_t^2 G_k^2
% 	\label{eq:g3}
% \end{equation}
% and
% \begin{equation}
% 	\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 \leq  \eta_t^2 G_k^2
% 	\label{eq:g2}
% \end{equation}


% Now the only term left in $C_1$ is $\eta_{t}^{2} \EE\| \vg_{t} \|^{2} $, follow the proof in Lemma 2~\cite{li2019convergence}: 
% \begin{align}
% 	  \eta_{t}^{2} \EE\| \vg_{t} \|^{2} 
% 	\leq   \eta_{t}^{2} \EE\| \sum_{k=1}^N p_k g_{t,k} \|^{2} 
% 	\leq   \eta_{t}^{2} \sum_{k=1}^N p_k \EE\| g_{t,k} \|^{2} 
% 	\leq   \eta_{t}^{2} \sum_{k=1}^N p_k G_k^2  \label{eq:g1}
% \end{align}
% where in the third inequality we use the convexity of the l2 norm.

% Combine \eq{\ref{eq:g4}},\eq{\ref{eq:g3}},\eq{\ref{eq:g2}}, \eq{\ref{eq:g1}},
% we have 
% \begin{align}
% \eta_t^2 C_1  = \eta_t^2 [\sum_{k=1}^N p_k G_k^2 \left(3 + 4(E-1)^2\right) + C]  = \eta_t^2 [C+ G^2 \left(3 + 4(E-1)^2\right)]
% \end{align}

\end{proof}


==> sec_exp_note.tex <==
% !TEX ROOT=./main.tex



\section{Numerical Experiments}
\subsection{Strongly Convex}

\begin{figure}[h!]
\centering
\begin{tabular}{cc}
	\includegraphics[width=0.45\textwidth]{fig/paper-stronglycvxsmthspeedupNodesT-min-w8a-epsilon0131-reg1e-05.pdf} & 
\includegraphics[width=0.45\textwidth]{fig/paper-stronglycvxsmthspeedupEpochsT-min-w8a-epsilon0131-reg1e-05.pdf} \\
\end{tabular}
	\caption{Logistic regression with regularization $1e-5$. The linear speed up w.r.t the number of nodes and number of epochs. The synthetic dataset has $N=49749$ samples, evenly distributed on $1, 2, 4, 8, 16, 32$ devices. The figure shows the number of iterations/rounds needed to converge to $\epsilon-$accuracy, where $\epsilon=0.005$. The learning rate is decayed as the $\eta_t = \min(32, \frac{Nc}{1 + t})$, where we extensively search the best learning rate $c \in \{2^{-1}c, 2^{-2}c, c, 2c, 2^{2}c\}$ and for each configuration. Batch size is 4 in this case.}
\end{figure}



\subsection{Convex smooth objective}

\begin{figure}[h!]
\centering
\begin{tabular}{cc}
	\includegraphics[width=0.45\textwidth]{fig/paper-cvxsmoothspeedupNodesT-min-w8a-epsilon0134-reg0.pdf} & 
\includegraphics[width=0.45\textwidth]{fig/paper-cvxsmoothspeedupEpochsT-min-w8a-epsilon0134-reg0.pdf} \\
\end{tabular}
	\caption{Logistic regression without regularization. The linear speed up w.r.t the number of nodes and number of epochs. The w8a dataset has $N=49749$ samples, evenly distributed on $1, 2, 4, 8, 16, 32, 64, 128, 256, 512, 1024$ devices. The figure shows the number of iterations needed to converge to $\epsilon-$accuracy, where $\epsilon=0.02$. The learning rate is decayed as the $\eta_t = \min(\eta_0, \frac{Nc}{1 + t})$, where we extensively search the best learning rate $c \in \{2^{-1}c, 2^{-2}c, c, 2c, 2^{2}c\}$, $\eta_0 \in \{1, 32\}$ and for each configuration. Batch size is 4 in this case.}
\end{figure}




\subsection{Linear regression}






% \begin{figure}
% \begin{tabular}{cc}
% 	\includegraphics[width=0.5\textwidth]{fig/synthetic_balance_0_0_loss.pdf} & 
% 	\includegraphics[width=0.5\textwidth]{fig/synthetic_balance_0_0_accuracy.pdf} \\
% 	\includegraphics[width=0.5\textwidth]{fig/synthetic_balance_0_0_lossuser30TuneE.pdf} & 
% 	\includegraphics[width=0.5\textwidth]{fig/synthetic_balance_0_0_lossuser40TuneE.pdf} \\
% \end{tabular}
% \caption{Each user has 250 samples, non-iid setting, full device participation. Constant learning rate 0.01.}
% \end{figure}

\subsection{SGD}
We examine the practical speedup on a linear regression problem, 
$ F(\vw) = \sum_{k=1}^N p_kF_k(\vw)$, the objective function on each local device $k$ is given by, $F_k(\vw) = \frac{1}{N_k} \sum_{i=1}^{N_k} (\vw^T\vx_i^k + b  - y_i^k)^2$, where we generated i.i.d. data $\vx_i^k$ for all devices. At each communication round, all devices participated
in synchronization. 

\begin{figure}
\centering
\begin{tabular}{cc}
	\includegraphics[width=0.5\textwidth]{fig/synthetic_linear_regression_1k_6k-epsilon01-logTrue.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/synthetic_linear_regression_1k_6k-epsilon001-logTrue-epoch-1.pdf} \\
(a) $\epsilon=0.01$  & (b) $\epsilon=0.001$
\end{tabular}
	\caption{The linear speed up w.r.t the number of nodes. The synthetic dataset has $6000$ samples, evenly distributed on $10, 50, 100, 500, 1000$ devices. The figure shows the number of iterations needed to converge to $\epsilon$. The learning rate is decayed as the $\eta_t = \frac{1}{c + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1\mathrm{e}{-2}, 1\mathrm{e}{-3}, 1\mathrm{e}{-4}, 1\mathrm{e}{-5}, 1\mathrm{e}{-6}\}$ for each configuration. Batch size is 6 in this case.}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{fig/synthetic_linear_regression_1k_6k-epsilon001-logTrue-epoch-1-2-3-4-b4-adapt0.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/iteration_EandN-synthetic_linear_regression_1k_6k-epsilon01.pdf} 
 \\
(a) $\epsilon=0.01$  & (b) $N/E = 10$ 
\end{tabular}
	\caption{linear regression. The linear speed up w.r.t the number of nodes. The synthetic dataset has $6000$ samples, evenly distributed on $10, 20, 30, 40, 50, 60, 80, 100, 200, 300, 400, 500, 600, 750, 1000$ devices. The figure shows the number of iterations needed to converge to $\epsilon$. The learning rate is decayed as the $\eta_t = \frac{1}{c + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1\mathrm{e}{-2}, 1\mathrm{e}{-3}, 1\mathrm{e}{-4}, 1\mathrm{e}{-5}, 1\mathrm{e}{-6}\}$ for each configuration. Batch size is 4 in this case.}
\end{figure}


\begin{figure}
\centering
% \begin{tabular}{cc}
% \includegraphics[width=0.5\textwidth]{fig/synthetic_linear_regression_noise1e-02-epsilon1e-02-logTrue-epoch-1-b4} \\ 
\includegraphics[width=0.5\textwidth]{fig/synthetic_linear_regression_noise1e-02-epsilon01008-logTrue-epoch-1-b4-adapt0.pdf} \\ 
% \end{tabular}
(a) $\epsilon=0.01$ \\
	\caption{The linear speed up w.r.t the number of nodes. The synthetic dataset has $6000$ samples, evenly distributed on $10, 20, 30, 40, 50, 60, 80, 100, 200, 300, 400, 500, 600, 750, 1000$ devices. The figure shows the number of iterations needed to converge to $\epsilon$. The learning rate is decayed as the $\eta_t = \frac{1}{c + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1\mathrm{e}{-2}, 1\mathrm{e}{-3}, 1\mathrm{e}{-4}, 1\mathrm{e}{-5}, 1\mathrm{e}{-6}\}$ for each configuration. Batch size is 4 in this case. 
	We add Gaussian noise with zero mean and 0.01 standard deviation.}
\end{figure}


What is the relationship between $N/E$ and iteration $T$ in strongly convex function? $linear regression$, no noise. 
\begin{itemize}
	\item $N/E = 10$
	\item $N=10, E=1$, $N=20, E=2$, $N=30, E=3$, $N=40, E=4$, $N=50, E=5$, $N=100, E=10$.
\end{itemize} 


Does convex smooth function have linear speedup?

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{fig/synthetic_logistic_regression_small-epsilon09-logTrue-epoch-1-b4-regularization0.pdf} \\ 
(a) $\epsilon=0.9$ \\
\caption{Convex smooth objectives (logistic regression with zero l2-regularization) The number of iterations w.r.t the number of nodes. The synthetic dataset has $6000$ samples, evenly distributed on $10, 50, 100, 500, 1000$ devices. The figure shows the number of iterations needed to converge to $\epsilon-$accuracy. The learning rate is decayed as the $\eta_t = \frac{1}{c + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1\mathrm{e}{-2}, 1\mathrm{e}{-3}, 1\mathrm{e}{-4}, 1\mathrm{e}{-5}, 1\mathrm{e}{-6}\}$ for each configuration. Batch size is 4 in this case.}
\end{figure}




\begin{figure}
\centering
\begin{tabular}{cc}
	\includegraphics[width=0.5\textwidth]{fig/speedupEpochsT-synthetic_logistic_regression_iclr300-epsilon07-b4-adapt0.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/speedupEpochsRounds-synthetic_logistic_regression_iclr300-epsilon07-b4-adapt0.pdf} \\
	\includegraphics[width=0.5\textwidth]{fig/speedupNodesT-synthetic_logistic_regression_iclr300-epsilon07-b4-adapt0.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/speedupNodesRounds-synthetic_logistic_regression_iclr300-epsilon07-b4-adapt0.pdf} \\
\end{tabular}
	\caption{Logistic regression with regularization $0.001$. The linear speed up w.r.t the number of nodes and number of epochs. The synthetic dataset has $42000$ samples, evenly distributed on $10, 20, 30, 40, 50, 100, 1000$ devices. The figure shows the number of iterations/rounds needed to converge to $\epsilon-$accuracy. The learning rate is decayed as the $\eta_t = \frac{1}{1 + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1, 0.1, 0.01\}$ for each configuration. Batch size is 4 in this case.}
\end{figure}



\begin{figure}
\centering
\begin{tabular}{cc}
	\includegraphics[width=0.5\textwidth]{fig/speedupEpochsT-synthetic_logistic_regression_iclr300-epsilon07-b4-reg0-adapt0.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/speedupEpochsRounds-synthetic_logistic_regression_iclr300-epsilon07-b4-reg0-adapt0.pdf} \\
	\includegraphics[width=0.5\textwidth]{fig/speedupNodesT-synthetic_logistic_regression_iclr300-epsilon07-b4-reg0-adapt0.pdf} & 
\includegraphics[width=0.5\textwidth]{fig/speedupNodesRounds-synthetic_logistic_regression_iclr300-epsilon07-b4-reg0-adapt0.pdf} \\
\end{tabular}
	\caption{Logistic regression with regularization $0$. The linear speed up w.r.t the number of nodes and number of epochs. The synthetic dataset has $42000$ samples, evenly distributed on $10, 20, 30, 40, 50, 100, 1000$ devices. The figure shows the number of iterations/rounds needed to converge to $\epsilon-$accuracy. The learning rate is decayed as the $\eta_t = \frac{1}{1 + t \times a}$, where we extensively search the best learning rate $c \in \{1, 10\}$ and $a \in \{1, 0.1, 0.01\}$ for each configuration. Batch size is 4 in this case.}
\end{figure}


% /media/Research/linkaixi/env/py36/bin/python /home/linkaixi/Dropbox/recsys/convexFed/main.py --dataset=synthetic_logistic_regression_small --epsilon=0.01 --num_rounds=500000 --num_epochs=1 --number_user=10 --learning_rate=0.001 --is_decay=True --lrconst=1 --machine=gpu --batch_size=4 --num_iteration=50000 --model=logisticregression --optimizer=fedave --dimension=60 --adapt=0
% \subsection{Nesterov}


==> sec_impact.tex <==
% !TEX ROOT=./main.tex

% Broader impact: Authors are asked to include a section in their submissions discussing the broader impact of their work, including possible societal consequences — -both positive and negative.
\section{Broader impact}
With the growing availability of mobile devices and their increasing ability to capture data, enormous amounts of information can potentially be integrated to help improve and transform people's lives in many aspects such as personalized and enhanced services~\cite{fallah2020personalized,47586} and precision medicine~\cite{uddin2019artificial,frohlich2018hype}, to name a few.

Meanwhile, data breaches from central servers of big companies have become increasingly common, raising concerns about privacy and information security when individual clients' information is aggregated and stored centrally. 

The challenge we face is therefore to properly integrate and leverage data from different sources to arrive at better solutions, while at the same time minimizing privacy risks. This trade-off between efficiency and privacy/security
lies at the heart of many applications, including 
but not limited to recommendation systems~\cite{chen2018federated}, virtual assistants~\cite{lamautonomy}, and mobile keyboard prediction~\cite{47586}.

Federated learning has emerged as a promising solution to the challenge. Built on insights from decentralized and distributed optimization, it aggregates information by integrating model \emph{parameters} learned locally at each source, eliminating the need to transmit and store data centrally. 

This desirable feature makes federated learning an effective tool to balance efficiency and privacy not just in the aforementioned applications with mobile devices, but also in other settings such as healthcare where it has the potential to save millions of lives. Under the unprecedented outbreak
of Covid'19, coronavirus patients have filled emergency rooms nationwide. It is imperative to have reliable, robust machine learning
solutions that could help doctors diagnose and treat patients. However,  Health Insurance Portability and Accountability (HIPAA) regulations~\cite{assistance2003summary}
impose strict restrictions on sharing patients' clinical data: privacy is a
top priority when developing solutions by leveraging information from different medical institutions. 
Therefore, propelling the frontiers of federated learning to develop more efficient 
algorithms under the privacy-preserving constraint has never been more
important.

Two important aspects where federated learning departs from traditional distributed optimization is the heterogeneity of data at different sources and the fact that not all local devices/sources are able to participate in the model averaging at every iteration. In this general setting, the question remains as to whether joint learning still enjoys the desirable feature of \emph{linear speedup} with respect to the number of participating devices/institutions.

In this work, we establish solid theoretical foundations for federated
learning and demonstrate that linear speedup is possible in a variety of settings with the FedAvg algorithm and its variants, under both data and system heterogeneity, significantly improving previous understanding of federated learning.

We therefore show that federated learning is able to achieve efficiency and privacy at the same time. On one hand, data is isolated in each local device/institution, preventing
the potential leakage of private information. On the other hand, joint learning can speed up substantially if the number of
participating devices/institutions increases. In conclusion, our work shows a promising machine learning pathway to simultaneously securing people's privacy and improving
their lives.





==> sec_intro_old.tex <==
% !TEX ROOT=./main.tex


\section{Introduction and Related Works}


\begin{table}[h!]
	\centering
	\small
	\begin{tabular}{|c|c|c|c|c|}\hline
		paper         &  Cvx Non-smth & Cvx L-smth & Strongly Cvx Non-smth& Strongly Cvx L-smth \\ \hline
		Accelerated	SGD   &   $\cO(\frac{1}{\sqrt{T}})$     & $\cO(\frac{1}{\sqrt{KT}})$   &    $\cO(\frac{1}{T})$   &  $\cO(\frac{1}{KT}+\frac{E^2}{T^2})$    \\\hline
		SGD    &    $\cO(\frac{1}{\sqrt{T}})$  &   $\cO(\frac{1}{\sqrt{KT}})$  &  $\cO(\frac{1}{T})$  & $\cO(\frac{1}{T})$\cite{li2019convergence,haddadpour2019convergence}, $\cO(\frac{1}{KT}+\frac{E^2}{T^2})$ ours    \\\hline
	\end{tabular}
	\caption{Summary of related work on federated learning, heterogeneous data.}
\end{table}

+ exponential acceleration of MaSS for linear regression: for $E=1$, 
\begin{align*}
\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq C\cdot\exp(-\frac{t}{\sqrt{(\kappa_{N})(\tilde{\kappa}_{N})}})\leq C\cdot\exp(-\frac{Nt}{\sqrt{(\kappa_{1})(\tilde{\kappa})}})
\end{align*}

Most recent result by Koloskova et. al gives same bounds for convex and strongly convex.   



==> sec_nagcvxnonsmth.tex <==
% !TEX ROOT=./main.tex

In this section, we study the convergence of accelerated FedAvg 
algorithm for convex, non-smooth function.

\textbf{NASGD updates}
\begin{align}
	\vy^k_{t+1} &= \vw^k_{t} - \alpha  \vg_{t,k}	\\
	\vw^k_{t+1} & = \vy^k_{t+1} + \beta(\vy^k_{t+1} - \vy^k_{t})
\end{align}
% $$ \vv_{t+1}^{k} =  \vy^k_{t+1} + \beta(\vy^k_{t+1} - \vy^k_{t}) $$
% \begin{align} 
% \mathbf{w}_{t+1}^{k} &=\left\{\begin{array}{ll}\mathbf{v}_{t+1}^{k} & \text { if } t+1 \notin \mathcal{I}_{E}, \\ 
% \sum_{k \in \cS_{t+1}} \mathbf{v}_{t+1}^{k} & \text { if } t+1 \in \mathcal{I}_{E}\end{array}\right.
% \end{align}

\begin{theorem}
	Let Assumption~\ref{ass:subgrad2} hold, choose the learning rate $\eta = \frac{\alpha}{1 - \beta} = \sqrt{\frac{\Delta_0}{(D+C)T}}$, $\beta \in (0, 1)$ and $\beta \leq \min\{1, \frac{1}{1 + \sqrt{\frac{\Delta_0}{(D+C)T}}}\}$, then the FedNestrovAve with partial device participation satisfies
	\begin{align}
		 \EE F(\hat{\vw}_T) - F^* &\leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} 
	\end{align}
	where $\hat{\vw}_T = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $C$ is defined in \eq{\ref{eq:partialsample}},
$D$ is given by $D = (8 + 8(E-1)^2)G^2$.
	\label{th:nasgcvxnonsmoth}
\end{theorem}

\begin{proof}
We define $\vp_t$ and it satisfies the recursive equation:
\begin{align}
	\ov{p}_{t}=\left\{\begin{array}{ll}\frac{\beta}{1-\beta}\left[\ov{w}_{t}-\ov{w}_{t-1}+\alpha \vg_{t-1}\right], & t \geqslant 1 \\ 0, & t=0\end{array}\right.
\end{align}
\begin{align}
	\vp_{t+1} =  \beta \vp_t - \frac{\beta^2}{1 - \beta} \vg_t
	\label{eq:recursivep}
\end{align}
We define $\ov{z}_{t+1}$ as $\ov{z}_{t+1} = \ov{w}_{t+1} + \ov{p}_{t+1}$. 
\begin{align}
	% \underbrace{\overline{\vw}_{t+1} + \overline{\vp}_{t+1}}_{\overline{\vz}_{t+1}} &= \underbrace{\overline{\vw}_{t} + \overline{\vp}_{t}}_{\overline{\vz}_{t}} - \frac{\alpha}{1- \beta} \vg_t
	\overline{\vz}_{t+1} = \overline{\vz}_{t} - \frac{\alpha}{1- \beta} \vg_t
	\label{eq:nasgdzt}
\end{align}
With the recursive equation \eq{\ref{eq:nasgdzt}}, we have the following 
inequality.
\begin{align}
	\EE\|\overline{\vz}_{t+1} - \vw^* \|^2  &= \EE\|\overline{\vz}_{t} - \eta_t\vg_t - \vw^* \|^2 \\
& \leq  \| \overline{\vz}_{t} - \vw^*\|^2  - 2\eta_t\left<\EE\vg_t, \overline{\vz}_{t} - \vw^*\right> +  \eta_t^2\EE\|\vg_t\|^2 \\
& \leq  \| \overline{\vz}_{t} - \vw^*\|^2  - 2\eta_t\sum_{k=1}^K p_k\left<\EE g_{t,k}, \overline{\vz}_{t} - \vw^*\right> +  \eta_t^2\EE\|\vg_t\|^2 \label{eq:nagcvx1}
\end{align}

where we set $\eta_t = \frac{\alpha}{1- \beta}$. Follow the same reasoning 
in \eq{\ref{eq:4}}, use convexity of the objective function, we have 
\begin{align}
   & - \left<\EE g_{t,k}, \overline{\vz}_{t} - \vw^*\right> \\
	\leq & \frac{1}{2\eta_t} \|\overline{\vz}_t - \vw_t^k\|^2 + \frac{\eta_t}{2} \|\EE \vg_{t,k}\|^2 - (F_k(\vw_t^k) - F_k(\vw^*)) \label{eq:nagcvx2}
\end{align}
Plug in \eq{\ref{eq:nagcvx2}} to \eq{\ref{eq:nagcvx1}}:
\begin{align}
	\EE\|\overline{\vz}_{t+1} - \vw^* \|^2 & \leq \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2\EE\|\vg_t\|^2  \\
	&  + \sum_{k=1}^K p_k \underbrace{\|\overline{\vz}_t - \vw_t^k\|^2}_{A_1}  +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2 \underbrace{- 2\eta_t\sum_{k=1}^K p_k(F_k(\vw_t^k) - F_k(\vw^*))}_{A_2} \label{eq:nagcvx3}
\end{align}
Bound $A_2$, use the convexity of $F_k$, same reasoning as \eq{\ref{eq:a24}}:
\begin{align*}
& -2\eta_t\sum_{k=1}^K p_k (F_k(\vw_t^k) - F_k(\vw^*)) \\
\leq &\sum_{k=1}^K p_k (\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t) \|^2 +\|\vw_t^k - \overline{\vw}_t\|^2) -2\eta_t (F(\overline{w}_t) - F^*)
\end{align*}
Plug in the upper bound of $A_2$ into the \eq{\ref{eq:nagcvx3}}, 
\begin{align}
	\EE\|\overline{\vz}_{t+1} - \vw^* \|^2 & \leq \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2\EE\|\vg_t\|^2  \nonumber\\
	&  + \sum_{k=1}^K p_k \underbrace{\|\overline{\vz}_t - \vw_t^k\|^2}_{A_1}  +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2 \nonumber \\
	& + \sum_{k=1}^K p_k (\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 + \|\vw_t^k - \overline{\vw}_t\|^2) - 2\eta_t(F(\overline{w}_t) - F^*) 
	\label{eq:nagcvx4}
\end{align}
Bound $\EE\|\overline{\vz}_t - \vw_t^k\|^2$ and $\EE \|\overline{\vw}_t- \vw_t^k \|^2$, this is similar to the proof in Lemma 3~\cite{li2019convergence}: 

\begin{align}
	\EE \|\ov{\vw}_t -\vw_t^k \|^2 & = \EE \|\ov{w}_t - \ov{w}_{t_0} + \ov{w}_{t_0}- \vw_t^k \|^2\\
% & \leq \EE\|\ov{w}_{t_0}- \vw_t^k \|^2 + \EE \|\ov{w}_t - \ov{w}_{t_0}\|^2\\
& \leq \EE\|\vw_t^k  - \ov{w}_{t_0}\|^2  \\
& \leq \EE \|\vz_t^k - \vp_t^k  - \vz^k_{t_0} + \vp^k_{t_0}\|^2  \\
& \leq \EE \|\vz_t^k - \vz^k_{t_0}\|^2 + \EE\|\vp_t^k - \vp^k_{t_0}\|^2  \\
& = \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \EE\|\vp_t^k - \vp^k_{t_0}\|^2  \\
& = \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \frac{(\beta^{t-t_0}-1)^2\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2  \label{eq:nagcvx4-1}
\end{align}
where the second line is same from Lemma 3~\cite{li2019convergence}. $\ov{w}_{t_0} = \vw^k_{t_0}$ and $t_0$ is the step we communicate. In the third line, we use the \eq{\ref{eq:nasgdzt}}. In fourth line, we use \eq{\ref{eq:recursivep}}. 
The upper bound of $\EE\|\vp_t^k - \vp^k_{t_0}\|^2$ is given as follows:
\begin{align}
	\EE\|\vp_t^k - \vp^k_{t_0}\|^2 & = \EE\|\beta \vp^k_{t-1} - \frac{\beta^2}{1 - \beta} \vg_{t-1,k} - \vp^k_{t_0}\|^2\\
	&= \EE\|\beta^{t-t_0} \vp^k_{t_0} - \frac{\beta^2}{1 - \beta} \sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k} - \vp^k_{t_0}\|^2\\
	&= \EE\|(\beta^{t-t_0}-1) \vp^k_{t_0} - \frac{\beta^2}{1 - \beta} \sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2\\
	&= \EE\|(\beta^{t-t_0}-1) \vp^k_{t_0}\|^2 + \frac{\beta^2}{1 - \beta} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2\\
	&= (\beta^{t-t_0}-1)^2\EE\|\ov{p}_{t_0}\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2\\
	&= (\beta^{t-t_0}-1)^2\frac{\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2 \label{eq:nagcvx5}
\end{align}

\begin{align}
	\EE \|\overline{\vz}_t - \vw_t^k\|^2 & =  \EE \|\overline{\vw}_t + \overline{\vp}_{t}  - \vw_t^k\|^2\\ 
 & \leq  \EE \|\overline{\vw}_t -\vw_t^k \|^2 + \EE\| \overline{\vp}_{t}\|^2  \\
 &  =\EE \|\overline{\vw}_t -\vw_t^k \|^2 + \frac{\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 \label{eq:nagcvx6}
\end{align}
Plug in \eq{\ref{eq:nagcvx5}} and \eq{\ref{eq:nagcvx6}} into
\eq{\ref{eq:nagcvx4}}:
\begin{align}
	\EE\|\overline{\vz}_{t+1} - \vw^* \|^2 & \leq \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2\EE\|\vg_t\|^2  \nonumber\\
	&  + \sum_{k=1}^K p_k \|\overline{\vz}_t - \vw_t^k\|^2  +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2 \nonumber \\
	& + \sum_{k=1}^K p_k (\eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2 + \|\vw_t^k - \overline{\vw}_t\|^2) - 2\eta_t(F(\overline{w}_t) - F^*) \\
	& =  \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2\EE\|\vg_t\|^2 +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2  \nonumber\\
	& + \sum_{k=1}^K p_k \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2  - 2\eta_t(F(\overline{w}_t) - F^*) \nonumber \\
	&  + \sum_{k=1}^K p_k \|\ov{p}_t\|^2 + 2\sum_{k=1}^K p_k \|\ov{w}_t - \vw_t^k\|^2  \\
	& \leq \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2\EE\|\vg_t\|^2 +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2  \nonumber\\
	& + \sum_{k=1}^K p_k \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2  - 2\eta_t(F(\overline{w}_t) - F^*) \nonumber \\
	& + \sum_{k=1}^K p_k \left(\frac{\beta^4}{(1-\beta)^2}\EE\|\underline{\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j}\|^2 \right) \nonumber\\
	& + 2\sum_{k=1}^K p_k \left(\EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \frac{(\beta^{t-t_0}-1)^2\beta^4}{(1-\beta)^2}\EE\|\underline{\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j}\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2 \right) \\
	& \leq \| \overline{\vz}_{t} - \vw^*\|^2  - 2\eta_t(F(\overline{w}_t) - F^*)  \nonumber\\
	& +  \eta_t^2\EE\|\vg_t\|^2 +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2 + \sum_{k=1}^K p_k \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2  \nonumber \\
	& + \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{(1-\beta)^2} \EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 \nonumber\\
	& + 2\sum_{k=1}^K p_k \left(\EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2  + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2 \right) \label{eq:nagcvx7}
\end{align}

Denote the last three lines in \eq{\ref{eq:nagcvx7}} as $C$: 
\begin{align}
C &= \eta_t^2\EE\|\vg_t\|^2 +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2+ \sum_{k=1}^K p_k \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2  \nonumber \\
% 2\sum_{k=1}^K p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 
	& +  \left(\underbrace{\frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{(1-\beta)^2} \EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2}_{C_1} \right) \nonumber\\
	& + 2\sum_{k=1}^K p_k \left(\underbrace{\EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 }_{C_2} + \underbrace{\frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2}_{C_3} \right)  \label{eq:nagcvxc}
\end{align}



We now bound $C_1$, we set $\Lambda_{t_0} = \sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j} = \frac{1 - \beta^{t_0}}{1- \beta} \leq \frac{1}{1 - \beta}$, \lkxcom{assume $\beta \in (0, 1)$ and set $\alpha \geq \beta$}.
\begin{align}
	C_1 &=  \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{(1-\beta)^2} \EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2\\
        &= \eta_t^2 \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\alpha^2} \EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2\\
        &= \eta_t^2  \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\alpha^2}\Lambda_{t_0}^2 \EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}/\Lambda_{t_0} \vg_j\|^2\\
        & \leq \eta_t^2  \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\alpha^2}\Lambda_{t_0}^2 \sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}/\Lambda_{t_0}\EE\| \vg_j\|^2\\ 
        & = \eta_t^2 \Lambda_{t_0} \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\alpha^2} \sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j} \EE\| \vg_j\|^2\\
		& \leq  \eta_t^2 \Lambda_{t_0} \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\alpha^2} \sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j} \sum_{k=1}^N p_k G_k^2   \\
		& =  \eta_t^2 \Lambda_{t_0} \frac{\beta^4(2(\beta^{t-t_0}-1)^2 + 1)}{\beta^2} \Lambda_{t_0}  \sum_{k=1}^N p_k G_k^2  \\
		& \leq  \eta_t^2 \frac{1}{(1-\beta)^2} \frac{\beta^2(2 \times 1 + 1)}{1} \sum_{k=1}^N p_k G_k^2   \\
		& \leq  3 \eta_t^4\sum_{k=1}^N p_k G_k^2   \label{eq:nagcvxc1}
\end{align}
In the fourth line we use the Jensen's inequality. In the fifth line, we use the assumption~\ref{ass:subgrad2}. 


To bound $C_2$, we assume $\eta_t$ is non-increasing and $\eta_t  \leq \eta_{t_0}  \leq 2 \eta_t$
\begin{align}
 C_2 = & 2\sum_{k=1}^K p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2\\
 \leq& 2\sum_{k=1}^K p_k \eta_{t_0}^2 \EE \|\sum_{j=t_0}^{t-1} \vg_{j,k}\|^2
 \leq 2\sum_{k=1}^K p_k  (E-1)\sum_{j=t_0}^{t-1}\eta_{j}^2 \EE \| \vg_{j,k}\|^2\\
 \leq & 2\sum_{k=1}^K p_k  (E-1)\eta_{t_0}^2 \sum_{j=t_0}^{t-1} \EE \| \vg_{j,k}\|^2\\
 \leq & 2\sum_{k=1}^K p_k  (E-1)4\eta_{t}^2 \sum_{j=t_0}^{t-1} \EE \| \vg_{j,k}\|^2 \leq 8(E-1)\eta_{t}^2 \sum_{k=1}^K p_k \sum_{j=t_0}^{t-1} \EE \| \vg_{j,k}\|^2 \\
 \leq & 8(E-1)\eta_{t}^2 \sum_{k=1}^K p_k (E-1)G_k^2 \\
 =  & 8(E-1)^2\eta_{t}^2 \sum_{k=1}^K p_k G_k^2   \label{eq:nagcvxc2}
\end{align}
To bound $C_3$, similar to $C_1$, we set $\Lambda_{t_0}^{t} = \sum_{j=t_0}^{t - 1}\beta^{t_0-1-j} =  \frac{1 - \beta^{t-t_0}}{1- \beta} \leq \frac{1}{1 - \beta} $
\begin{align}
	C_3 & = 2\sum_{k=1}^K p_k \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2\\
        & = 2\eta_t^2 \Lambda_{t_0}^{t}\sum_{k=1}^K p_k \frac{\beta^4}{\alpha^2} \sum_{j=t_0}^{t-1}\beta^{t-j-1} \EE\|\vg_{j,k}\|^2 \\
        & \leq 2 \eta_t^4 \sum_{k=1}^K p_k G_k^2  \label{eq:nagcvxc3}
\end{align}

Based on \eq{\ref{eq:nagcvxc}}, \eq{\ref{eq:nagcvxc1}}, \eq{\ref{eq:nagcvxc2}}, and \eq{\ref{eq:nagcvxc3}}, we can denote $C \leq \eta_t^2 D$.
\begin{align}
	C \leq& \eta_t^2\EE\|\vg_t\|^2 +\eta^2_t \sum_{k=1}^K p_k\|\EE \vg_{t,k}\|^2+ \sum_{k=1}^K p_k \eta_t^2 \|\EE \vg_{t,k}(\overline{\vw}_t)\|^2  \nonumber \\
	& + \underbrace{3 \eta_t^4\sum_{k=1}^N p_k G_k^2}_{C_1\text{'s upper bound}} + \underbrace{8(E-1)^2\eta_{t}^2 \sum_{k=1}^K p_k G_k^2}_{C_2\text{'s upper bound}} + \underbrace{2 \eta_t^4 \sum_{k=1}^K p_k G_k^2 }_{C_1\text{'s upper bound}} \\
	  \leq & \eta_t^2 \left(3 + 8(E-1)^2\right)\sum_{k=1}^N p_k G_k^2   + \eta_t^4 \times 5 \sum_{k=1}^N p_k G_k^2 \\
	  \leq & \eta_t^2 \underbrace{\left(3 + 8(E-1)^2\right)G^2}_{D_1}   + \eta_t^4 \times \underbrace{5 G^2}_{D_2} \\
	  = &  \eta_t^2 D_1 + \eta_t^4 D_2 
\end{align}

We plug in $C$ back to \eq{\ref{eq:nagcvx7}} and set $D=D_1 + D_2 = D = (8 + 8(E-1)^2)G^2$, we have 
\begin{align}
\EE\|\overline{\vz}_{t+1} - \vw^* \|^2 & \leq \EE \| \overline{\vz}_{t} - \vw^*\|^2  +  \eta_t^2 D   - 2\eta_t(F(\overline{w}_t) - F^*) \nonumber\\	
 2\eta_t(F(\overline{w}_t) - F^*) & \leq  \Delta_{t}  - \Delta_{t+1}  +  \eta_t^2 D    \nonumber
\end{align}

Sum two sides over time step $t$, take totoal expectation and use constant rate $\eta_t = \eta$:
\begin{align}
\EE \frac{1}{T}\sum_{t=0}^{T-1} 2 \eta (F(\overline{w}_t) - F^*) & \leq \Delta_0 - \Delta_{T} + \sum_{t=0}^{T-1} (\eta^2 D_1 + \eta^4 D_2) \nonumber\\
\EE \frac{1}{T}\sum_{t=0}^{T-1} 2 \eta (F(\overline{w}_t) - F^*) & \leq \Delta_0/T  + \sum_{t=0}^{T-1} (\eta^2 D_1 + \eta^4 D_2)\nonumber\\
 \EE F(\hat{w}_t) - F^* & \leq \frac{\Delta_0}{2T\eta}   + \frac{\eta D_1}{2} + \frac{\eta^3 D_1}{2}\nonumber\\
 \EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0D}{4T}} + \sqrt{\frac{\Delta_0}{DT}}\frac{ D_1}{2} + (\frac{\Delta_0}{DT})^{3/2}\frac{ D_2}{2} \nonumber\\
 \EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0D}{4T}} + \sqrt{\frac{\Delta_0}{DT}}\frac{ D}{2} + (\frac{\Delta_0}{DT})^{3/2}\frac{ D}{2} \nonumber\\
 \EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0D}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D}}\frac{1}{T^{3/2}} \label{eq:nagcvxc4}\\
\end{align}
where $\hat{w}_t = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $\eta = \sqrt{\frac{\Delta_0}{DT}}$.


In partial participation, we define vitural sequence $ \ov{v}_{t+1} = \ov{z}_{t} - \eta_t \vg_t$.
\begin{align}
\ov{v}_{t+1} =  \left\{\begin{array}{ll}
    \ov{z}_{t+1},  & t + 1 \notin \cI_{E}\\
	\EE_{S_{t+1}} \ov{z}_{t+1}, &  t + 1 \in \cI_{E}
\end{array} \right.
\end{align}
\begin{align}
  & \EE\|\ov{z}_{t+1} - \vw^* \|^2  \\
=&  \EE\|\ov{z}_{t+1} - \ov{v}_{t+1} + \ov{v}_{t+1} -  \vw^* \|^2 	\\
=&  \EE\|\ov{z}_{t+1} - \ov{v}_{t+1}\|^2  + \EE\|\ov{v}_{t+1} -  \vw^* \|^2 - 2 \left<\underbrace{\EE \ov{z}_{t+1} - \ov{v}_{t+1}}_{= 0}, \ov{v}_{t+1} -  \vw^*\right> 	 \\
=&  \EE\|\ov{z}_{t+1} - \ov{v}_{t+1}\|^2  + \EE\|\ov{v}_{t+1} -  \vw^* \|^2 \\
\leq& \eta_t^2 C	 + \EE\|\ov{v}_{t+1} -  \vw^* \|^2 \\
 = & \eta_t^2 C	 + \EE\|\overline{\vz}_{t} - \eta_t\vg_t - \vw^* \|^2  \\
\leq& \EE\|\ov{z}_{t} - \vw^* \|^2 +  \eta_t^2 C +  \eta_t^2 D   - 2\eta_t(F(\overline{w}_t) - F^*)
\end{align} 
Follow the same derivation in full participation case, choose $\eta = \sqrt{\frac{\Delta_0}{(D+C)T}}$, we have
\begin{align*}
	 \EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} \nonumber\\
\end{align*}

\end{proof}


% \begin{itemize}
% 	\item Update NASG or MSG.
% 	\item Store the momentum every $E$~\cite{huo2020faster} , every step~\cite{liu2019accelerating}, rely on L-smoothness.
% \end{itemize}
% \begin{itemize}
% 	\item MGD vs NASGD: currently we use NASGD. 
% 	\begin{align}
% 	\vy^k_{t+1} &= \gamma \vy^k_t + \grad F_k(\vw^k_{t})	\\
% 	\vw^k_{t+1} & = \vw^k_{t} - \eta \vy^k_{t+1}
% 	\end{align}
% 	\begin{align}
% 	\vy^k_{t+1} &= \vw^k_{t} - \alpha \grad F_k(\vw^k_{t})	\\
% 	\vw^k_{t+1} & = \vy^k_{t+1} + \beta(\vy^k_{t+1} - \vy^k_{t})
% 	\end{align}
% \end{itemize}


==> sec_nasgd_cvx_smth.tex <==
% !TEX ROOT=./main.tex


\begin{theorem}
	Let Assumption~\ref{ass:lsmooth} and Assumption~\ref{ass:subgrad2} hold,  choose the learning rate $\eta = \frac{\alpha}{1 - \beta} = \sqrt{\frac{\Delta_0}{(D+C)T}}$, $\beta \in (0, 1)$ and $\beta \leq \min\{1, \frac{1}{1 + \sqrt{\frac{\Delta_0}{(D+C)T}}}\}$, then the FedNestrovAve with partial device participation satisfies
	\begin{align}
		 \EE F(\hat{\vw}_T) - F^* &\leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} 
	\end{align}
	where $\hat{\vw}_T = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $C$ is defined in \eq{\ref{eq:partialsample}},
$D$ is given by $D =  G^2[6 + (4(E-1)^2+1)L]$.
\end{theorem}

\begin{proof}
Follow the same derivation in \eq{\ref{eq:nagcvx1}}, we have the follow inequality.
\begin{align}
		\EE\|\overline{\vz}_{t+1} - \vw^* \|^2  & \leq  \| \overline{\vz}_{t} - \vw^*\|^2  - 2\eta_t\sum_{k=1}^K p_k\left<\EE g_{t,k}, \overline{\vz}_{t} - \vw^*\right> +  \eta_t^2\EE\|\vg_t\|^2 \label{eq:nasgdcvxsm0}
\end{align}

Bound $- 2\eta_t\sum_{k=1}^K p_k\left<\EE g_{t,k}, \overline{\vz}_{t} - \vw^*\right>$, 
\begin{align}
	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}-\vw^{*}\right> \nonumber \\
 =  & -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}- \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t}, \vw^{k}_t - \vw^{*}\right>\nonumber \\
 \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}- \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\nonumber \\
 \leq &\sum_{k=1}^N p_k \left[2 \eta_{t} (F_k(\vw^{k}_t) - F_k(\ov{z}_t) + \frac{L}{2} \|\ov{z}_t - \vw^{k}_t\|^2 ) + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\right]\nonumber \\
 = & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{z}_t)) 
  \label{eq:nasgdcvxsm1}\\
  = & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t) +  F_k(\ov{w}_t) -  F_k(\ov{z}_t)) \\
  = & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) +  2 \eta_{t} \sum_{k=1}^N p_k  (F_k(\ov{w}_t) -  F_k(\ov{z}_t)) \label{eq:nasgdcvxsm1}
\end{align}

Now we bound $2 \eta_{t} \sum_{k=1}^N p_k  (F_k(\ov{w}_t) -  F_k(\ov{z}_t)) $

\begin{align}
	 & 2 \eta_{t} \sum_{k=1}^N p_k  (F_k(\ov{w}_t) -  F_k(\ov{z}_t))  \\
\leq & 2 \eta_{t} \sum_{k=1}^N p_k  (\left<\vg_{t,k}(\ov{z}_t), \ov{w}_t - \ov{z}_t\right> + \frac{L}{2}\|\ov{w}_t - \ov{z}_t\|^2)\\
\leq & 2 \eta_{t} \sum_{k=1}^N p_k (\frac{\eta_t}{2}\|\vg_{t,k}(\ov{z}_t)\|^2 + \frac{1}{2\eta_t}\|\ov{w}_t - \ov{z}_t\|^2+ \frac{L}{2}\|\ov{w}_t - \ov{z}_t\|^2)\\
\leq & \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + (1+ \eta_t L)\|\ov{w}_t - \ov{z}_t\|^2 \label{eq:nasgdcvxsm2}
\end{align}
Plug in \eq{\ref{eq:nasgdcvxsm2}} to \eq{\ref{eq:nasgdcvxsm1}}, 

\begin{align}
	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}-\vw^{*}\right> \nonumber \\
\leq & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \nonumber \\
 & +  2 \eta_{t} \sum_{k=1}^N p_k  (F_k(\ov{w}_t) -  F_k(\ov{z}_t)) \\
\leq & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \nonumber \\
  & +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + (1+ \eta_t L)\|\ov{w}_t - \ov{z}_t\|^2 \label{eq:nasgdcvxsm3}
\end{align}

Now we can bound $\|\ov{w}_t - \ov{z}_t\|^2 = \| \ov{p}_t\|^2$ follow the \eq{\ref{eq:nagcvx6}}: 
\begin{align}
	\EE \|\ov{w}_t - \ov{z}_t\|^2 \leq \frac{\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 
	\label{eq:nasgdcvxsm4}
\end{align}

Follow the proof in \eq{\ref{eq:nagcvx4-1}}, we can bound $\|\ov{w}_t - \vw^{k}_t\|^2$ as follows:
\begin{align}
	\EE \|\ov{w}_t - \vw^{k}_t\|^2  \leq \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \frac{(\beta^{t-t_0}-1)^2\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2 \label{eq:nasgdcvxsm5}
\end{align}

Plug in \eq{\ref{eq:nasgdcvxsm4}}, \eq{\ref{eq:nasgdcvxsm5}}, and \eq{\ref{eq:nasgdcvxsm3}} to \eq{\ref{eq:nasgdcvxsm0}}: 
\begin{align}
		\EE\|\overline{\vz}_{t+1} - \vw^* \|^2  & \leq  \| \overline{\vz}_{t} - \vw^*\|^2 +  \eta_t^2\EE\|\vg_t\|^2  \\
 & + \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2  + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \nonumber \\
  & +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + (1+ \eta_t L)\|\ov{w}_t - \ov{z}_t\|^2 \\
 & \leq  \| \overline{\vz}_{t} - \vw^*\|^2 +  \eta_t^2\EE\|\vg_t\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \\
 & +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2  	  \nonumber \\
  & + \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2    + (1+ \eta_t L)\|\ov{w}_t - \ov{z}_t\|^2 \\
& \leq  \| \overline{\vz}_{t} - \vw^*\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \\
 & + \eta_t^2\EE\|\vg_t\|^2  +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2  	  \nonumber \\
  & + \eta_t L \sum_{k=1}^N p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \frac{(\beta^{t-t_0}-1)^2\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 + \frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2   \\
  &   + (1+ \eta_t L)\frac{\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2  \label{eq:nasgdcvxsm6}
\end{align}
Denote last three lines in \eq{\ref{eq:nasgdcvxsm6}} as $C_1$, we now give upper bound of $C_1$
\begin{align*}
C_1 &= 	\eta_t^2\EE\|\vg_t\|^2  +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2  	  \nonumber \\
  &  + \eta_t L \sum_{k=1}^N p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2 + \frac{(\beta^{t-t_0}-1)^2\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 + \sum_{k=1}^N p_k\frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2   \\
  & + (1+ \eta_t L)\frac{\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2 \\
  & = \underbrace{\eta_t^2\EE\|\vg_t\|^2  +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2}_{C_2} + \underbrace{\eta_t L \sum_{k=1}^N p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2}_{C_3}   \nonumber \\
  & + \underbrace{\frac{[1+ \eta_t L + (\beta^{t-t_0}-1)^2]\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2}_{C_4} + \underbrace{\sum_{k=1}^N p_k\frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2}_{C_5}   \label{eq:nasgdcvxsm7}
\end{align*}

With Assumption~\ref{ass:subgrad2}, the upper bound of first line is given by:
\begin{align*}
		C_2 = \eta_t^2\EE\|\vg_t\|^2  +  \sum_{k=1}^N p_k \eta_t^2\|\vg_{t,k}(\ov{z}_t)\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2  	  \leq 3 \eta_t^2 G^2
\end{align*}
\begin{align*}
C_3 =	& \eta_t L \sum_{k=1}^N p_k \EE \|\sum_{j=t_0}^{t-1}\eta_j \vg_{j,k}\|^2  \leq \eta_t L (4 (E-1)^2\eta_t^2 G^2) = 4(E-1)^2\eta_t^3L G^2 
\end{align*}
\begin{align*}
C_4 = 	\frac{[1+ \eta_t L + (\beta^{t-t_0}-1)^2]\beta^4}{(1-\beta)^2}\EE\|\sum_{j=0}^{t_0 - 1}\beta^{t_0-1-j}\vg_j\|^2  \leq \eta_t^4(2 + L) G^2 
\end{align*}
\begin{align*}
	C_5 = \sum_{k=1}^N p_k\frac{\beta^4}{(1 - \beta)^2} \EE\|\sum_{j=t_0}^{t-1}\beta^{t-j-1}\vg_{j,k}\|^2 
	\leq \eta_t^4 G^2
\end{align*}

Plug in $C_2 - C_5$ into \eq{\ref{eq:nasgdcvxsm6}}, 

\begin{align}
	\EE\|\overline{\vz}_{t+1} - \vw^* \|^2 & \leq  \| \overline{\vz}_{t} - \vw^*\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t))  + 3\eta_t G^2 + 4(E-1)^2\eta_t^3L G^2  +  \eta_t^4(2 + L) G^2  + \eta_t^4 G^2 \\
& \leq  \| \overline{\vz}_{t} - \vw^*\|^2 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t))  + \eta_t^2 \underbrace{G^2[6 + (4(E-1)^2+1)L] }_{D}
\end{align}
Sum two sides over time step $t$, take totoal expectation and use constant rate $\eta_t = \eta$ and follow \eq{\ref{eq:nagcvxc4}}:
\begin{align}
	\EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0D}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D}}\frac{1}{T^{3/2}} \nonumber\\
\end{align}
where $D = G^2[6 + (4(E-1)^2+1)L] $, $\hat{w}_t = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $\eta = \sqrt{\frac{\Delta_0}{DT}}$.

\textbf{Consider partial device participation:}
\begin{align*}
	 \EE F(\hat{w}_t) - F^* & \leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} \nonumber\\
\end{align*}
where $\eta = \sqrt{\frac{\Delta_0}{(D+C)T}}$. 
\end{proof}

% Approach 1. 
% \begin{align}
% 	& -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}-\vw^{*}\right> \nonumber \\
%  =  & -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}- \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t}, \vw^{k}_t - \vw^{*}\right>\nonumber \\
%  \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{z}_{t}- \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\nonumber \\
%  \leq & -2 \eta_{t} \left<\EE \vg_{t}, \ov{w}_{t} - \vw^{k}_t \right> -2 \eta_{t} \left<\EE \vg_{t},  \ov{p}_{t} - \vw^{k}_t \right> + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\nonumber \\
%  \leq &\sum_{k=1}^N p_k \left[2 \eta_{t} (F_k(\vw^{k}_t) - F_k(\ov{w}_t) + \frac{L}{2} \|\ov{w}_t - \vw^{k}_t\|^2 ) + \|\ov{p}_t - \vw_t^k\|^2 + \eta_t^2 \|\EE \vg_{t,k}\|^2  + 2 \eta_{t} (F_k(w^*) - F_k(\vw^{k}_t))\right]\nonumber \\
%  = & \eta_t L \sum_{k=1}^N p_k  \|\ov{w}_t - \vw^{k}_t\|^2 + \sum_{k=1}^N p_k \|\ov{p}_t - \vw_t^k\|^2 + \sum_{k=1}^N p_k\eta_t^2 \|\EE \vg_{t,k}\|^2 	 + 2 \eta_{t} \sum_{k=1}^N p_k (F_k(w^*) - F_k(\ov{w}_t)) \label{eq:nasgdcvxsm1}
% \end{align}

==> sec_nasgd_scvx_nonsmooth.tex <==
We show that FedAvg with Accelerated SGD has $O(1/T)$ rate under
$\mu$-strong convexity. The FedAv algorithm with Nesterov Accelerated
SGD (NASGD) follows the updates
\begin{align*}
y_{t+1}^{k} & =w_{t}^{k}-\alpha_{t}g_{t,k}\\
w_{t+1}^{k} & =\begin{cases}
y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}) & \text{if }t+1\notin\mathcal{I}_{E}\\
\sum_{k=1}^{N}p_{k}\left[y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})\right] & \text{if }t+1\in\mathcal{I}_{E}
\end{cases}
\end{align*}
where 
\begin{align*}
g_{t,k} & :=\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})
\end{align*}
is the stochastic gradient. 

Define the virtual sequences $\overline{y}_{t}=\sum_{k=1}^{N}p_{k}y_{t}^{k}$,
$\overline{w}_{t}=\sum_{k=1}^{N}p_{k}w_{t}^{k}$, and $\overline{g}_{t}=\sum_{k=1}^{N}p_{k}\mathbb{E}g_{t,k}$.
We have $\mathbb{E}g_{t}=\overline{g}_{t}$ and $\overline{y}_{t+1}=\overline{w}_{t}-\alpha_{t}g_{t}$,
and $\overline{w}_{t+1}=\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})$. 
\begin{remark}
	The difference between the smooth and non-smooth cases under strong
	convexity lies in the following key properties: with $L$-smoothness,
	we have
	\begin{align*}
	F(w)-F^{\ast} & \leq\frac{L}{2}\|w-w^{\ast}\|^{2}
	\end{align*}
	so that we may show the decay of optimality gap by the convergence
	of parameters. This is not available in the non-smooth case, and in
	order to apply the decay result of $\|\overline{w}_{t}-w^{\ast}\|^{2}$,
	we need to make use of the averaging trick found for example in CITE.
	The more important difference is that the lower bound $\|\nabla F(w)\|^{2}\leq2L(F(w)-F^{\ast})$
	under $L$-smoothness allows us to bound the terms $\|\nabla F_{k}(\overline{w}_{t})\|\leq2L(F_{k}(\overline{w}_{t}))$
	which combined with convexity gives an upper bound on $-2\alpha_{t}\sum_{k=1}^{N}(F_{k}(w_{t}^{k})-F^{\ast})$,
	acrucial quantity in the proof under strong convexity, and this allows
	us to separate out the heterogeneity term $\Gamma$. When we do not
	have $L$-smoothness, in order to upper bound $-2\alpha_{t}\sum_{k=1}^{N}(F_{k}(w_{t}^{k})-F^{\ast})$,
	we must resort to bounding $\mathbb{E}(\|\nabla F_{k}(\overline{w}_{t})\|^{2})$,
	which is different from the assumption $\mathbb{E}(\|g_{t,k}\|^{2})=\mathbb{E}(\|\nabla F_{k}(w_{t}^{k})\|^{2})\leq G^{2}$,
	and requires a possibly stronger assumption. A different approach
	is the following 
	\begin{align*}
	-2\alpha_{t}\sum_{k=1}^{N}(F_{k}(w_{t}^{k})-F^{\ast}) & =-2\alpha_{t}\sum_{k=1}^{N}(F_{k}(w_{t}^{k})-F_{k}^{\ast}+F_{k}^{\ast}-F^{\ast})\\
	& =-2\alpha_{t}\sum_{k=1}^{N}(F_{k}(w_{t}^{k})-F_{k}^{\ast})+2\alpha_{t}\Gamma\\
	& \leq\sum_{k=1}^{N}p_{k}\alpha_{t}^{2}\|\nabla F_{k}(w_{t}^{k})\|^{2}+\|w_{t}^{k}-w^{k,\ast}\|^{2}+2\alpha_{t}\Gamma
	\end{align*}
	and resort to bounding $\mathbb{E}\|w_{t}^{k}-w^{k,\ast}\|^{2}$.
	The problem is that $2\alpha_{t}\Gamma$ is not $O(\alpha_{t}^{2})$,
	and it is unclear how to show $\|w_{t}^{k}-w^{k,\ast}\|^{2}$ converges. 
\end{remark}
\begin{theorem}
	(Full device participation) Suppose $F_{k}$ is $\mu$-strongly convex
	for all $k$. Let $E$ be the communication interval, and learning
	rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(E+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $c$ is small enough
	such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|\nabla F_{k}(w,\xi_{t}^{k})\|^{2}\leq G^{2}$
	for $w=\overline{w}_{t}$ or $w=w_{t}^{k}$ and all $t,k$.
	
	Then with full device participation, \textbf{
		\begin{align*}
		F(\sum_{t=1}^{T}\frac{2t}{T(T+1)}\overline{w}_{t})-F^{\ast} & \leq\frac{2B'}{\mu(T+1)}
		\end{align*}
	} where
	\begin{align*}
	B' & =6G^{2}+32(E-1)^{2}G^{2}+2K^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =6G^{2}+32(E-1)^{2}G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}
\begin{proof}
	The bounds 
	\begin{align*}
	\mathbb{E}\|y_{t}^{k}-y_{t-1}^{k}\|^{2} & \leq G^{2}\\
	\mathbb{E}\|\overline{y}_{t}-\overline{y}_{t-1}\|^{2} & \leq G^{2}
	\end{align*}
	hold as before. However, we no longer have the upper bound
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & =\mathbb{E}(F(\overline{w}_{t})-F(w^{\ast}))\\
	& \leq\frac{L}{2}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}
	\end{align*}
	
	Fortunately we can still use an averaging trick to convert the decay
	of $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}$ into that of $\mathbb{E}(F(\overline{w}_{t}))-F^{\ast}$,
	but this time replacing $\overline{w}_{t}$ with the time-averaged
	version $\sum_{t=1}^{T}\frac{2t}{T(T+1)}\overline{w}_{t}$.
	
	Our main step is to prove the bound 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'
	\end{align*}
	where $B'$ is define in the statement of the theorem. We have 
	\begin{align*}
	\|\overline{w}_{t+1}-w^{\ast}\|^{2} & =\|\overline{w}_{t}-w^{\ast}-\alpha_{t}g_{t}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}\\
	& =\|\overline{w}_{t}-w^{\ast}\|^{2}+2\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}g_{t}\rangle+\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}g_{t}\|^{2}\\
	& \leq\|\overline{w}_{t}-w^{\ast}\|^{2}+2\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}g_{t}\rangle+2\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}+2\|\alpha_{t}g_{t}\|^{2}
	\end{align*}
	and the last two terms satisfy 
	\begin{align*}
	\mathbb{E}\left(2\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}+2\|\alpha_{t}g_{t}\|^{2}\right) & \leq4\alpha_{t}^{2}G^{2}
	\end{align*}
	sicne $\beta_{t}\leq\alpha_{t}$, $\|(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}\leq G^{2}$,
	and $\mathbb{E}\|g_{t}\|^{2}=\mathbb{E}\|\sum_{k=1}^{N}p_{k}g_{t,k}\|^{2}\leq\mathbb{E}\sum_{k=1}^{N}p_{k}\|g_{t,k}\|^{2}\leq G^{2}$. 
	
	Now 
	\begin{align*}
	2\mathbb{E}\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}g_{t}\rangle & =2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle-2\alpha_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle
	\end{align*}
	and we first bound $-2\alpha_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle$.
	We have
	\begin{align*}
	-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle & =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w^{\ast},g_{t,k}\rangle\\
	& =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w_{t}^{k},g_{t,k}\rangle-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle w_{t}^{k}-w^{\ast},g_{t,k}\rangle
	\end{align*}
	and again we bound the two terms separately. Using $\|\frac{1}{\sqrt{\alpha_{t}}}(\overline{w}_{t}-w_{t}^{k})-\sqrt{\alpha_{t}}g_{t,k}\|^{2}\geq0$,
	we have
	\begin{align*}
	-2\langle\overline{w}_{t}-w_{t}^{k},g_{t,k}\rangle & \leq\frac{1}{\alpha_{t}}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}\|g_{t,k}\|^{2}
	\end{align*}
	
	Letting $\mathbb{E}_{t}$ denote the conditional expectation $\mathbb{E}\left[\cdot\mid\{w_{t}^{k}\}_{k=1}^{N}\right]$,
	i.e. the expectation with respect to the randomness of $\xi_{t}^{k}$s
	in the stochastic gradients, the $\mu$-strong convexity of $F_{k}$
	implies 
	\begin{align*}
	-\mathbb{E}_{t}\langle w_{t}^{k}-w^{\ast},g_{t,k}\rangle & =-\mathbb{E}_{t}\langle w_{t}^{k}-w^{\ast},g_{t}\rangle=-\mathbb{E}_{t}\langle w_{t}^{k}-w^{\ast},\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})\rangle=-\langle w_{t}^{k}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle\\
	& \leq-(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))-\frac{\mu}{2}\|w_{t}^{k}-w^{\ast}\|^{2}
	\end{align*}
	
	Combining the above, it follows that 
	\begin{align*}
	-2\alpha_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle & \le\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}\left[(\frac{1}{\alpha_{t}}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}\|g_{t,k}\|^{2})-2(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))-\mu\|w_{t}^{k}-w^{\ast}\|^{2}\right]\\
	& =\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}-\mu\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w^{\ast}\|^{2}+\alpha_{t}^{2}\mathbb{E}\sum_{k=1}^{N}p_{k}\|g_{t,k}\|^{2}\\
	& -2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))\\
	& \leq\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}-\mu\alpha_{t}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}G^{2}-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))
	\end{align*}
	where we have again used Jensen's inequality on $\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w^{\ast}\|^{2}$. 
	
	Thus 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{k}^{t}\|^{2}-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))\\
	& +5\alpha_{t}^{2}G^{2}+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle
	\end{align*}
	We note that 
	\begin{align*}
	\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{k}^{t}\|^{2} & \leq16(E-1)^{2}\alpha_{t}^{2}G^{2}
	\end{align*}
	by the same argument as in the proof for the strongly convex and
	smooth case. Now we bound 
	\begin{align*}
	-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast})) & \leq-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))\\
	& =-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(\overline{w}_{t})+F(\overline{w}_{t})-F_{k}(w^{\ast}))\\
	& \leq-2\alpha_{t}\mathbb{E}\sum_{k=1}^{N}p_{k}(\langle w_{t}^{k}-\overline{w}_{t},\nabla F_{k}(\overline{w}_{t})\rangle+F(\overline{w}_{t})-F_{k}(w^{\ast}))\\
	& \leq\mathbb{E}\sum_{k=1}^{N}p_{k}\left[\alpha_{t}^{2}\|\nabla F_{k}(\overline{w}_{t})\|^{2}+\|w_{t}^{k}-\overline{w}_{t}^{k}\|^{2}\right]-2\alpha_{t}(F(\overline{w}_{t})-F^{\ast})\\
	& \leq\alpha_{t}^{2}G^{2}+\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{k}^{t}\|^{2}-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})
	\end{align*}
	using convexity of $F_{k}$, the assumption that $\mathbb{E}\|\nabla F_{k}(\overline{w}_{t})\|^{2}\leq G^{2}$.
	This is where the proof differs from the smooth case, where we bounded
	$\|\nabla F_{k}(\overline{w}_{t})\|^{2}\leq2L(F(\overline{w}_{t})-F^{\ast})$. 
	
	Thus 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+2\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{k}^{t}\|^{2}-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})\\
	& +6\alpha_{t}^{2}G^{2}+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle\\
	& \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle
	\end{align*}
	where 
	\begin{align*}
	B & =6G^{2}+32(E-1)^{2}G^{2}
	\end{align*}
	
	Now we bound $|2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle|$.
	As in the proof for the strongly convex and smooth case, with appropriate
	choice of constant $K$ depending on the other constants, we first
	show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq K^{2}
	\end{align*}
	for all $t$, i.e. the updates always stay in a large ball around
	the optimum during the Nesterov accelerated gradient descent. Note
	that $(F(\overline{w}_{t})-F^{\ast})\geq0$ and 
	\begin{align*}
	\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle & \leq\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot\sqrt{\mathbb{E}\|\overline{y}_{t+1}-\overline{y}_{t}\|^{2}}
	\end{align*}
	so that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B+2\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot\sqrt{\mathbb{E}\|\overline{y}_{t+1}-\overline{y}_{t}\|^{2}}\\
	& \leq(1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B+2\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot G
	\end{align*}
	and again we can conclude that $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq K^{2}$
	for $t\geq0$, for $K$ satisfying 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}
	\end{align*}
	and
	\begin{align*}
	\|w_{0}-w^{\ast}\|^{2} & \leq K^{2}
	\end{align*}
	
	Finally, the bound on $\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle$
	is exactly the same as in the proof for the strongly convex and smooth
	case, and we may conclude that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})
	\end{align*}
	where 
	\begin{align*}
	B' & =B+2K^{2}\\
	& =6G^{2}+32(E-1)^{2}G^{2}+2K^{2}
	\end{align*}
	
	To conclude the proof, we apply the averaging trick of \textbf{TODO:CITE
		LACOSTE }to get \textbf{
		\begin{align*}
		F(\sum_{t=1}^{T}\frac{2t}{T(T+1)}\overline{w}_{t})-F^{\ast} & \leq\frac{2B'}{\mu(T+1)}
		\end{align*}
	}
\end{proof}
%
We now move on to prove the result in the case of partial participation.
Now the FedAvg algorithm with Nesterov Accelerated SGD (NASGD) follows
the updates
\begin{align*}
y_{t+1}^{k} & =w_{t}^{k}-\alpha_{t}g_{t,k}\\
w_{t+1}^{k} & =\begin{cases}
y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}) & \text{if }t+1\notin\mathcal{I}_{E}\\
\sum_{k\in\mathcal{S}_{t+1}}\left(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})\right) & \text{if }t+1\in\mathcal{I}_{E}
\end{cases}
\end{align*}
where $\mathcal{S}_{t+1}$ is the multiset obtained by sampling from
$[N]$ according to $p_{k}$, \emph{with replacement, }a total of
$S=|\mathcal{S}_{t+1}|$ times. 

As before we define the virtual sequences $\overline{y}_{t}=\sum_{k=1}^{N}p_{k}y_{t}^{k}$,
$\overline{w}_{t}=\sum_{k=1}^{N}p_{k}w_{t}^{k}$, and $\overline{g}_{t}=\sum_{k=1}^{N}p_{k}\mathbb{E}g_{t,k}$.
We have $\mathbb{E}g_{t}=\overline{g}_{t}$ and $\overline{y}_{t+1}=\overline{w}_{t}-\alpha_{t}g_{t}$,
and as in the full participation case, $\overline{w}_{t+1}=\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})$
for $t+1\notin\mathcal{I}_{E}$. When $t+1$ is a communication round,
because of the sampling step, this identity is no longer true, but
is true when we take expectation with respect to the sampling distribution
$\mathbb{P}_{\mathcal{S}_{t+1}}$. 
\begin{theorem}
	(Partial device participation) Suppose $F_{k}$ is $\mu$-strongly
	convex for all $k$. Let $E$ be the communication interval, and learning
	rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(E+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $c$ is small enough
	such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|\nabla F_{k}(w,\xi_{t}^{k})\|^{2}\leq G^{2}$
	for $w=\overline{w}_{t}$ or $w=w_{t}^{k}$ and all $t,k$.
	
	Then with partial device participation, \textbf{
		\begin{align*}
		F(\sum_{t=1}^{T}\frac{2t}{T(T+1)}\overline{w}_{t})-F^{\ast} & \leq\frac{2(B'+C)}{\mu(T+1)}
		\end{align*}
	} where
	\begin{align*}
	B' & =6G^{2}+32(E-1)^{2}G^{2}+2K^{2}\\
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =6G^{2}+32(E-1)^{2}G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}
%
\begin{proof}
	We have
	\begin{align*}
	\|\overline{w}_{t+1}-w^{\ast}\|^{2} & =\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))+(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\|^{2}\\
	& =\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}+\|(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\|^{2}\\
	& +2\langle\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})),(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\rangle
	\end{align*}
	
	Note that 
	\begin{align*}
	\mathbb{E}_{\mathcal{S}_{t+1}}\langle\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})),(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\rangle & =0
	\end{align*}
	since 
	\begin{align*}
	\mathbb{E}_{\mathcal{S}_{t+1}}\overline{w}_{t+1} & =\mathbb{E}_{\mathcal{S}_{t+1}}\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}\mathbb{E}_{\mathcal{S}_{t+1}}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\frac{1}{S}\cdot S\cdot\sum_{k=1}^{N}p_{k}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})
	\end{align*}
	Moreover, if $t+1\notin\mathcal{I}_{E}$, $\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}=0$
	as well, while if $t+1\notin\mathcal{I}_{E}$, we show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2} & \leq\frac{16}{S}\alpha_{t}^{2}E^{2}G^{2}
	\end{align*}
	using the same proof as the strongly convex and smooth case. Moreover,
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})
	\end{align*}
	by the proof from the full participation case. Now we can conclude
	that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}(B'+C)-2\alpha_{t}\mathbb{E}(F(\overline{w}_{t})-F^{\ast})
	\end{align*}
	where 
	\begin{align*}
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	
	The proof then following by applying the averaging trick from the
	full participation case replacing $B'$ with $B'+C$.
\end{proof}

==> sec_nasgd_scvx_smooth.tex <==
We show that FedAvg with Accelerated SGD has $O(1/T)$ rate under
$\mu$-strong convexity and $L$-smoothness. The proof follows the
framework of the ICLR paper. The FedAv algorithm with Nesterov Accelerated
SGD (NASGD) follows the updates
\begin{align*}
y_{t+1}^{k} & =w_{t}^{k}-\alpha_{t}g_{t,k}\\
w_{t+1}^{k} & =\begin{cases}
y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}) & \text{if }t+1\notin\mathcal{I}_{E}\\
\sum_{k=1}^{N}p_{k}\left[y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})\right] & \text{if }t+1\in\mathcal{I}_{E}
\end{cases}
\end{align*}
where 
\begin{align*}
g_{t,k} & :=\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})
\end{align*}
is the stochastic gradient. 

Define the virtual sequences $\overline{y}_{t}=\sum_{k=1}^{N}p_{k}y_{t}^{k}$,
$\overline{w}_{t}=\sum_{k=1}^{N}p_{k}w_{t}^{k}$, and $\overline{g}_{t}=\sum_{k=1}^{N}p_{k}\mathbb{E}g_{t,k}$.
We have $\mathbb{E}g_{t}=\overline{g}_{t}$ and $\overline{y}_{t+1}=\overline{w}_{t}-\alpha_{t}g_{t}$,
and $\overline{w}_{t+1}=\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})$. 

We first summarize some properties of $L$-smooth and $\mu$-strongly
convex functions. 
\begin{lemma}
	Let $F$ be a convex $L$-smooth function. Then we have the following
	inequalities:
	
	1. Quadratic upper bound: $0\leq F(w)-F(w')-\langle\nabla F(w'),w-w'\rangle\leq\frac{L}{2}\|w-w'\|^{2}$. 
	
	2. Coercivity: $\frac{1}{L}\|\nabla F(w)-\nabla F(w')\|^{2}\leq\langle\nabla F(w)-\nabla F(w'),w-w'\rangle$.
	
	3. Lower bound: $F(w)\geq F(w')+\langle\nabla F(w'),w-w'\rangle+\frac{1}{2L}\|\nabla F(w)-\nabla F(w')\|^{2}$.
	In particular, $\|\nabla F(w)\|^{2}\leq2L(F(w)-F(w^{\ast}))$.
	
	4. Optimality gap: $F(w)-F(w^{\ast})\leq$$\langle\nabla F(w),w-w^{\ast}\rangle$.
\end{lemma}
%
\begin{lemma}
	Let $F$ be a $\mu$-strongly convex function. Then 
	\begin{align*}
	F(w) & \leq F(w')+\langle\nabla F(w'),w-w'\rangle+\frac{1}{2\mu}\|\nabla F(w)-\nabla F(w')\|^{2}\\
	F(w)-F(w^{\ast}) & \leq\frac{1}{2\mu}\|\nabla F(w)\|^{2}
	\end{align*}
\end{lemma}
\begin{theorem}
	(Full device participation) Suppose $F_{k}$ is $L$-smooth and $\mu$-strongly
	convex for all $k$. Let $\kappa=\frac{L}{\mu}$, $\gamma=\max\{8\kappa-1,E\}$
	where $E$ is the communication interval, and learning rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(\gamma+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $0\leq c\leq1$
	is small enough such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	\alpha_{t} & \leq\frac{1}{4L}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|g_{t,k}\|^{2}\leq G^{2}$ for all $t,k$. 
	
	Then with full device participation, 
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq\frac{\kappa}{\gamma+t}(\frac{B'}{\mu}+4L\|w_{0}-w^{\ast}\|^{2})\\
	B' & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}+2K^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}
\begin{proof}
	First, we derive a bound on $\mathbb{E}\|\overline{y}_{t+1}-\overline{y}_{t}\|^{2}$
	that is useful in the proof. We have the recursion 
	\begin{align*}
	y_{t+1}^{k}-y_{t}^{k} & =w_{t}^{k}-w_{t-1}^{k}-(\alpha_{t}g_{t,k}-\alpha_{t-1}g_{t-1,k})\\
	w_{t+1}^{k}-w_{t}^{k} & =-\alpha_{t}g_{t,k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})
	\end{align*}
	so that 
	\begin{align*}
	y_{t+1}^{k}-y_{t}^{k} & =-\alpha_{t-1}g_{t-1,k}+\beta_{t-1}(y_{t}^{k}-y_{t-1}^{k})-(\alpha_{t}g_{t,k}-\alpha_{t-1}g_{t-1,k})\\
	& =\beta_{t-1}(y_{t}^{k}-y_{t-1}^{k})-\alpha_{t}g_{t,k}
	\end{align*}
	Since the identity $y_{t+1}^{k}-y_{t}^{k}=\beta_{t-1}(y_{t}^{k}-y_{t-1}^{k})-\alpha_{t}g_{t,k}$
	implies 
	\begin{align*}
	\mathbb{E}\|y_{t+1}^{k}-y_{t}^{k}\|^{2} & \leq2\beta_{t-1}^{2}\mathbb{E}\|y_{t}^{k}-y_{t-1}^{k}\|^{2}+2\alpha_{t}^{2}G^{2}
	\end{align*}
	as long as $\alpha_{t},\beta_{t}$ satisfy $2\beta_{t-1}^{2}+2\alpha_{t}^{2}\leq1$,
	and\textbf{ $\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}\leq G^{2}$},
	we can guarantee that $\mathbb{E}\|y_{t}^{k}-y_{t-1}^{k}\|^{2}\leq G^{2}$.
	This together with Jensen's inequality gives $\mathbb{E}\|\overline{y}_{t}-\overline{y}_{t-1}\|^{2}\leq G^{2}$
	for all $t$. 
	
	The idea of the proof is to observe that the $L$-smoothness of $F$
	provides the upper bound
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & =\mathbb{E}(F(\overline{w}_{t})-F(w^{\ast}))\\
	& \leq\frac{L}{2}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}
	\end{align*}
	and to show that $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}=O(\frac{1}{t})$. 
	
	Our main step is to prove the bound 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'
	\end{align*}
	where $B'$ is define in the statement of the theorem. 
	
	We have 
	\begin{align*}
	\|\overline{w}_{t+1}-w^{\ast}\|^{2} & =\|(\overline{w}_{t}-\alpha_{t}g_{t})+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-w^{\ast}\|^{2}\\
	& =\|(\overline{w}_{t}-\alpha_{t}\overline{g}_{t}-w^{\ast})+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}(g_{t}-\overline{g}_{t})\|^{2}\\
	& =A_{1}+A_{2}+A_{3}
	\end{align*}
	where 
	\begin{align*}
	A_{1} & =\|\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}\\
	A_{2} & =2\alpha_{t}\langle\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}),\overline{g}_{t}-g_{t}\rangle\\
	A_{3} & =\alpha_{t}^{2}\|g_{t}-\overline{g}_{t}\|^{2}
	\end{align*}
	$\mathbb{E}A_{2}=0$ by definition of $g_{t}$ and $\overline{g}_{t}$,
	while for $A_{3}$ we have
	\begin{align*}
	\alpha_{t}^{2}\mathbb{E}\|g_{t}-\overline{g}_{t}\|^{2} & =\alpha_{t}^{2}\mathbb{E}\|g_{t}-\mathbb{E}g_{t}\|^{2}\leq\alpha_{t}^{2}\mathbb{E}\|g_{t}\|^{2}\\
	& =\alpha_{t}^{2}\mathbb{E}\|\sum_{k=1}^{N}p_{k}g_{t,k}\|^{2}\leq\alpha_{t}^{2}\mathbb{E}\sum_{k=1}^{N}p_{k}\|g_{t,k}\|^{2}\leq\alpha_{t}^{2}G^{2}
	\end{align*}
	again by Jensen's inequality.
	
	Next we bound $A_{1}$: 
	\begin{align*}
	\|\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2} & =\|\overline{w}_{t}-w^{\ast}\|^{2}+2\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}\overline{g}_{t}\rangle+\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}\overline{g}_{t}\|^{2}\\
	& \leq\|\overline{w}_{t}-w^{\ast}\|^{2}+2\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}\overline{g}_{t}\rangle+2\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}+2\|\alpha_{t}\overline{g}_{t}\|^{2}
	\end{align*}
	
	The last two terms are straightforward to bound: $\mathbb{E}\|\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})\|^{2}\leq\beta_{t}^{2}G^{2}\leq\alpha_{t}^{2}G^{2}$,
	while by the convexity of $\|\cdot\|^{2}$ and $L$-smoothness of
	$F_{k}$,
	\begin{align*}
	2\alpha_{t}^{2}\|\overline{g}_{t}\|^{2} & \leq2\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}\|\nabla F_{k}(w_{t}^{k})\|^{2}\leq4L\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast})
	\end{align*}
	
	Now 
	\begin{align*}
	2\langle\overline{w}_{t}-w^{\ast},\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})-\alpha_{t}\overline{g}_{t}\rangle & =2\beta_{t}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle\\
	& =B_{1}+B_{2}
	\end{align*}
	where 
	\begin{align*}
	B_{1} & =2\beta_{t}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle\\
	B_{2} & =-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle
	\end{align*}
	we first bound $B_{2}$. We have
	\begin{align*}
	-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle & =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle\\
	& =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w_{t}^{k},\nabla F_{k}(w_{t}^{k})\rangle-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle w_{t}^{k}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle
	\end{align*}
	and again we bound the two terms separately. 
	
	Using $\|\frac{1}{\sqrt{\alpha_{t}}}(\overline{w}_{t}-w_{t}^{k})-\sqrt{\alpha_{t}}\nabla F_{k}(w_{t}^{k})\|^{2}\geq0$,
	we have
	\begin{align*}
	-2\langle\overline{w}_{t}-w_{t}^{k},\nabla F_{k}(w_{t}^{k})\rangle & \leq\frac{1}{\alpha_{t}}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}\|\nabla F_{k}(w_{t}^{k})\|^{2}
	\end{align*}
	Using the $L$-smoothness of $F_{k}$,
	\begin{align*}
	-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w_{t}^{k},\nabla F_{k}(w_{t}^{k})\rangle & \leq\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+2\alpha_{t}^{2}L\cdot\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast})
	\end{align*}
	
	On the other hand, the $\mu$-strong convexity of $F_{k}$ implies
	\begin{align*}
	-(w_{t}^{k}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle & \leq-\langle F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))-\frac{\mu}{2}\|w_{t}^{k}-w^{\ast}\|^{2}
	\end{align*}
	
	Combining the above, 
	\begin{align*}
	B_{2}=-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle & \leq\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+2\alpha_{t}^{2}L\cdot\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast})\\
	& -2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))-\mu\alpha_{t}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w^{\ast}\|^{2}
	\end{align*}
	and the last term $-\mu\alpha_{t}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w^{\ast}\|^{2}\leq-\mu\alpha_{t}\|\sum_{k=1}^{N}p_{k}w_{t}^{k}-w^{\ast}\|^{2}=-\mu\alpha_{t}\|\overline{w}_{t}-w^{\ast}\|^{2}$
	by Jensen. 
	
	Plugging in the bound for $B_{2}$, we have so far proved 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+3\alpha_{t}^{2}G^{2}+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle\\
	& +\underset{C}{\underbrace{6L\alpha_{t}^{2}\mathbb{E}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast})-2\alpha_{t}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))}}
	\end{align*}
	To bound $C$, note that 
	\begin{align*}
	\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast}) & =\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast})+F_{k}(w^{\ast})-F_{k}^{\ast})\\
	& =\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))+\Gamma
	\end{align*}
	and 
	\begin{align*}
	C & =-2\alpha_{t}(1-3\alpha_{t}L)\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast}))+6L\alpha_{t}^{2}\Gamma
	\end{align*}
	Furthermore, by convexity and $L$-smoothness,
	\begin{align*}
	\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(w^{\ast})) & =\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}(\overline{w}_{t})+F_{k}(\overline{w}_{t})-F_{k}(w^{\ast}))\\
	& \geq\sum_{k=1}^{N}p_{k}\langle\nabla F_{k}(\overline{w}_{t}),w_{t}^{k}-\overline{w}_{t}\rangle+F_{k}(\overline{w}_{t})-F_{k}(w^{\ast}))\\
	& \geq-\frac{1}{2}\sum_{k=1}^{N}p_{k}\left[\alpha_{t}\|\nabla F_{k}(\overline{w}_{t})\|^{2}+\frac{1}{\alpha_{t}}\|w_{t}^{k}-\overline{w}_{t}\|^{2}\right]+F_{k}(\overline{w}_{t})-F_{k}(w^{\ast}))\\
	& \geq-\sum_{k=1}^{N}p_{k}\left[\alpha_{t}L(F_{k}(\overline{w}_{k})-F_{k}^{\ast})+\frac{1}{2\alpha_{t}}\|w_{t}^{k}-\overline{w}_{t}\|^{2}\right]+F_{k}(\overline{w}_{t})-F_{k}(w^{\ast}))
	\end{align*}
	and so 
	\begin{align*}
	C & \leq2\alpha_{t}(1-3\alpha_{t}L)\sum_{k=1}^{N}p_{k}\left[\alpha_{t}L(F_{k}(\overline{w}_{k})-F_{k}^{\ast})+\frac{1}{2\alpha_{t}}\|w_{t}^{k}-\overline{w}_{t}\|^{2}\right]-2\alpha_{t}(1-3\alpha_{t}L)(F_{k}(\overline{w}_{t})-F_{k}(w^{\ast}))+6L\alpha_{t}^{2}\Gamma\\
	& =2\alpha_{t}(1-3\alpha_{t}L)(\alpha_{t}L-1)\sum_{k=1}^{N}p_{k}\alpha_{t}L(F_{k}(\overline{w}_{k})-F^{\ast})+(6L\alpha_{t}^{2}+2\alpha_{t}(1-3\alpha_{t}L)\alpha_{t}L)\Gamma+(1-3\alpha_{t}L)\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t}\|^{2}\\
	& \leq(6L\alpha_{t}^{2}+2\alpha_{t}(1-3\alpha_{t}L)\alpha_{t}L)\Gamma+(1-3\alpha_{t}L)\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t}\|^{2}\\
	& \leq8\alpha_{t}^{2}\Gamma+\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t}\|^{2}
	\end{align*}
	using $\alpha_{t}\leq\frac{1}{4L}$, $F_{k}(\overline{w}_{k})-F^{\ast}\geq0$,
	and 
	
	Plugging this back in, we get 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+2\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+3\alpha_{t}^{2}G^{2}+8L\alpha_{t}^{2}\Gamma+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle
	\end{align*}
	
	Now we bound $\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}$.
	Since communication is done every $E$ steps, for any $t\geq0$, we
	can find a $t_{0}\leq t$ such that $t-t_{0}\leq E-1$ and $w_{t_{0}}^{k}=\overline{w}_{t_{0}}$for
	all $k$. Moreover, using $\eta_{t}$ is non-increasing and $\alpha_{t_{0}}\leq\alpha{}_{t}$
	for any $t-t_{0}\leq E-1$, we have 
	\begin{align*}
	\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2} & =\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t_{0}}-(\overline{w}_{t}-\overline{w}_{t_{0}})\|^{2}\\
	& \leq\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t_{0}}\|^{2}\\
	& =\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w_{t_{0}}^{k}\|^{2}\\
	& =\mathbb{E}\sum_{k=1}^{N}p_{k}\|\sum_{i=t_{0}}^{t-1}\beta_{i}(y_{i+1}^{k}-y_{i}^{k})-\sum_{i=t_{0}}^{t-1}\alpha_{i}g_{i,k}\|^{2}\\
	& \leq2\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\alpha_{i}^{2}\|g_{i,k}\|^{2}+2\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\beta_{i}^{2}\|(y_{i+1}^{k}-y_{i}^{k})\|^{2}\\
	& \leq2\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\alpha_{i}^{2}(\|g_{i,k}\|^{2}+\|(y_{i+1}^{k}-y_{i}^{k})\|^{2})\\
	& \leq4\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\alpha_{i}^{2}G^{2}\\
	& \leq4(E-1)^{2}\alpha_{t_{0}}^{2}G^{2}\leq16(E-1)^{2}\alpha_{t}^{2}G^{2}
	\end{align*}
	where we have used $\mathbb{E}\|(y_{i+1}^{k}-y_{i}^{k})\|^{2}\leq G^{2}$
	as proved earlier. 
	
	Using the bound on $\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}$,
	we can conclude that 
	
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+8L\alpha_{t}^{2}\Gamma+32\alpha_{t}^{2}(E-1)^{2}G^{2}+3\alpha_{t}^{2}G^{2}\\
	& +2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle\\
	& =(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B+2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle
	\end{align*}
	where 
	\begin{align*}
	B & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}
	\end{align*}
	Our next step is to show that $2\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle=O(\alpha_{t}^{2})$
	as well. 
	
	With appropriate choice of constant $K$ depending on the other constants,
	we first show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq K^{2}
	\end{align*}
	for all $t$, i.e. the updates always stay in a large ball around
	the optimum during the Nesterov accelerated gradient descent. In general
	this can be shown for coercive functions using Lyapunov function arguments.
	We prove it here using elementary arguments. Note that
	\begin{align*}
	\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle & \leq\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot\sqrt{\mathbb{E}\|\overline{y}_{t+1}-\overline{y}_{t}\|^{2}}
	\end{align*}
	by Cauchy-Schwarz so that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B+2\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot\sqrt{\mathbb{E}\|\overline{y}_{t+1}-\overline{y}_{t}\|^{2}}\\
	& \leq(1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B+2\beta_{t}\sqrt{\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}}\cdot G
	\end{align*}
	where $B=8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}$. For a large $K$ satisfying
	$\|w_{0}-w^{\ast}\|^{2}\leq K^{2}$, we show by induction that $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq K^{2}$
	for all $t\geq0$. 
	
	Suppose $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq K^{2}$ for
	some $t$, then 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\alpha_{t}\mu)K^{2}+\alpha_{t}^{2}B+2\beta_{t}K\cdot G\\
	& \leq K^{2}+(\alpha_{t}^{2}B+2\alpha_{t}K\cdot G-\alpha_{t}\mu K^{2})
	\end{align*}
	and as long as $\alpha_{0}$ and $K$ satisfy 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}
	\end{align*}
	then since $\alpha_{t}\leq\alpha_{0}$, we get $\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2}\leq K$,
	where $K$ only depends on $G,L,\mu,\Gamma,\|w_{0}-w^{\ast}\|^{2},E$. 
	
	Now we can finally bound $\beta_{t}\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle$.
	Recall the recursive relation
	\begin{align*}
	\overline{y}_{t+1}-\overline{y}_{t} & =\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})-\alpha_{t}g_{t}
	\end{align*}
	and so 
	\begin{align*}
	\beta_{t}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle & =\beta_{t}\langle\overline{w}_{t}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})-\alpha_{t}g_{t}\rangle\\
	& =\beta_{t}\langle\overline{w}_{t}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle-\beta_{t}\langle\overline{w}_{t}-w^{\ast},\alpha_{t}g_{t}\rangle
	\end{align*}
	and we further expand the first term: 
	\begin{align*}
	\beta_{t}\langle\overline{w}_{t}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle & =\beta_{t}\langle\overline{w}_{t}-\overline{w}_{t-1}+\overline{w}_{t-1}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle\\
	& =\beta_{t}\langle\overline{w}_{t}-\overline{w}_{t-1},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle+\beta_{t}\langle\overline{w}_{t-1}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle\\
	& =\beta_{t}\beta_{t-1}\langle-\alpha_{t-1}g_{t-1}+\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1}),(\overline{y}_{t}-\overline{y}_{t-1})\rangle+\beta_{t}\langle\overline{w}_{t-1}-w^{\ast},\beta_{t-1}(\overline{y}_{t}-\overline{y}_{t-1})\rangle\\
	& =\beta_{t}\beta_{t-1}\langle-\alpha_{t-1}g_{t-1},(\overline{y}_{t}-\overline{y}_{t-1})\rangle+\beta_{t}\beta_{t-1}^{2}\|\overline{y}_{t}-\overline{y}_{t-1}\|^{2}+\beta_{t}\beta_{t-1}\langle\overline{w}_{t-1}-w^{\ast},(\overline{y}_{t}-\overline{y}_{t-1})\rangle
	\end{align*}
	and so 
	\begin{align*}
	\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle & =-\beta_{t-1}\alpha_{t-1}\langle g_{t-1},\overline{y}_{t}-\overline{y}_{t-1}\rangle+\beta_{t-1}^{2}\|\overline{y}_{t}-\overline{y}_{t-1}\|^{2}+\beta_{t-1}\langle\overline{w}_{t-1}-w^{\ast},(\overline{y}_{t}-\overline{y}_{t-1})\rangle-\alpha_{t}\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle
	\end{align*}
	Noting the recursive structure of the above identity, we can show
	by induction that $|\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle|\leq2\alpha_{t}K^{2}$\textbf{
	}for all $t\geq0$ if $4\alpha_{t-1}^{2}\leq\alpha_{t}$. We check
	that 
	\begin{align*}
	\mathbb{E}|\langle w_{0}-w^{\ast},w_{0}-\alpha_{0}g_{0,k}\rangle| & \leq\sqrt{\|w_{0}-w^{\ast}\|^{2}}\cdot\sqrt{\|w_{0}-\alpha_{0}g_{0,k}\|^{2}}\leq GK\leq2\alpha_{0}K^{2}
	\end{align*}
	if $2\alpha_{0}K\geq G$, then $|\mathbb{E}\langle\overline{w}_{t-1}-w^{\ast},(\overline{y}_{t}-\overline{y}_{t-1})\rangle|\leq2\alpha_{t-1}K^{2}$
	for some $t$ implies 
	\begin{align*}
	|\mathbb{E}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle| & \leq\beta_{t-1}\alpha_{t-1}\mathbb{E}|\langle g_{t-1},\overline{y}_{t}-\overline{y}_{t-1}\rangle|+\beta_{t-1}^{2}\mathbb{E}\|\overline{y}_{t}-\overline{y}_{t-1}\|^{2}+2\alpha_{t-1}K^{2}+\alpha_{t}\mathbb{E}|\langle\overline{w}_{t}-w^{\ast},g_{t}\rangle|\\
	& \leq\alpha_{t-1}^{2}G^{2}+\alpha_{t-1}^{2}G^{2}+2\alpha_{t-1}^{2}K^{2}+\alpha_{t}KG\\
	& \leq4\alpha_{t-1}^{2}K^{2}+\alpha_{t}K^{2}\leq2\alpha_{t}^{2}K^{2}
	\end{align*}
	
	This gives the bound
	\begin{align*}
	|\mathbb{E}\beta_{t}\langle\overline{w}_{t}-w^{\ast},(\overline{y}_{t+1}-\overline{y}_{t})\rangle| & \leq2\alpha_{t}^{2}K^{2}
	\end{align*}
	and so
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'
	\end{align*}
	where 
	\begin{align*}
	B' & =B+2K^{2}\\
	& =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}+2K^{2}
	\end{align*}
	
	To complete the proof of convergence, for $\alpha_{t}=\frac{\delta}{t+\gamma}$
	for $\delta>\frac{1}{\mu}$ and $\gamma>0$ such that $\alpha_{1}\leq\min\{\frac{1}{\mu},\frac{1}{4L}\}$and
	$\alpha_{t}\leq2\alpha_{t+E}$, we can show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2} & \leq\frac{v}{\gamma+t}
	\end{align*}
	where $v=\max\{\frac{\delta^{2}B'}{\delta\mu-c+1},(\gamma+1)\|w_{0}-w^{\ast}\|^{2}\}$
	by induction. The definition of $v$ ensures that 
	\begin{align*}
	\|w_{0}-w^{\ast}\|^{2} & \leq\frac{v}{\gamma}
	\end{align*}
	and suppose $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq\frac{v}{\gamma+t}$
	holds for some $t\geq0$. Then 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2}\leq & (1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'\\
	& \leq(1-\frac{\delta\mu}{t+\gamma})\frac{v}{t+\gamma}+\frac{\delta^{2}B'}{(t+\gamma)^{2}}\\
	& =\frac{t+\gamma-1}{(t+\gamma)^{2}}v+\left[\frac{\delta^{2}B'}{(t+\gamma)^{2}}-\frac{\delta\mu-1}{(t+\gamma)^{2}}v\right]\\
	& \leq\frac{v}{t+\gamma+1}
	\end{align*}
	by definition of $v$.
	
	Finally, the $L$-smoothness of $F$ implies 
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & =\mathbb{E}(F(\overline{w}_{t})-F(w^{\ast}))\\
	& \leq\frac{L}{2}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq\frac{L}{2}\frac{v}{\gamma+t}
	\end{align*}
	Now if we choose $\delta=\frac{c}{\mu}$ where $c\leq1$ is small
	enough such that the required conditions 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	\alpha_{t} & \leq\frac{1}{4L}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	hold for all $t\geq0$, $\gamma=\max\{8\kappa-1,E\}$, then $\alpha_{t}=\frac{c}{\mu}\frac{1}{\gamma+t}$
	and recalling $v=\max\{\frac{\delta^{2}B'}{\delta\mu-c+1},(\gamma+1)\|w_{0}-w^{\ast}\|^{2}\}$,
	we finally have 
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & \leq\frac{L}{2}\frac{v}{\gamma+t}\leq\frac{L/2}{\gamma+t}(\frac{\delta^{2}B'}{\delta\mu-c+1}+(\gamma+1)\|w_{0}-w^{\ast}\|^{2})\\
	& \leq\frac{\kappa}{\gamma+t}(\frac{B'}{\mu}+4L\|w_{0}-w^{\ast}\|^{2})
	\end{align*}
\end{proof}
%
We now move on to prove the result in the case of partial participation.
Now the FedAvg algorithm with Nesterov Accelerated SGD (NASGD) follows
the updates
\begin{align*}
y_{t+1}^{k} & =w_{t}^{k}-\alpha_{t}g_{t,k}\\
w_{t+1}^{k} & =\begin{cases}
y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}) & \text{if }t+1\notin\mathcal{I}_{E}\\
\sum_{k\in\mathcal{S}_{t+1}}\left(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})\right) & \text{if }t+1\in\mathcal{I}_{E}
\end{cases}
\end{align*}
where $\mathcal{S}_{t+1}$ is the multiset obtained by sampling from
$[N]$ according to $p_{k}$, \emph{with replacement, }a total of
$S=|\mathcal{S}_{t+1}|$ times. 

As before we define the virtual sequences $\overline{y}_{t}=\sum_{k=1}^{N}p_{k}y_{t}^{k}$,
$\overline{w}_{t}=\sum_{k=1}^{N}p_{k}w_{t}^{k}$, and $\overline{g}_{t}=\sum_{k=1}^{N}p_{k}\mathbb{E}g_{t,k}$.
We have $\mathbb{E}g_{t}=\overline{g}_{t}$ and $\overline{y}_{t+1}=\overline{w}_{t}-\alpha_{t}g_{t}$,
and as in the full participation case, $\overline{w}_{t+1}=\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})$
for $t+1\notin\mathcal{I}_{E}$. When $t+1$ is a communication round,
because of the sampling step, this identity is no longer true, but
is true when we take expectation with respect to the sampling distribution
$\mathbb{P}_{\mathcal{S}_{t+1}}$. 
\begin{theorem}
	(Partial device participation) Suppose $F_{k}$ is $L$-smooth and
	$\mu$-strongly convex for all $k$. Let $\kappa=\frac{L}{\mu}$,
	$\gamma=\max\{8\kappa-1,E\}$ where $E$ is the communication interval,
	and learning rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(\gamma+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $0\leq c\leq1$
	is small enough such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	\alpha_{t} & \leq\frac{1}{4L}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|g_{t,k}\|^{2}\leq G^{2}$ for all $t,k$. 
	
	Then with the partial device participation scheme described above,
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq\frac{\kappa}{\gamma+T}(\frac{B'+C}{\mu}+4L(\|w_{0}-w^{\ast}\|^{2})\\
	B' & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}+2K^{2}\\
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}
%
\begin{proof}
	We have
	\begin{align*}
	\|\overline{w}_{t+1}-w^{\ast}\|^{2} & =\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))+(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\|^{2}\\
	& =\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}+\|(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\|^{2}\\
	& +2\langle\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})),(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\rangle
	\end{align*}
	Note that 
	\begin{align*}
	\mathbb{E}_{\mathcal{S}_{t+1}}\langle\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})),(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\rangle & =0
	\end{align*}
	since 
	\begin{align*}
	\mathbb{E}_{\mathcal{S}_{t+1}}\overline{w}_{t+1} & =\mathbb{E}_{\mathcal{S}_{t+1}}\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}\mathbb{E}_{\mathcal{S}_{t+1}}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\frac{1}{S}\cdot S\cdot\sum_{k=1}^{N}p_{k}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))\\
	& =\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t})
	\end{align*}
	Moreover, if $t+1\notin\mathcal{I}_{E}$, $\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}=0$
	as well, while if $t+1\notin\mathcal{I}_{E}$, we show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2} & =O(\alpha_{t}^{2})
	\end{align*}
	assuming $\eta_{t}$ is non-increasing and $\eta_{t}\leq2\eta_{t+E}$
	for all $t\geq0$. We have 
	\begin{align*}
	\mathbb{E}_{\mathcal{S}_{t+1}}\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2} & =\mathbb{E}_{\mathcal{S}_{t+1}}\|\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}(y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k}))-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}\\
	& =\frac{1}{S^{2}}\sum_{k\in\mathcal{S}_{t+1}}\mathbb{E}_{\mathcal{S}_{t+1}}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}\\
	& =\frac{1}{S}\sum_{k=1}^{N}p_{k}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}
	\end{align*}
	where we have used the general fact that $\mathbb{E}\|\frac{1}{S}\sum_{k\in\mathcal{S}_{t+1}}x_{k}-\mathbb{E}x_{k}\|^{2}=\frac{1}{S^{2}}\sum_{k\in\mathcal{S}_{t+1}}\mathbb{E}\|x_{k}-\mathbb{E}x_{k}\|^{2}$
	for $x_{k}$ iid. Since $t+1\in\mathcal{I}_{E}$, we know that $t_{0}=t-E+1\in\mathcal{I}_{E}$
	is also a communication round, so that $w_{t_{0}}^{k}\equiv\overline{w}_{t_{0}}$
	does not depend on $k$. Then 
	\begin{align*}
	\sum_{k=1}^{N}p_{k}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2} & =\sum_{k=1}^{N}p_{k}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-\overline{w}_{t_{0}}+\overline{w}_{t_{0}}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2}\\
	& \leq\sum_{k=1}^{N}p_{k}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-\overline{w}_{t_{0}}\|^{2}
	\end{align*}
	so that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))\|^{2} & \leq\frac{1}{S}\sum_{k=1}^{N}p_{k}\mathbb{E}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-\overline{w}_{t_{0}}\|^{2}\\
	& =\frac{1}{S}\sum_{k=1}^{N}p_{k}\mathbb{E}\|y_{t+1}^{k}+\beta_{t}(y_{t+1}^{k}-y_{t}^{k})-w_{t_{0}}^{k}\|^{2}\\
	& =\frac{1}{S}\sum_{k=1}^{N}p_{k}\mathbb{E}\|\sum_{i=t_{0}}^{t}\beta_{i}(y_{i+1}^{k}-y_{i}^{k})-\sum_{i=t_{0}}^{t}\alpha_{i}g_{i,k}\|^{2}\\
	& \leq\frac{2}{S}\left[\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t}E\alpha_{i}^{2}\|g_{i,k}\|^{2}+\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t}E\beta_{i}^{2}\|(y_{i+1}^{k}-y_{i}^{k})\|^{2}\right]\\
	& \leq\frac{16}{S}\alpha_{t}^{2}E^{2}G^{2}
	\end{align*}
	Now we turn to $\mathbb{E}\|(\overline{y}_{t+1}+\beta_{t}(\overline{y}_{t+1}-\overline{y}_{t}))-w^{\ast}\|^{2}$.
	This term is bounded in the proof of the full participation case,
	with 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'
	\end{align*}
	
	
	Now we can conclude that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}(B'+C)
	\end{align*}
	where 
	\begin{align*}
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	
	The exact argument then yields 
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq\frac{\kappa}{\gamma+T}(\frac{B'+C}{\mu}+4L(\|w_{0}-w^{\ast}\|^{2})
	\end{align*}
\end{proof}

==> sec_noncvx.tex <==
% !TEX ROOT=./main.tex



\section{Non-convex convergence rate}

{\centering
\begin{tabular}{l} 
Algorithm 1 MKL-SGD \\
\hline 1: Initialize $\boldsymbol{w}_{\mathbf{0}}$ \\
2: Given samples $D=\left(\boldsymbol{x}_{\boldsymbol{t}}, y_{t}\right)_{t=1}^{\infty}$ \\
3: for $t=1, \ldots$ do \\
4: Choose a set $S_{t}$ of $k$ samples \\
5: Select $i_{t}=\arg \min _{i \in S_{t}} f_{i}\left(\boldsymbol{w}_{t}\right)$ \\
6: Update $\boldsymbol{w}_{t+1}=\boldsymbol{w}_{t}-\eta_t \nabla f_{i_{t}}\left(\boldsymbol{w}_{t}\right)$ \\
7: end for \\
8: Return $\boldsymbol{w}_{t}$ \\
\hline
\end{tabular}}
In the algorithm, we require the step size satisfies
\begin{equation}
\sum_{t=1}^{\infty} \eta_t = \infty \text{ and } \sum_{t=1}^{\infty}\eta_t^2 < \infty
\label{eq:stepsize}
\end{equation}


\subsection{Problem Setup and Notation}
In this subsection, we analyze the convergence rate of MKL-SGD for Non-convex objective. Formally, 
we study the problem of 
 $$\min _{\boldsymbol{w}} F(\boldsymbol{w}),$$
we denote the objective function on clean dataset as $F(\vw) = \frac{1}{\|G\|} \sum_{i \in G} f_i(\vw)$ and
the objective function on noisy dataset $F_a(\vw) =\frac{1}{N} \sum_{i=1}^N f_i(\vw)$, where the
$N$ data point includes both clean data and abnormal data. 
We use $p_i(\vw_t)$ denote the probability that sample $i$ will be used for computing
gradient using MKL-SGD.

\begin{assumption}[Gradient purity]
The expected gradient of MKL-SGD in noisy dataset move in the same direction as the 
expected gradient in clean dataset.
$\langle \grad F(\vw_t),\sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) - \grad F(\vw_t) \rangle \geq 0$
\label{ass:gp}
\end{assumption}

\begin{remark}
	The Assumption~\ref{ass:gp} is relatively weak in terms of gradient norm as it tolerates the
	where noisy gradient is persistent, while it has strict requirement on the noisy gradient moves
	the object toward the correct direction with sufficient distance.
\end{remark}
In the noiseless case, we have $ \sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) = \grad F(\vw_t)$, the 
assumption is satisfied and the results reduce to regular non-convex objective convergence 
results. 

\begin{assumption}[L-smooth]
	$F(\mathbf{v}) \leq F(\mathbf{w})+\langle \mathbf{v}-\mathbf{w}, \nabla F(\mathbf{w}) \rangle +\frac{L}{2}\|\mathbf{v}-\mathbf{w}\|_{2}^{2}$.
	\label{ass:lsmooth}
\end{assumption}

\begin{assumption}[Bounded gradient norm]
	The expected square of gradient norm is bounded $\EE \|\grad F_a(\vw_t)\|_2^2  \leq G$: 
	\label{ass:bgn}
\end{assumption}





\begin{theorem}
	With assumption~\ref{ass:gp}, \ref{ass:lsmooth}, \ref{ass:bgn}, the MKL-SGD is running with
	step size $\eta_t$ satisfying \eq{\ref{eq:stepsize}}, then, with $A_T =\sum_{t=0}^T\eta_t $, 
	\begin{equation}
		\EE \frac{1}{A_T}\sum_{t=0}^T \eta_t\|\grad F(\vw_t)\|_2^2 \rightarrow 0
	\end{equation}
\end{theorem}
\begin{proof}
$\vw_{t+1} = \vw_t - \eta_t \grad f_i(\vw_t)$
\begin{align*}
	F(\vw_{t+1}) - F(\vw_{t}) & \leq \langle \grad F(\vw_t), \vw_{t+1} - \vw_t \rangle + \frac{L}{2}\|\vw_{t+1} - \vw_t\|_2^2  \\
                              &  = - \eta_t \langle \grad F(\vw_t), \grad f_i(\vw_t)\rangle  + \frac{L}{2}\|\vw_{t+1} - \vw_t\|_2^2  \\
                              & \leq - \eta_t \langle \grad F(\vw_t), \grad f_i(\vw_t)\rangle  + \frac{\eta_t^2 L}{2}\|\grad f_i(\vw_t)\|_2^2 
\end{align*}
Take expectation w.r.t $i$, condition on $\vw_t$, 
\begin{align*}
	\EE[F(\vw_{t+1})] - F(\vw_{t}) & \leq - \eta_t \langle \grad F(\vw_t),\sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) \rangle + \sum_{i=1}^N p_i(\vw_t) \frac{\eta_t^2 L}{2}\|\grad f_i(\vw_t)\|_2^2 \\
	&  \leq - \eta_t \langle \grad F(\vw_t),\sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) - \grad F(\vw_t) \rangle - \eta_t \|\grad F(\vw_t)\|_2^2 +  \frac{\eta_t^2 LG}{2}\\
\end{align*}
Take total expectation: 
\begin{align*}
	\eta_t\EE \|\grad F(\vw_t)\|_2^2 &\leq \EE[F(\vw_{t})] - \EE[F(\vw_{t+1})] + \EE[- \eta_t \langle \grad F(\vw_t),\sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) - \grad F(\vw_t) \rangle] + \frac{\eta_t^2 LG}{2}
\end{align*}
Summing both sides from $t = 0$ to $T$
\begin{align*}
	\sum_{t=0}^T \eta_t\EE \|\grad F(\vw_t)\|_2^2 &\leq \EE[F(\vw_{1})] - F_{\inf} -\sum_{t=0}^T \eta_t \EE[ \langle \grad F(\vw_t),\sum_{i=1}^N p_i(\vw_t)\grad f_i(\vw_t) - \grad F(\vw_t) \rangle] + \sum_{t=0}^T \frac{\eta_t^2 LG}{2} \\
	& \leq \EE[F(\vw_{1})] - F_{\inf} + \sum_{t=0}^T \frac{\eta_t^2 LG}{2} 
\end{align*}
The learning rate satisfies\eq{\ref{eq:stepsize}}, therefore, $\EE \frac{1}{A_T}\sum_{t=0}^T \eta_t \|\grad F(\vw_t)\|_2^2 \rightarrow 0$
	
\end{proof}



==> sec_overparameterized.tex <==
% !TEX ROOT=./main.tex



\section{Geometric Convergence of FedAvg in the Overparameterized Setting}
\label{sec:overparameterized}
% In this section, we turn to the special setting of overparameterized
% problems, where a non-negative loss function admits a zero-loss global
% minimizer. Such problems are prevalent especially at the age of deep learning,
% where the number of parameters far exceeds the number of data points,
% and perfect fitting is possible. There have been a line of recent
% works showing that SGD and accelerated methods achieve geometric
% convergence in similar settings thanks to the property of \textit{automatic
% variance reduction}~\cite{ma2017power,moulines2011non,needell2014stochastic,schmidt2013fast,strohmer2009randomized}.
% The natural question is whether such a result also holds in the federated
% learning setting. 
% We show that this is indeed the case and establish
% the geometric (linear) convergence of FedAvg with local SGD updates
% with constant step size for general strongly convex and smooth overparameterized
% problems. In addition, we show that the convergence rate speeds up
% linearly in the number of workers $N$ when $N$ is below some problem-dependent
% threshold, while it decreases with $E$ through $1/E$. 
Overparameterization is a prevalent machine learning setting where the
statistical model has much more parameters than the number of training samples
and the existence of parameter choices with zero training loss is
ensured~\cite{allen2018convergence,zhang2016understanding}.  Due to the
property of \textit{automatic variance reduction} in overparameterization,  a
line of recent works proved that SGD and accelerated methods achieve geometric
convergence~\cite{ma2017power,moulines2011non,needell2014stochastic,schmidt2013fast,strohmer2009randomized}.
A natural question is whether such a result still holds in the federated
learning setting. 
In this section, we establish the geometric convergence
of FedAvg for the overparameterized strongly convex and smooth problems,
and show that it preserves linear speedup at the same time.  
We then sharpen this result in the special case of
linear regression.
Inspired by recent advances in accelerating SGD~\cite{liu2019accelerating,jain2017accelerating}, 
we further propose a novel momentum-based FedAvg algorithm, which enjoys an
improved convergence rate over FedAvg. Detailed proofs are deferred to Appendix Section~\ref{sec:interpolation}. In particular, we do not need Assumptions~\ref{ass:boundedvariance} and~\ref{ass:subgrad2} and use modified versions of Assumptions~\ref{ass:lsmooth} and~\ref{ass:stroncvx} detailed in this section.
\begin{comment}
we deal with the question of whether FedAvg with momentum-based
local updates can outperform FedAvg with SGD updates. In contrast
to the gradient descent setting, Nesterov and Heavy Ball updates are
known to fail to accelerate over SGD, both in the overparameterized
setting and standard convex setting \cite{liu2018accelerating,kidambi2018insufficiency,liu2018toward,yuan2016influence}.
Thus in general one cannot hope to obtain acceleration results for
the FedAvg algorithm with Nesterov and Heavy Ball updates. On the
hopeful side, \cite{jain2017accelerating,liu2018accelerating} introduced
similar algorithms that make modifications of the Nesterov updates
to correct for its ``over-descent''. For quadratic objectives in
the overparamterized setting, \cite{liu2018accelerating} show their
algorithm achieves acceleration over the geometric convergence of
SGD that recovers the well-known $\mathcal{O}(\exp(-t/\sqrt{\kappa})$
acceleration of Nesterov over GD. In the last part, we introduce a
new accelerated FedAvg algorithm by adapting the MaSS algorithm of
\cite{liu2018accelerating} to the FL setting. We
show that it achieves geometric convergence for overparameterized
linear regression with an $\mathcal{O}(\exp(-\frac{NT}{E\sqrt{\kappa_{1}\tilde{\kappa}}}))$ rate,
where $\tilde{\kappa}$ is a ``statistical condition number''\cite{liu2018accelerating,jain2017accelerating}
that satisfies $\tilde{\kappa}\leq\kappa_{1}$. Thus our new FedAvg
algorithm achieves a speedup of factor $\sqrt{\kappa_{1}/\tilde{\kappa}}$
over FedAvg with local SGD updates. 
\end{comment}


\subsection{Geometric Convergence of FedAvg in the Overparameterized Setting}
Recall the FL problem $\min_{w}\sum_{k=1}^{N}p_{k}F_{k}(\mathbf{w})$
with $F_{k}(\mathbf{w})=\frac{1}{n_{k}}\sum_{j=1}^{n_{k}}\ell(\mathbf{w};\mathbf{x}_{k}^{j})$.
In this section, we consider the standard Empirical Risk Minimization (ERM) setting where $\ell$
is non-negative, $l$-smooth, and convex, and as before, each $F_{k}(\mathbf{w})$ is $L$-smooth and $\mu$-strongly convex. Note that $l\geq L$. This
setup includes many important problems in practice. In the overparameterized
setting, there exists $\mathbf{w}^{\ast}\in\arg\min_{w}\sum_{k=1}^{N}p_{k}F_{k}(\mathbf{w})$
such that $\ell(\mathbf{w}^{\ast};\mathbf{x}_{k}^{j})=0$ for all
$\mathbf{x}_{k}^{j}$. We first show that FedAvg achieves geometric convergence
with linear speedup in the number of workers. 
\begin{theorem}
	\label{thm:overparameterized_general}In the overparameterized setting,
	FedAvg with communication every $E$ iterations
	and constant step size $\overline{\alpha}=\mathcal{O}(\frac{1}{E}\frac{N}{l\nu_{\max}+L(N-\nu_{\min})})$
	has geometric convergence:
	\begin{align*}
	\mathbb{E}F(\overline{\mathbf{w}}_{T}) & \leq\frac{L}{2}(1-\overline{\alpha})^{T}\|\mathbf{w}_{0}-\mathbf{w}^{\ast}\|^{2}=\mathcal{O}\left(L\exp\left(-\frac{\mu}{E}\frac{NT}{l\nu_{\max}+L(N-\nu_{\min})}\right)\cdot\|\mathbf{w}_{0}-\mathbf{w}^{\ast}\|^{2}\right).
	\end{align*}
\end{theorem}
%
\textbf{Linear speedup and Communication Complexity} The linear speedup factor is on the order of $\mathcal{O}(N/E)$ %\frac{N}{E(l\nu_{\max}+L(N-\nu_{\min}))}/\frac{1}{l\nu_{\max}+L(1-\nu_{\min})}\approx\frac{Nl}{E(l+L(N-1))}=
for $N\leq\mathcal{O}(\frac{l}{L})$, i.e. FedAvg with $N$ workers and communication
every $E$ iterations provides a geometric convergence speedup factor
of $\mathcal{O}(N/E)$, for $N\leq\mathcal{O}(\frac{l}{L})$. When $N$ is above
this threshold, however, the speedup is almost constant in the number
of workers. This matches the findings in \cite{ma2017power}. Our
result also illustrates that $E$ can be taken $\mathcal{O}(T^{\beta})$
for any $\beta<1$ to achieve geometric convergence, achieving better communication efficiency than
the standard FL setting. 

\subsection{Overparameterized Linear Regression Problems}

We now turn to quadratic problems and show that the bound in Theorem~\ref{thm:overparameterized_general} can be improved to $\mathcal{O}(\exp(-\frac{N}{E\kappa_{1}}t))$ for a larger range of $N$. We then propose a variant of FedAvg that has provable acceleration over FedAvg with SGD updates. The local device objectives are now given by the sum of squares {\small$F_{k}(\mathbf{w})=\frac{1}{2n_{k}}\sum_{j=1}^{n_{k}}(\mathbf{w}^{T}\mathbf{x}_{k}^{j}-z_{k}^{j})^{2}$},
and there exists $\mathbf{w}^{\ast}$ such that $F(\mathbf{w}^{\ast})\equiv0$. Two notions of condition number are important in our results: $\kappa_1$ which is based on local Hessians, and $\tilde{\kappa}$, which is termed the statistical condition number~\cite{liu2018accelerating,jain2017accelerating}. For their detailed definitions, please refer to Appendix Section~\ref{sec:interpolation}. Here we use the fact $\tilde{\kappa} \leq \kappa_1$. Recall $\nu_{\max}=\max _k p_k N$ and $\nu_{\min}=\min _k p_k N$.

\begin{comment}
Define the local Hessian matrix as $H^{k}:=\frac{1}{n_{k}}\sum_{j=1}^{n_{k}}\mathbf{x}_{k}^{j}(\mathbf{x}_{k}^{j})^{T}$, and the stochastic Hessian matrix as $\tilde{H}_{t}^{k}:=\xi_{t}^{k}(\xi_{t}^{k})^{T}$. Define $l$ to be the smallest positive number such that $\mathbb{E}\|\xi_{t}^{k}\|^{2}$$\mathbf{\xi}_{t}^{k}$($\mathbf{\xi}_{t}^{k})^{T}\preceq lH^{k}$
for all $k$. Note that $l\leq\max_{k,j}\|\mathbf{x}_{k}^{j}\|^{2}$.
Let $L$ and $\mu$ be lower and upper bounds of non-zero eigenvalues
of $H^{k}$. Define $\kappa_{1}:=l/\mu$ and $\kappa:=L/\mu$. Following
\cite{liu2018accelerating,jain2017accelerating}, we define the statistical
condition number $\tilde{\kappa}$ as the smallest positive real number
such that $\mathbb{E}\left[\langle\xi_{t}^{k}(H^{k})^{-1},\xi_{t}^{k}\rangle\xi_{t}^{k}(\xi_{t}^{k})^{T}\right] \  \preceq\tilde{\kappa}H^{k}$, for all $k$. 
The condition numbers $\kappa_{1}$ and $\tilde{\kappa}$
are important in the characterization of convergence rates for FedAvg
algorithms. Note that $\kappa_{1}>\kappa$ and $\kappa_{1}>\tilde{\kappa}$.
\end{comment}
%details to be moved to the appendix.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
In general $H$ has zero eigenvalues. However, because the null space
of $H$ and range of $H$ are orthogonal, in our subsequence analysis
it suffices to project $\overline{\mathbf{w}}_{t}-\mathbf{w}^{\ast}$
onto the range of $H$, thus we may restrict to the non-zero eigenvalue
of $H$. We can use $\mathbf{w}^{\ast T}\mathbf{x}_{k}^{j}-z_{k}^{j}\equiv0$
to rewrite the local objectives as $F_{k}(\mathbf{w})=\frac{1}{2}\langle\mathbf{w}-\mathbf{w}^{\ast},H^{k}(\mathbf{w}-\mathbf{w}^{\ast})\rangle\equiv\frac{1}{2}\|\mathbf{w}-\mathbf{w}^{\ast}\|_{H^{k}}^{2}$
so that $F(\mathbf{w})=\frac{1}{2}\|\mathbf{w}-\mathbf{w}^{\ast}\|_{H}^{2}$.
\end{comment}
\begin{comment}
\begin{align*}
F_{k}(w) & =\frac{1}{2n_{k}}\sum_{j=1}^{n_{k}}(w^{T}x_{k,j}-z_{k,j}-(w^{\ast T}x_{k,j}-z_{k,j}))^{2}=\frac{1}{2n_{k}}\sum_{j=1}^{n_{k}}((w-w^{\ast})^{T}x_{k,j})^{2}\\
& =\frac{1}{2}\langle w-w^{\ast},H^{k}(w-w^{\ast})\rangle=\frac{1}{2}\|w-w^{\ast}\|_{H^{k}}^{2}
\end{align*}
\end{comment}
\begin{comment}
Let $\xi_{t}^{k}$ be the stochastic sample on the $k$th device at
time $t$, and define $\tilde{H}_{t}^{k}:=\xi_{t}^{k}(\xi_{t}^{k})^{T}$
as the stochastic Hessian matrix. %	
\end{comment}
\begin{comment}
Note that $\mathbb{E}\tilde{H}_{t}^{k}=\frac{1}{n_{k}}\sum_{j=1}^{n_{k}}\mathbf{x}_{k}^{j}(\mathbf{x}_{k}^{j})^{T}=H^{k}$
and $\mathbf{g}_{t,k}=\nabla F_{k}(\mathbf{w}_{t}^{k},\xi_{t}^{k})=\tilde{H}_{t}^{k}(\mathbf{w}_{t}^{k}-\mathbf{w}^{\ast})$
while $\mathbf{g}_{t}=\sum_{k=1}^{N}p_{k}\nabla F_{k}(\mathbf{w}_{t}^{k},\xi_{t}^{k})=\sum_{k=1}^{N}p_{k}\tilde{H}_{t}^{k}(\mathbf{w}_{t}^{k}-\mathbf{w}^{\ast})$.
\end{comment}

\begin{theorem}
	\label{thm:overparameterized_quadratic}For the overparamterized linear regression problem, FedAvg with communication every $E$
	iterations with constant step size $\overline{\alpha}=\mathcal{O}(\frac{1}{E}\frac{N}{l\nu_{\max}+\mu(N-\nu_{\min})})$
	has geometric convergence:
	\begin{align*}
	\mathbb{E}F(\overline{\mathbf{w}}_{T}) & \leq\mathcal{O}\left(L\exp(-\frac{NT}{E(\nu_{\max}\kappa_{1}+(N-\nu_{\min}))})\|\mathbf{w}_{0}-\mathbf{w}^{\ast}\|^{2}\right).
	\end{align*}
\end{theorem}

When $N=\mathcal{O}(\kappa_{1})$, the convergence rate is $\mathcal{O}((1-\frac{N}{E\kappa_{1}})^{T})=\mathcal{O}(\exp(-\frac{NT}{E\kappa_{1}}))$,
which exhibits linear speedup in the number of workers, as well as
a $1/\kappa_{1}$ dependence on the condition number $\kappa_{1}$.
Inspired by \cite{liu2018accelerating}, we propose the \textbf{MaSS
	accelerated FedAvg algorithm} (FedMaSS):
\begin{align*}
\mathbf{w}_{t+1}^{k} & =\begin{cases}
\mathbf{u}_{t}^{k}-\eta_{1}^{k}\mathbf{g}_{t,k} & \text{if }t+1\notin\mathcal{I}_{E},\\
\sum_{k \in \cS_{t+1}}\left[\mathbf{u}_{t}^{k}-\eta_{1}^{k}\mathbf{g}_{t,k}\right] & \text{if }t+1\in\mathcal{I}_{E},
\end{cases}\\
\mathbf{u}_{t+1}^{k} & =\mathbf{w}_{t+1}^{k}+\gamma^{k}(\mathbf{w}_{t+1}^{k}-\mathbf{w}_{t}^{k})+\eta_{2}^{k}\mathbf{g}_{t,k}. 
\end{align*}
When $\eta_{2}^{k}\equiv0$, this algorithm reduces to the Nesterov
accelerated FedAvg algorithm. In the next theorem, we demonstrate
that FedMaSS improves the convergence to $\mathcal{O}(\exp(-\frac{NT}{E\sqrt{\kappa_{1}\tilde{\kappa}}}))$.
To our knowledge, this is the first acceleration result of
FedAvg with momentum updates over SGD updates.
\begin{theorem}
	\label{thm:overparameterized_MaSS}For the overparamterized linear regression problem, FedMaSS with communication every $E$ iterations and constant
	step sizes $\overline{\eta}_1=\mathcal{O}(\frac{1}{E}\frac{N}{l\nu_{\max}+\mu(N-\nu_{\min})}),\overline{\eta}_{2}=\frac{\overline{\eta}_{1}(1-\frac{1}{\tilde{\kappa}})}{1+\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}},\overline{\gamma}=\frac{1-\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}}{1+\frac{1}{\sqrt{\kappa_{1}\tilde{\kappa}}}}$
	has geometric convergence:
	\begin{align*}
	\mathbb{E}F(\overline{\mathbf{w}}_{T}) & \leq\mathcal{O}\left(L\exp(-\frac{NT}{E(\nu_{\max}\sqrt{\kappa_{1}\tilde{\kappa}}+(N-\nu_{\min}))})\|\mathbf{w}_{0}-\mathbf{w}^{\ast}\|^{2}\right).
	\end{align*}
\end{theorem}
\textbf{Speedup of FedMaSS over FedAvg} 
To better understand the significance of the above result, we briefly discuss related works on accelerating SGD.
Nesterov and Heavy Ball updates are known to fail to accelerate over SGD in both the overparameterized
and convex settings~\cite{liu2018accelerating,kidambi2018insufficiency,liu2018toward,yuan2016influence}.
Thus in general one cannot hope to obtain acceleration results for
the FedAvg algorithm with Nesterov and Heavy Ball updates. 
Luckily, recent works in SGD~\cite{jain2017accelerating,liu2018accelerating} introduced
an additional compensation term to the Nesterov updates to address the non-acceleration issue. Surprisingly, 
we show the same approach can effectively improve the rate of FedAvg.
Comparing the convergence rate of FedMass (Theorem~\ref{thm:overparameterized_MaSS}) and FedAvg (Theorem~\ref{thm:overparameterized_quadratic}), when $N=\mathcal{O}(\sqrt{\kappa_{1}\tilde{\kappa}})$,
the convergence rate is $\mathcal{O}((1-\frac{N}{E\sqrt{\kappa_{1}\tilde{\kappa}}})^{T})=\mathcal{O}(\exp(-\frac{NT}{E\sqrt{\kappa_{1}\tilde{\kappa}}}))$
as opposed to $\mathcal{O}(\exp(-\frac{NT}{E\kappa_{1}}))$. Since
$\kappa_{1}\geq\tilde{\kappa}$, this implies a speedup factor of
$\sqrt{\frac{\kappa_{1}}{\tilde{\kappa}}}$ for FedMaSS. On the other
hand, the same linear speedup in the number of workers holds for $N$
in a smaller range of values. 

==> sec_overview.tex <==
% !TEX ROOT=./main.tex





\section{Proof for Convergence Results on Strongly Convex and Smooth Objectives}

% 	Stochastic gradient of device $k$ at time step $t$, at point $\vw_t^k$: $$\vg_{t,k} \coloneqq \vg_{t,k}(w_t^k)$$
% 	$$ \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}, \xi_{t}^{k}\right) $$
% 	$$\EE \vg_{t, k} = \grad F_{k}\left(w_{t}^{k}\right)$$
%   One-step stochastic subgradient of all devices.
% $$\vg_{t}=\sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) $$
% \begin{align}
% 	\EE \vg_{t}= \EE \sum_{k=1}^{N} p_{k} \vg_{t, k}\left(w_{t}^{k}\right) \coloneqq \sum_{k=1}^{N} p_{k} \EE \vg_{t, k}
% 	\label{eq:egtsgd}
% \end{align}


\subsection{Stochastic gradient descent}
\subsubsection{Convex}
\label{sec:convexsmoothsgd}
% \input{sec_convexsmoothsgd}
\input{sec_convexsmoothsgdwthvariance}

% \subsubsection{Convex}
% \label{sec:sgdcvxnonsmth}
\input{sec_cvxnonsm}

\subsection{Strongly Convex}
\input{sec_sgd_scvx_smooth}

\subsection{Stochastic Subgradient methods}
\subsubsection{Convex}
\label{sec:sgdcvxnonsmth}
\input{sec_cvxnonsm}

\subsubsection{Strongly Convex}
\label{sec:sgdscvxnonsmth}
\input{sec_sgdscvxnonsmth}



\section{Accelerated methods}
\subsection{stochastic gradient descent}
\subsubsection{Convex}
\label{sec:nasgdcvxsmth}
\input{sec_nasgd_cvx_smth}

\subsubsection{Strongly Convex}
\label{sec:nasgdscvxsmth}
\input{sec_nasgd_scvx_smooth}

\subsection{Stochastic Subgradient methods}

\subsubsection{Convex}
\label{sec:nasgdcvxnonsmth}
\input{sec_nagcvxnonsmth}

\subsubsection{Strongly Convex}
\label{sec:nasgdscvxnonsmth}
\input{sec_nasgd_scvx_nonsmooth}

\section{Exponential Acceleration of FedAvg in the Interpolation Setting}
\label{sec:interpolation}
\input{sec_interpolation}





==> sec_relatedwork.tex <==
% !TEX ROOT=./main.tex

\section{Related Work}

% Version 1.
% related work on convergence rate
% Federated learning (FL) was originally proposed
% in~\cite{mcmahan2016communication} for learning a single, global statistical
% model from the isolated data stored in a massive number of devices.  The
% empirical success of FL~\cite{chen2018federated,47586} has attracted much attention to the rigorous theoretical understanding of the leading algorithm in the field: Federated Averaging (FedAvg) and its accelerated variants~\cite{liu2019accelerating,haddadpour2019convergence,khaled2019first,li2019convergence,huo2020faster,yu2019linear,yu2019parallel}.

% % Non-convex linear speedup
% In particular, we focus on the convergence analysis of FedAvg, which
% has been studied in various scenarios. 
% In~\cite{yu2019parallel,wang2019adaptive}, the authors provide the convergence rate of FedAvg for the non-convex problem, given all the devices are active at each communication round. \cite{haddadpour2019convergence}
% improves the convergence analysis for non-convex problem under the setting of partial participation. 
% In addition, \cite{yu2019linear} provides $O(1/\sqrt{NT})$ 
% convergence (i.e., linear speedup) of FedAvg for the non-convex problem in the full participation setting. 
% For convex smooth problems, \cite{khaled2019first} prove the 
% convergence rate of local GD (a full batch version of FedAvg with full participation) on heterogeneous data. 
% Concurrently, \cite{li2019convergence} provides exponential convergence of FedAvg for the strongly convex problem,
% under the more practical setting of partial participation and Non-IID data while their results did not achieve linear speedup. 
% \cite{stich2018local} prove linear speedup convergence of FedAvg for the strongly convex problem, while they assume full participation and identically distributed data. Comparing to previous works, our results provide the linear speedup on strongly convex problems in the practical partial participation setting and heterogeneous data. In \cite{liu2019accelerating}, the authors provide a convergence rate of accelerated FedAvg for strongly convex problems, while it is considered in full participation setting. To the best of our knowledge,
% we provide the first linear speedup convergence results for accelerated FedAvg in the practical setting.


\textbf{The Convergence of FedAvg and Linear Speedup.}
There has been a vast amount of convergence analysis for FedAvg in different settings. However, most of the prior works provide the
convergence guarantee under a simplified setting, where either statistical
heterogeneity~\cite{stich2018local,zhou2017convergence,wang2018cooperative,woodworth2018graph} or system
heterogeneity~\cite{yu2019parallel,wang2019adaptive,khaled2019first,jiang2018linear} are not
considered. This simplified setting is also referred as local SGD. 
In~\cite{li2019convergence},
the authors for the first time provide convergence of FedAvg for strongly convex problem considering both statistical heterogeneity and system heterogeneity, yet it
didn't achieve linear speedup. In~\cite{haddadpour2019convergence,liang2019variance,huo2020faster,jiang2018linear}, the convergence of FedAvg for non-convex problems has been studied. 
However, \cite{huo2020faster} did not discuss the linear speedup and the theorems in \cite{haddadpour2019convergence,liang2019variance} failed to cover the accelerated version of
FedAvg. 


\textbf{Federated Learning Beyond Local SGD.}
% The accelerated SGD methods has achieved optimal convergence rate in strongly convex
% optimization~\cite{nesterov1983method}.
In \cite{liu2019accelerating}, the authors provide a convergence rate of accelerated FedAvg for strongly convex problems, while it is considered in full participation setting.
\cite{yu2019linear} and \citep{huo2020faster} provide
convergence guarantee for Nesterov accelerated FedAvg for non-convex. 
However, \cite{yu2019linear} did not consider the system heterogeneity and \cite{huo2020faster} haven't discuss the linear speedup.
Furthermore, the accelerated FedAvg admitting a similar convergence rate as FedAvg in all previous works.  In this work, we provide a novel accelerated FedAvg with improved convergence rates under a popular overparameterized setting. 








==> sec_sgd_scvx_smooth.tex <==
We first summarize some properties of $L$-smooth and $\mu$-strongly
convex functions. 
\begin{lemma}
	Let $F$ be a convex $L$-smooth function. Then we have the following
	inequalities:
	
	1. Quadratic upper bound: $0\leq F(w)-F(w')-\langle\nabla F(w'),w-w'\rangle\leq\frac{L}{2}\|w-w'\|^{2}$. 
	
	2. Coercivity: $\frac{1}{L}\|\nabla F(w)-\nabla F(w')\|^{2}\leq\langle\nabla F(w)-\nabla F(w'),w-w'\rangle$.
	
	3. Lower bound: $F(w)\geq F(w')+\langle\nabla F(w'),w-w'\rangle+\frac{1}{2L}\|\nabla F(w)-\nabla F(w')\|^{2}$.
	In particular, $\|\nabla F(w)\|^{2}\leq2L(F(w)-F(w^{\ast}))$.
	
	4. Optimality gap: $F(w)-F(w^{\ast})\leq$$\langle\nabla F(w),w-w^{\ast}\rangle$.
\end{lemma}
%
\begin{lemma}
	Let $F$ be a $\mu$-strongly convex function. Then 
	\begin{align*}
	F(w) & \leq F(w')+\langle\nabla F(w'),w-w'\rangle+\frac{1}{2\mu}\|\nabla F(w)-\nabla F(w')\|^{2}\\
	F(w)-F(w^{\ast}) & \leq\frac{1}{2\mu}\|\nabla F(w)\|^{2}
	\end{align*}
\end{lemma}
%
\begin{assumption}
	The stochastic gradients have bounded variance 
	\begin{align*}
	\mathbb{E}\|\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})-\nabla F_{k}(w_{t}^{k})\|^{2} & \leq\sigma_{k}^{2}
	\end{align*}
	for all $k$. Moreover, the expected squared norm of stochastic gradients
	is uniformly bounded, 
	\begin{align*}
	\mathbb{E}\|\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})\|^{2} & \leq G^{2}
	\end{align*}
\end{assumption}
\begin{theorem}
	Suppose $F_{k}$ is $L$-smooth and $\mu$-strongly convex for all
	$k$. Let $\kappa=\frac{L}{\mu}$, $\gamma=\max\{8\kappa-1,E\}$ where
	$E$ is the communication interval, and learning rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(\gamma+t)}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $0\leq c\leq1$
	is small enough such that
	$\alpha_{t} \leq\frac{1}{4L}$ and 
	$\alpha_{t} \leq\frac{1}{N}$ for all $t\geq0$. 
	
	Then with full device participation, if $\nu_{max}=\max_{k}\frac{1}{N}p_{k}$,
	we have 
	\begin{align*}
	\mathbb{E}F(\overline{w}_{T})-F^{\ast}\leq C\frac{\kappa}{\gamma+T}\cdot(8E^{2}LG^{2}/T+\frac{1}{N}\nu_{max}^{2}\sigma^{2})
	\end{align*}
	so that as long as $E=O(\sqrt{\frac{N}{T}})$, 
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq C(8LG^{2}+\nu_{max}^{2}\sigma^{2})\frac{\kappa}{N(\gamma+T)}
	\end{align*}
	and with partial participation with $K$ sampled devices at each
	communication round, $\frac{4}{K}\alpha_{t}^{2}E^{2}G^{2}$
	\begin{align*}
	\mathbb{E}F(\overline{w}_{T})-F^{\ast}\leq C\frac{\kappa}{\gamma+T}\cdot(8E^{2}LG^{2}/T+\frac{1}{N}\nu_{max}^{2}\sigma^{2}+\frac{4}{K}E^{2}G^{2})
	\end{align*}
	so that if $E=O(1)$, 
	\begin{align*}
	\mathbb{E}F(\overline{w}_{T})-F^{\ast} & \leq C(4E^{2}G^{2}+\nu_{max}^{2}\sigma^{2})\frac{\kappa}{K(\gamma+T)}+\frac{8E^{2}LG^{2}}{T^{2}}
	\end{align*}
\end{theorem}

\begin{proof}
	The idea of the proof is to observe that the $L$-smoothness of $F$
	provides the upper bound
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & =\mathbb{E}(F(\overline{w}_{t})-F(w^{\ast}))\\
	& \leq\frac{L}{2}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}
	\end{align*}
	and to show that $\mathbb{E}\|\overline{w}_{T}-w^{\ast}\|^{2}=O(\frac{1}{NT})$. 
	
	Our main step is to prove the bound 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq(1-\mu\alpha_{t})\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B
	\end{align*}
	where $B$ is define in the statement of the theorem. 
	
	We have 
	\begin{align*}
	\|\overline{w}_{t+1}-w^{\ast}\|^{2} & =\|(\overline{w}_{t}-\alpha_{t}g_{t})-w^{\ast}\|^{2}\\
	& =\|(\overline{w}_{t}-\alpha_{t}\overline{g}_{t}-w^{\ast})-\alpha_{t}(g_{t}-\overline{g}_{t})\|^{2}\\
	& =A_{1}+A_{2}+A_{3}
	\end{align*}
	where 
	\begin{align*}
	A_{1} & =\|\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t}\|^{2}\\
	A_{2} & =2\alpha_{t}\langle\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t},\overline{g}_{t}-g_{t}\rangle\\
	A_{3} & =\alpha_{t}^{2}\|g_{t}-\overline{g}_{t}\|^{2}
	\end{align*}
	$\mathbb{E}A_{2}=0$ by definition of $g_{t}$ and $\overline{g}_{t}$,
	while for $A_{3}$ we have
	\begin{align*}
	\alpha_{t}^{2}\mathbb{E}\|g_{t}-\overline{g}_{t}\|^{2} & =\alpha_{t}^{2}\mathbb{E}\|g_{t}-\mathbb{E}g_{t}\|^{2}=\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}^{2}\|g_{t,k}-\mathbb{E}g_{t,k}\|^{2}\leq\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}^{2}\sigma_{k}^{2}
	\end{align*}
	again by Jensen's inequality and using the independence of $g_{t,k},g_{t,k'}$. 
	
	Next we bound $A_{1}$: 
	\begin{align*}
	\|\overline{w}_{t}-w^{\ast}-\alpha_{t}\overline{g}_{t}\|^{2} & =\|\overline{w}_{t}-w^{\ast}\|^{2}+2\langle\overline{w}_{t}-w^{\ast},-\alpha_{t}\overline{g}_{t}\rangle+\|\alpha_{t}\overline{g}_{t}\|^{2}
	\end{align*}
	and we will show that the third term $\|\alpha_{t}\overline{g}_{t}\|^{2}$
	can be canceled by an upper bound of the second term. %
	\begin{comment}
	The last term is straightforward to bound by the convexity of $\|\cdot\|^{2}$
	and $L$-smoothness of $F_{k}$,
	\begin{align*}
	\alpha_{t}^{2}\|\overline{g}_{t}\|^{2} & \leq\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}\|\nabla F_{k}(w_{t}^{k})\|^{2}\leq2L\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}(F_{k}(w_{t}^{k})-F_{k}^{\ast})
	\end{align*}
	or 
	\begin{align*}
	\alpha_{t}^{2}\|\overline{g}_{t}\|^{2} & \leq\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}\|\nabla F_{k}(w_{t}^{k})\|^{2}\leq\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}\mathbb{E}\|\nabla F_{k}(w_{t}^{k},\xi_{t}^{k})\|^{2}\leq\alpha_{t}^{2}G^{2}
	\end{align*}
	\end{comment}
	
	Now 
	\begin{align*}
	-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle & =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle\\
	& =-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w_{t}^{k},\nabla F_{k}(w_{t}^{k})\rangle-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle w_{t}^{k}-w^{\ast},\nabla F_{k}(w_{t}^{k})\rangle\\
	& \leq-2\alpha_{t}\sum_{k=1}^{N}p_{k}\langle\overline{w}_{t}-w_{t}^{k},\nabla F_{k}(w_{t}^{k})\rangle+2\alpha_{t}\sum_{k=1}^{N}p_{k}(F_{k}(w^{\ast})-F_{k}(w_{t}^{k}))-\alpha_{t}\mu\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w^{\ast}\|^{2}\\
	& \leq2\alpha_{t}\sum_{k=1}^{N}p_{k}\left[F_{k}(w_{t}^{k})-F_{k}(\overline{w}_{t})+\frac{L}{2}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+F_{k}(w^{\ast})-F_{k}(w_{t}^{k})\right]-\alpha_{t}\mu\|\sum_{k=1}^{N}p_{k}w_{t}^{k}-w^{\ast}\|^{2}\\
	& =\alpha_{t}L\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+2\alpha_{t}\sum_{k=1}^{N}p_{k}\left[F_{k}(w^{\ast})-F_{k}(\overline{w}_{t})\right]-\alpha_{t}\mu\|\overline{w}_{t}-w^{\ast}\|^{2}
	\end{align*}
	For the second term, which is negative, we can ignore it, but this
	yields a suboptimal bound that fails to provide the desired linear
	speedup. This is the flaw in the analysis of the ICLR paper. Instead,
	we upper bound it using the following derivation: 
	\begin{align*}
	2\alpha_{t}\sum_{k=1}^{N}p_{k}\left[F_{k}(w^{\ast})-F_{k}(\overline{w}_{t})\right] & \leq2\alpha_{t}\left[F(\overline{w}_{t+1})-F(\overline{w}_{t})\right]\\
	& \leq2\alpha_{t}\mathbb{E}\langle\nabla F(\overline{w}_{t}),\overline{w}_{t+1}-\overline{w}_{t}\rangle+\alpha_{t}L\mathbb{E}\|\overline{w}_{t+1}-\overline{w}_{t}\|^{2}\\
	& =-2\alpha_{t}^{2}\mathbb{E}\langle\nabla F(\overline{w}_{t}),g_{t}\rangle+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& =-2\alpha_{t}^{2}\mathbb{E}\langle\nabla F(\overline{w}_{t}),\overline{g}_{t}\rangle+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& =-\alpha_{t}^{2}\left[\|\nabla F(\overline{w}_{t})\|^{2}+\|\overline{g}_{t}\|^{2}-\|\nabla F(\overline{w}_{t})-\overline{g}_{t}\|^{2}\right]+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& =-\alpha_{t}^{2}\left[\|\nabla F(\overline{w}_{t})\|^{2}+\|\overline{g}_{t}\|^{2}-\|\nabla F(\overline{w}_{t})-\sum_{k}p_{k}\nabla F(w_{t}^{k})\|^{2}\right]+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& \leq-\alpha_{t}^{2}\left[\|\nabla F(\overline{w}_{t})\|^{2}+\|\overline{g}_{t}\|^{2}-\sum_{k}p_{k}\|\nabla F(\overline{w}_{t})-\nabla F(w_{t}^{k})\|^{2}\right]+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& \leq-\alpha_{t}^{2}\left[\|\nabla F(\overline{w}_{t})\|^{2}+\|\overline{g}_{t}\|^{2}-L^{2}\sum_{k}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}\right]+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}\\
	& \leq-\alpha_{t}^{2}\|\overline{g}_{t}\|^{2}+\alpha_{t}^{2}L^{2}\sum_{k}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}
	\end{align*}
	where we have used the smoothness of $F$ twice. 
	
	Note that the term $-\alpha_{t}^{2}\|\overline{g}_{t}\|^{2}$ exactly
	cancels the $\alpha_{t}^{2}\|\overline{g}_{t}\|^{2}$ in the bound
	for $A_{1}$, so that plugging in the bound for $-2\alpha_{t}\langle\overline{w}_{t}-w^{\ast},\overline{g}_{t}\rangle$,
	we have so far proved 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}L\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}^{2}\sigma_{k}^{2}\\
	& +\alpha_{t}^{2}L^{2}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}+\alpha_{t}^{3}L\mathbb{E}\|g_{t}\|^{2}
	\end{align*}
	The term $\mathbb{E}\|g_{t}\|^{2}\leq G^{2}$ by assumption. 
	
	Now we bound $\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}$.
	Since communication is done every $E$ steps, for any $t\geq0$, we
	can find a $t_{0}\leq t$ such that $t-t_{0}\leq E-1$ and $w_{t_{0}}^{k}=\overline{w}_{t_{0}}$for
	all $k$. Moreover, using $\eta_{t}$ is non-increasing and $\alpha_{t_{0}}\leq\alpha{}_{t}$
	for any $t-t_{0}\leq E-1$, we have 
	\begin{align*}
	\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2} & =\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t_{0}}-(\overline{w}_{t}-\overline{w}_{t_{0}})\|^{2}\\
	& \leq\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-\overline{w}_{t_{0}}\|^{2}\\
	& =\mathbb{E}\sum_{k=1}^{N}p_{k}\|w_{t}^{k}-w_{t_{0}}^{k}\|^{2}\\
	& =\mathbb{E}\sum_{k=1}^{N}p_{k}\|-\sum_{i=t_{0}}^{t-1}\alpha_{i}g_{i,k}\|^{2}\\
	& \leq\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\alpha_{i}^{2}\|g_{i,k}\|^{2}\\
	& \leq\sum_{k=1}^{N}p_{k}\mathbb{E}\sum_{i=t_{0}}^{t-1}(E-1)\alpha_{t_{0}}^{2}G^{2}\\
	& \leq4E^{2}\alpha_{t}^{2}G^{2}
	\end{align*}
	
	Using the bound on $\mathbb{E}\sum_{k=1}^{N}p_{k}\|\overline{w}_{t}-w_{t}^{k}\|^{2}$,
	we can conclude that, with $\nu_{max}:=N\cdot\max_{k}p_{k}$ and $\nu_{min}:=N\cdot\min_{k}p_{k}$, 
	
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+4E^{2}L\alpha_{t}^{3}G^{2}+4E^{2}L^{2}\alpha_{t}^{4}G^{2}+\alpha_{t}^{2}\sum_{k=1}^{N}p_{k}^{2}\sigma_{k}^{2}+\alpha_{t}^{3}LG^{2}\\
	& =\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+4E^{2}L\alpha_{t}^{3}G^{2}+4E^{2}L^{2}\alpha_{t}^{4}G^{2}+\alpha_{t}^{2}\frac{1}{N^{2}}\sum_{k=1}^{N}(p_{k}N)^{2}\sigma_{k}^{2}+\alpha_{t}^{3}LG^{2}\\
	& \leq\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+4E^{2}L\alpha_{t}^{3}G^{2}+4E^{2}L^{2}\alpha_{t}^{4}G^{2}+\alpha_{t}^{2}\frac{1}{N^{2}}\nu_{max}^{2}\sum_{k=1}^{N}\sigma_{k}^{2}+\alpha_{t}^{3}LG^{2}\\
	& \leq\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}+4E^{2}L\alpha_{t}^{3}G^{2}+4E^{2}L^{2}\alpha_{t}^{4}G^{2}+\alpha_{t}^{2}\frac{1}{N}\nu_{max}^{2}\sigma^{2}+\alpha_{t}^{3}LG^{2}
	\end{align*}
	where $\sigma^{2}=\max_{k}\sigma_{k}^{2}$. We show next that $\|\overline{w}_{t}-w^{\ast}\|^{2}=O(\frac{\alpha_{t}}{N})=O(\frac{1}{Nt})$.
	Before we do, we remark briefly on the choice of $E$. The leading
	term among terms other than $\mathbb{E}(1-\mu\alpha_{t})\|\overline{w}_{t}-w^{\ast}\|^{2}$
	is $\alpha_{t}^{2}\frac{1}{N}\nu_{max}^{2}\sigma^{2}$. This means
	we can take $E=O(\sqrt{\frac{1}{N\alpha_{t}}})=O(\sqrt{\frac{t}{N}})$
	which means $4E^{2}L\alpha_{t}^{3}G^{2}=O(\frac{\alpha_{t}}{N})$
	will be on the same order as the leading term. This is in contrast
	with previous results where $E$ cannot scale with $t$. Thus our
	bound yields a more efficient communication complexity than current
	analyses. We note however that this is only possible when there is
	full participation, and when $\nu_{max}$ is close to 1. When there
	is partial participation, however, $E$ has to stay $O(1)$, as we
	will soon see. Thus our result hightlights the difference between
	the communication efficiency of full and partial participation when
	an $O(1/T)$ bound on the optimality gap is desired. 
	
	\textbf{}%
	\begin{comment}
	The leading term on the right hand side the bound is $\alpha_{t}^{2}\frac{1}{N}\nu_{max}^{2}\sigma^{2}$,
	which when summed using the recursive relations gives $O(\alpha_{t})=O(1/t)$,
	but the constant now is scaled down by $1/N$. \textbf{To achieve
	this linear speedup, we need $\sum_{t=0}^{T}(1-\mu\alpha_{t})\|w_{0}-w^{\ast}\|^{2}$
	to be small enough. Note also that the above bound implies that $E$
	can be chosen to be as large as $O(\sqrt{\frac{T}{N}})$ without degrading
	the performance, since $E^{2}\alpha_{t}^{3}=O(\alpha_{t}^{2}/N)$
	which is the order of the leading term. As we will see, in the partial
	participation case, this is no longer true, and $E$ cannot be chosen
	$O(T^{\beta})$ for any $\beta>0$. }
	\end{comment}
	
	To complete the proof of convergence, let $B=$ $B_{t}=4E^{2}L\alpha_{t}G^{2}+4E^{2}L^{2}\alpha_{t}^{2}G^{2}+\frac{1}{N}\nu_{max}^{2}\sigma^{2}+\alpha_{t}LG^{2}$.
	Set the learning rate $\alpha_{t}=\frac{\delta}{t+\gamma}$ for $\delta>\frac{1}{\mu}$
	and $\gamma=\max\{8\kappa-1,E\}$ such that $\alpha_{1}\leq\min\{\frac{1}{\mu},\frac{1}{4L}\}$and
	$\alpha_{t}\leq2\alpha_{t+E}$, we can show that 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2} & \leq\frac{v}{N(\gamma+t)}
	\end{align*}
	where $v=\max\{\frac{\delta^{2}B}{\delta\mu-1},(\gamma+1)\|w_{0}-w^{\ast}\|^{2}\}$,
	by induction. The definition of $v$ ensures that 
	\begin{align*}
	\|w_{0}-w^{\ast}\|^{2} & \leq\frac{v}{\gamma}
	\end{align*}
	and suppose $\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq\frac{v}{N(\gamma+t)}$
	holds for some $t\geq0$. Then 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t+1}-w^{\ast}\|^{2}\leq & (1-\alpha_{t}\mu)\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}+\alpha_{t}^{2}B'\\
	& \leq(1-\frac{\delta\mu}{t+\gamma})\frac{v}{N(t+\gamma)}+\frac{\delta^{2}B'}{N^{2}(t+\gamma)^{2}}\\
	& =\frac{t+\gamma-1}{N(t+\gamma)^{2}}v+\left[\frac{\delta^{2}B'}{N^{2}(t+\gamma)^{2}}-\frac{\delta\mu-1}{N(t+\gamma)^{2}}v\right]\\
	& \leq\frac{t+\gamma-1}{N(t+\gamma)^{2}}v+\left[\frac{\delta^{2}B'}{N(t+\gamma)^{2}}-\frac{\delta\mu-1}{N(t+\gamma)^{2}}v\right]\\
	& \leq\frac{1}{N}\frac{v}{t+\gamma+1}
	\end{align*}
	by definition of $v$.
	
	Finally, the $L$-smoothness of $F$ implies 
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & =\mathbb{E}(F(\overline{w}_{t})-F(w^{\ast}))\\
	& \leq\frac{L}{2}\mathbb{E}\|\overline{w}_{t}-w^{\ast}\|^{2}\leq\frac{L}{2}\frac{v}{\gamma+t}
	\end{align*}
	Now if we choose $\delta=\frac{c}{\mu}$ where $c\leq1$ is small
	enough such that the required conditions 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	\alpha_{t} & \leq\frac{1}{4L}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	hold for all $t\geq0$, $\gamma=\max\{8\kappa-1,E\}$, then $\alpha_{t}=\frac{c}{\mu}\frac{1}{\gamma+t}$
	and recalling $v=\max\{\frac{\delta^{2}B'}{\delta\mu-c+1},(\gamma+1)\|w_{0}-w^{\ast}\|^{2}\}$,
	we finally have 
	\begin{align*}
	\mathbb{E}(F(\overline{w}_{t}))-F^{\ast} & \leq\frac{L}{2}\frac{v}{\gamma+t}\leq\frac{L/2}{\gamma+t}(\frac{\delta^{2}B'}{\delta\mu-c+1}+(\gamma+1)\|w_{0}-w^{\ast}\|^{2})\\
	& \leq\frac{\kappa}{\gamma+t}(\frac{B'}{\mu}+4L\|w_{0}-w^{\ast}\|^{2})
	\end{align*}
	where $B'=8E^{2}L^{2}G^{2}/t+\frac{1}{N}\nu_{max}^{2}\sigma^{2}$. 
	
	With partial participation, the update at each communication round
	is now given by averages over a subset of sampled devices. The key
	is to bound 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t}-\overline{y}_{t}\|^{2} & =\frac{1}{K}\sum_{k}p^{k}\|w_{t}^{k}-\sum_{k}p_{k}w_{t}^{k}\|^{2}
	\end{align*}
	This can be bounded by the same argument as before and yield 
	\begin{align*}
	\mathbb{E}\|\overline{w}_{t}-\overline{y}_{t}\|^{2} & \leq\frac{4}{K}\alpha_{t}^{2}E^{2}G^{2}
	\end{align*}
	and so this is also a leading term, and together with the term $\alpha_{t}^{2}\frac{1}{N}\nu_{max}^{2}\sigma^{2}$
	determines the convergence rate, which is now $O(\frac{(\nu_{max}^{2}\sigma^{2}+4E^{2}G^{2})}{KT})$.
	This implies that $E$ canot be chosen $O(T^{\beta})$ for any $\beta>0$
	without degrading the performance. This should be checked in experiments,
	whether with partial participation if the communication round is set
	to scale with $T$, the convergence deteriorates. This is in constrast
	with the full participation case, where $E=O(\sqrt{\frac{T}{N}})$
	is allowed. \textbf{If we can confirm that full participation allows
		linear speedup with $\nu=N\cdot\max_{k}p_{k}\approx1$ and $E=O(\sqrt{\frac{T}{N}})$,
		whereas partial participation only allows $E=O(1)$, then this would
		an interesting phenomenon that is not reported by previous studies!}
\end{proof}

==> sec_sgdscvxnonsmth.tex <==
% !TEX ROOT=./main.tex

In this section, we prove the convergence rate of stochastic for strongly convex
non-smooth problem.


\begin{theorem}
	Let Assumption~\ref{ass:subgrad2} and Assumption~\ref{ass:stroncvx} hold, choose learning rate $\eta_t = \frac{2}{\mu(t+1)} $.Then,
	\begin{align}
		\EE[F(\hat{\vw}_T)] - F^* \leq \frac{2(B + C)}{\mu(T+1)}.
	\end{align}
	where $B =  G^2 (3  + 8 (E-1)^2)$, $C$ is defined in \eq{\ref{eq:partialsample}}.
\end{theorem}


\begin{proof}

\textbf{Full Device activation: }  $\ov{w}_{t+1} = \ov{v}_{t+1}, \forall t$ 
\begin{align}
\Delta_{t+1} = \EE\left[\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\bar{\vw}_{t}-\vw^{*}\|^{2} \underbrace{ - 2 \eta_{t} \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)}_{B_1} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2}	
\label{eq:expand2}
\end{align}


Now we focus on bounding $B_1$ in \eq{\ref{eq:expand}}: 
\begin{align}
	& -2 \eta_{t} \left<\EE \vg_{t}, \bar{\vw}_{t}-\vw^{*} \right>\\
  = & 2 \eta_{t} \sum_{k=1}^N p_k \left(-\left<\EE \vg_{t,k}, \bar{\vw}_{t}-\vw_t^k + \vw_t^k - \vw^{*} \right> \right) \\
  \leq& 2 \eta_{t} \sum_{k=1}^N p_k  \left(\frac{1}{2\eta_t} \|\overline{\vw}_t - \vw_t^k\|^2 + \frac{\eta_t}{2} \|\EE \vg_{t,k}\|^2 - F_k(\vw_t^k) - F_k(\vw^*) - \frac{\mu}{2} \|\vw_t^k - \vw^*\|^2 \right) \\
  =& \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 
  - 2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*) - \eta_t \mu \sum_{k=1}^N p_k \|\vw_t^k - \vw^*\|^2 \\
  \leq & \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 
  - 2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*) - \eta_t \mu \|\ov{w}_t- \vw^*\|^2  \label{eq:scvxnsmth1}
\end{align}
where in the third line we use Cauchy-Schwarz inequality, AM-GM inequality and strong convexity.
In the last line we use convexity of l2 norm and Jensen's inequality.

Now we plug in $B_1$ into \eq{\ref{eq:expand2}}, we have,
\begin{align}
	\EE\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2 & \leq (1 - \eta_t\mu)\|\bar{\vw}_{t}-\vw^{*}\|^{2} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 \\
	& \underbrace{-2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*)}_{C_1} + \sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2 \label{eq:scvxnsmth2}
\end{align}

Now we bound $C_1$
\begin{align}
	-2\eta_t\sum_{k=1}^N p_k (F_k(\vw_t^k) - F^*) & = -2\eta_t\sum_{k=1}^N p_k \left(F_k(\vw_t^k) - F_k(\ov{w}_t)\right) + F(\ov{w}_t) -  F^*\\
& \leq \sum_{k=1}^{k} p_{k}[\eta_{t}^{2}\|\EE \vg_{t,k}(\ov{w}_{t})\|^{2}+\| \vw_{t}^{k}-\ov{w}_t^{k} \|^{2}]-2 \eta_{t}(F(\ov{w}_{t})- F^{*}). 
\end{align}

Plug in $C_1$ into \eq{\ref{eq:scvxnsmth2}}:
\begin{align}
	\EE\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2 \leq
	&  (1 - \eta_t\mu)\|\bar{\vw}_{t}-\vw^{*}\|^{2} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2 \\& + \sum_{k=1}^{k} p_{k}\eta_{t}^{2}\|\EE \vg_{t,k}(\ov{w}_{t})\|^{2}-2 \eta_{t}(F(\ov{w}_{t})- F^{*})  + 2 \underbrace{\sum_{k=1}^N p_k \|\overline{\vw}_t - \vw_t^k\|^2}_{C_2} \label{eq:scvxnsmth3}
\end{align}
$C_2 \leq  4\eta_t^2 (E-1)^2 G^2$ can be bounded by Lemma 3 in \cite{li2019convergence}, we plug in $C_2$ into \eq{\ref{eq:scvxnsmth3}},


\begin{align}
	\underbrace{\EE\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2}_{\Delta_{t+1}} \leq &  (1 - \eta_t\mu)\|\bar{\vw}_{t}-\vw^{*}\|^{2} -2 \eta_{t}(F(\ov{w}_{t})- F^{*})\\
	+ & \underbrace{\eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2  + \sum_{k=1}^{k} p_{k}\eta_{t}^{2}\|\EE \vg_{t,k}(\ov{w}_{t})\|^{2} + 8\eta_t^2 (E-1)^2 G^2}_{\eta_t^2 B} \label{eq:scvxnsmth4} \\
	\Delta_{t+1}  \leq &  (1 - \eta_t\mu) \Delta_t + \eta^2_t B - 2 \eta_t [F(\ov{w}_{t})- F^{*}] \label{eq:scvxnsmth5}
\end{align}
where 
\begin{align*}
\eta_t^2 B &= \eta_{t}^{2} \EE\| \vg_{t} \|^{2} +  \sum_{k=1}^N p_k \eta_t^2 \|\EE \vg_{t,k}\|^2  + \sum_{k=1}^{k} p_{k}\eta_{t}^{2}\|\EE \vg_{t,k}(\ov{w}_{t})\|^{2} + 8\eta_t^2 (E-1)^2 G^2 \\
& \leq \eta_t^2 G^2 (3  + 8 (E-1)^2) 	
\end{align*}

Rearrange, set $\eta_t = \frac{2}{\mu(t+1)} $, using the weighted average trick in \cite{lacoste2012simpler}, and sum two sides of \eq{\ref{eq:scvxnsmth5}}, we have
\begin{align}
F\left(\ov{w}_{t}\right)-F^{*} &\leqslant \left(\frac{1}{2 \eta_{t}}-\frac{\mu}{2}\right) \Delta t-\frac{\Delta_{t+1}}{2 \eta_{t}}+\frac{\eta_{t}}{2} B\\
t(F\left(\ov{w}_{t}\right)-F^{*}) & \leqslant t\left(\frac{1}{2 \eta_{t}}-\frac{\mu}{2}\right) \Delta t-\frac{t\Delta_{t+1}}{2 \eta_{t}}+\frac{\eta_{t}}{2} Bt\\
t(F\left(\ov{w}_{t}\right)-F^{*}) & \leqslant \frac{\mu t(t-1)}{4} \Delta t- \frac{\mu t(t+1)\Delta_{t+1}}{4}+\frac{t}{\mu(t+1)} B\\
t(F\left(\ov{w}_{t}\right)-F^{*}) & \leqslant \frac{\mu t(t-1)}{4} \Delta t- \frac{\mu t(t+1)\Delta_{t+1}}{4}+\frac{B}{\mu}\\
\sum_{t=1}^T \frac{2t}{T(T+1)}F\left(\ov{w}_{t}\right)-F^{*} & \leqslant \frac{2B}{\mu(T+1)} \\
F\left(\sum_{t=1}^T \frac{2t}{T(T+1)} \ov{w}_{t}\right)-F^{*} & \leqslant \frac{2B}{\mu(T+1)} 
\end{align}

\textbf{Partial Device activation: }

If $t + 1 \notin \cI_{E}$, $\ov{w}_{t+1} = \ov{v}_{t+1}$, 
\begin{align}
\EE\left[\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2| \ov{w}_{t}\right] = \EE\left[\left\|\bar{\vv}_{t+1}-\vw^{*}\right\|^2| \vw_{t}\right]=\|\bar{\vw}_{t}-\vw^{*}\|^{2} \underbrace{ - 2 \eta_{t} \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)}_{B_1} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2}	
\label{eq:expandp1}
\end{align}

If $t + 1 \in \cI_{E}$, $\ov{w}_{t+1} = \frac{1}{K}\sum_{l=1}^K \vv_{t+1}^{i_l}$, 
\begin{align}
\EE\left\|\ov{w}_{t+1}-\vw^{*}\right\|^2 & =  \EE\left\|\ov{w}_{t+1} - \ov{v}_{t+1} + \ov{v}_{t+1} -\vw^{*}\right\|^2 \\
& \leq \EE\left\|\ov{w}_{t+1} - \ov{v}_{t+1}\right\|^2 + \EE \left\| \ov{v}_{t+1} -\vw^{*}\right\|^2 \\
&= \|\bar{\vw}_{t}-\vw^{*}\|^{2} \underbrace{ - 2 \eta_{t} \EE \vg_{t}^{\top}\left(\bar{\vw}_{t}-\vw^{*}\right)}_{B_1} + \eta_{t}^{2} \EE\| \vg_{t} \|^{2}	+ \EE\left\|\ov{w}_{t+1} - \ov{v}_{t+1}\right\|^2
\label{eq:expandp2}
\end{align}


Similar to the full device derivation:
\begin{align}
F\left(\sum_{t=1}^T \frac{2t}{T(T+1)} \ov{w}_{t}\right)-F^{*} & \leqslant \frac{2(B + C)}{\mu(T+1)} 	
\end{align}
where $B =  G^2 (3  + 8 (E-1)^2)$ and $C =\frac{4(N - K)}{K(N-1)} \eta_t^2 E^2G^2 $ or
$C = \frac{4}{K} \eta_t^2 E^2G^2$ depends on the sampling scheme.



\end{proof}

==> sec_theorems.tex <==
% !TEX ROOT=./main.tex



\section{Convergence Results}
This section summarizes the current results and assumptions.
\begin{table}[h!]
\centering
\small
	\begin{tabular}{|c|c|c|c|c|}\hline
		paper         &  Cvx Non-smth & Cvx L-smth & Strongly Cvx Non-smth& Strongly Cvx L-smth \\ \hline
	Accelerated	SGD   &   $\cO(\frac{1}{\sqrt{T}})$     & $\cO(\frac{1}{\sqrt{T}})$   &    $\cO(\frac{1}{T})$   &  $\cO(\frac{1}{KT})$    \\\hline
	SGD    &    $\cO(\frac{1}{\sqrt{T}})$  &   $\cO(\frac{1}{\sqrt{T}})$  &  $\cO(\frac{1}{T})$  & $\cO(\frac{1}{T})$\cite{li2019convergence,haddadpour2019convergence}, $\cO(\frac{1}{KT})$ ours    \\\hline
	\end{tabular}
	\caption{Summarize of related work on federated learning, heterogeneous data.}
\end{table}

Linear speedup of SGD and MaSS for linear regression, full participation: 
\begin{align*}
\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq C\cdot\exp(-\frac{t}{\sqrt{(\kappa_{N}+(E-1)^{2})(\tilde{\kappa}_{N}+(E-1)^{2})}})
\end{align*}

 which implies that for $E=1$, there is linear speedup, i.e. 
\begin{align*}
\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq C\cdot\exp(-\frac{t}{\sqrt{(\kappa_{N})(\tilde{\kappa}_{N})}})\leq C\cdot\exp(-\frac{Nt}{\sqrt{(\kappa_{1})(\tilde{\kappa})}})
\end{align*}
when $N$ satifies $N=O(\min(L_{1}/L,\tilde{\kappa}))$, and for $(E-1)^{2}\leq\min(\kappa_{N},\tilde{\kappa}_{N})$,
\begin{align*}
\|\overline{w}_{t+1}-w^{\ast}\|^{2} & \leq C\cdot\exp(-\frac{Nt}{4\sqrt{\kappa_{1}\tilde{\kappa}}})
\end{align*}

Acceleration of MaSS for linear regression, partial participation $O((1+\frac{4}{K}\cdot(\frac{t}{E}-1))\exp(-\frac{t}{\sqrt{\kappa_{m}\tilde{\kappa}_{m}}}))$
over $O((1+\frac{4}{K}\cdot(\frac{t}{E}-1))\exp(-\frac{t}{\kappa_{m}}))$. 

Linear speedup of SGD and Nesterov SGD for strongly convex and smooth
objectives: full participation $O(\frac{\nu_{max}^{2}\sigma^{2}}{NT}+\frac{E^{2}LG^{2}}{T^{2}})$
with $\nu_{max}=N\cdot\max_{k}p_{k}$; partial participation $O(\frac{\nu_{max}^{2}\sigma^{2}+4E^{2}G^{2}L}{KT})$.
In particular, this implies full participation allows $E=O(\sqrt{\frac{T}{N}})$
to achieve $O(1/NT)$, whereas partial participation only allows $E=O(1)$
to achieve $O(1/KT)$. 

Other accelerations likely not possible. 



\begin{assumption}[Bounded local variance]
Let $\xi_{t}^{k}$ be sampled from the $k$ -th device's local data uniformly at random. The variance of stochastic gradients in each device is bounded: $\mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)-\nabla F_{k}\left(\mathbf{w}_{t}^{k}\right)\right\|^{2} \leq \sigma_{k}^{2}$,
for $k=1, \cdots, N$.	
\end{assumption}



% \begin{assumption}
% The expected squared norm of stochastic subgradients is uniformly bounded. i.e.,
% $\mathbb{E}\|\vg_{t,k}\|^2  \leq G_k^{2}$, for all $k = 1,..., N$ and $t=0, \dots, T-1$.  This also implies $\left\| \mathbb{E}\vg_{t,k}\right\|^2  \leq \mathbb{E}\|\vg_{t,k}\|^2 \leq G_k^2$. Denote $G^2 = \sum_{k=1}^N p_k G_k^2$
% \label{ass:subgrad2}
% \end{assumption}


\begin{assumption}[Expected square norm of gradient]
The expected squared norm of stochastic gradients is uniformly bounded. i.e.,
$\mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right)\right\|^{2} \leq G^{2}$, for all $k = 1,..., N$ and $t=0, \dots, T-1$. This also implies $\left\| \mathbb{E}\vg_{t,k}\right\|^2  \leq \mathbb{E}\|\vg_{t,k}\|^2 \leq G_k^2$.
\label{ass:subgrad2}
\end{assumption}

\begin{assumption}[L-smooth]
$F_{1}, \cdots, F_{N}$ are all $L$-smooth: for all  $\mathbf{v}$  and $\mathbf{w}$, $F_{k}(\mathbf{v}) \leq F_{k}(\mathbf{w})+(\mathbf{v}- \\ \mathbf{w})^{T} \nabla F_{k}(\mathbf{w})+\frac{L}{2}\|\mathbf{v}-\mathbf{w}\|_{2}^{2}$.
\label{ass:lsmooth}
\end{assumption}
\begin{assumption}[Strongly-convex]
$	F_{1}, \cdots, F_{N} \text { are all } \mu \text { -strongly convex: for all v and } \mathbf{w}, F_{k}(\mathbf{v}) \geq F_{k}(\mathbf{w})+(\mathbf{v}-\mathbf{w})^{T} \nabla F_{k}(\mathbf{w})+\frac{\mu}{2}\|\mathbf{v}-\mathbf{w}\|_{2}^{2}$
\label{ass:stroncvx}
\end{assumption}

\begin{definition}[Squared Weighted Gradient Diversity]
	We indicate the following quantity as weighted gradient diversity among the local 
	objectives:
	\begin{align*}
		\frac{\sum_{k=1}^K p_k  \mathbb{E}\left\|\nabla F_{k}\left(\mathbf{w}, \xi^{k}\right)\right\|^{2} }{\mathbb{E}\left\| \sum_{k=1}^K p_k   \nabla F_{k}\left(\mathbf{w}, \xi^{k}\right)\right\|^{2} } \leq \lambda 
	\end{align*}
\end{definition}
This definition is similar to the weighted gradient diversity defined in~\cite{haddadpour2019convergence}.

\begin{definition}[Gradient Dissimilarity~\cite{li2018federated}]
	We indicate the following quantity as gradient diversity among the local 
	objectives:
	\begin{align*}
		\frac{\sum_{k=1}^K p_k \left\|\nabla F_{k}\left(\mathbf{w}\right)\right\|^{2} }{\left\|   \nabla F\left(\mathbf{w}\right)\right\|^{2} } \leq \lambda 
	\end{align*}
	For some $\epsilon>0$, for all the points $\vw \in \mathcal{S}_{\epsilon}^{c}=\left\{\vw |\|\nabla F(\vw)\|^{2}>\epsilon\right\}$
\end{definition}

\section{The Convergence of FedAvg for General Convex Functions}
This section summarizes the convergence of FedAvg.
The updates of FedAvg with partial device activation is given by: 
\begin{align} 
\mathbf{v}_{t+1}^{k} &=\mathbf{w}_{t}^{k}-\eta_{t} \nabla F_{k}\left(\mathbf{w}_{t}^{k}, \xi_{t}^{k}\right) \\ \mathbf{w}_{t+1}^{k} &=\left\{\begin{array}{ll}\mathbf{v}_{t+1}^{k} & \text { if } t+1 \notin \mathcal{I}_{E}, \\ 
\sum_{k \in \cS_{t+1}} \mathbf{v}_{t+1}^{k} & \text { if } t+1 \in \mathcal{I}_{E}\end{array}\right.
\end{align}

\subsection{The Convergence of FedAvg for Convex Functions}
In this subsection, we discuss the convergence of FedAvg for convex functions,
we consider both smooth (Theorem~\ref{th:sgdcvxsmth}) and non-smooth (Theorem~\ref{th:sgdcvxnonsmoth})
functions. 

\begin{theorem}
Let Assumption~\ref{ass:subgrad2} and Assumption~\ref{ass:lsmooth} hold, suppose we have a bound 
on our starting distance, i.e., $\|\vw_{0} - \vw^*\|^2 \leq \Delta_0$, set learning rate $\eta_t =  \left(\frac{\Delta_0}{ T A}\right)^{1/2}$, we have,
$$\EE[ F_T^*] - F^*  \leq \left(\frac{ \Delta_0 A }{T}\right)^{1/2},$$
where we denote $F^*_T = \min_{t \in [0, T-1]} F(\ov{w}_t)$, $A = G^2( 4L(E-1)^2 + 1)) + C$.
\label{th:sgdcvxsmth}
\end{theorem}

\begin{theorem}
If we remove the smoothness assumption in Theorem~\ref{th:sgdcvxsmth}, i.e., 
	Let Assumption~\ref{ass:subgrad2} hold, replacing the constant $A$ with $A=G^2 \left(4(E-1)^2 + 3\right) + C$, then the same convergence rate in Theorem~\ref{th:sgdcvxsmth}.
	\label{th:sgdcvxnonsmoth}
\end{theorem}
The proof is deferred to Section~\ref{sec:convexsmoothsgd} in the Appendix. 

\subsection{The Convergence of FedAvg for Strongly Convex Functions}

\subsection{Smooth}
We improve on the result of \cite{li2019convergence} and show the linear speedup of FedAvg with the number of devices. 

\begin{theorem}
	(Full device participation) Suppose $F_{k}$ is $L$-smooth and $\mu$-strongly
	convex for all $k$. Let $\kappa=\frac{L}{\mu}$, $\gamma=\max\{8\kappa-1,E\}$
	where $E$ is the communication interval, and learning rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(\gamma+t)}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $0\leq c\leq1$
	is small enough such that the following hold: 
	\begin{align*}
	\alpha_{t} & \leq\frac{1}{4L}\\
	\alpha_{t} & \leq\frac{1}{N}
	\end{align*}
	for all $t\geq0$. 
	
	Then with full device participation,
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq C\frac{\kappa}{N(\gamma+t)}\\
	C & =4E^{2}LG^{2}+\nu_{max}^{2}\sigma^{2}+LG^{2}
	\end{align*}
	
\end{theorem}

\subsection{Non-smooth}
\begin{theorem}
	Let assumption~\ref{ass:stroncvx} and assumption~\ref{ass:subgrad2} hold, choose learning rate $\eta_t = \frac{2}{\mu(t+1)} $.Then,
	\begin{align}
		\EE[F(\hat{\vw}_T)] - F^* \leq \frac{2(B + C)}{\mu(T+1)}.
	\end{align}
	where $B =  G^2 (3  + 8 (E-1)^2)$, for sampling scheme I $C =\frac{4(N - K)}{K(N-1)} \eta_t^2 E^2G^2 $ or
sampling scheme II $C = \frac{4}{K} \eta_t^2 E^2G^2$, for full device participation $C= 0$.
\end{theorem}


\section{Accelerated methods}
\subsection{stochastic gradient descent}
\subsubsection{Convex}
\begin{theorem}
	Let Assumption~\ref{ass:lsmooth} and Assumption~\ref{ass:subgrad2} hold,  choose the learning rate $\eta = \frac{\alpha}{1 - \beta} = \sqrt{\frac{\Delta_0}{(D+C)T}}$, $\beta \in (0, 1)$ and $\beta \leq \min\{1, \frac{1}{1 + \sqrt{\frac{\Delta_0}{(D+C)T}}}\}$, then the FedNestrovAve with partial device participation satisfies
	\begin{align}
		 \EE F(\hat{\vw}_T) - F^* &\leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} 
	\end{align}
	where $\hat{\vw}_T = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $C$ is defined in \eq{\ref{eq:partialsample}},
$D$ is given by $D =  G^2[6 + (4(E-1)^2+1)L]$.
\end{theorem}

\subsubsection{Strongly Convex}
\begin{theorem}
	(Partial device participation) Suppose $F_{k}$ is $L$-smooth and
	$\mu$-strongly convex for all $k$. Let $\kappa=\frac{L}{\mu}$,
	$\gamma=\max\{8\kappa-1,E\}$ where $E$ is the communication interval,
	and learning rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(\gamma+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $0\leq c\leq1$
	is small enough such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	\alpha_{t} & \leq\frac{1}{4L}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|g_{t,k}\|^{2}\leq G^{2}$ for all $t,k$. 
	
	Then with the partial device participation scheme described above,
	\begin{align*}
	\mathbb{E}F(w_{T})-F^{\ast} & \leq\frac{\kappa}{\gamma+T}(\frac{B'+C}{\mu}+4L(\|w_{0}-w^{\ast}\|^{2})\\
	B' & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}+2K^{2}\\
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =8L\Gamma+32(E-1)^{2}G^{2}+3G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}

\subsection{Stochastic Subgradient methods}

\subsubsection{Convex}
\begin{theorem}
	Let Assumption~\ref{ass:subgrad2} hold, choose the learning rate $\eta = \frac{\alpha}{1 - \beta} = \sqrt{\frac{\Delta_0}{(D+C)T}}$, $\beta \in (0, 1)$ and $\beta \leq \min\{1, \frac{1}{1 + \sqrt{\frac{\Delta_0}{(D+C)T}}}\}$, then the FedNestrovAve with partial device participation satisfies
	\begin{align}
		 \EE F(\hat{\vw}_T) - F^* &\leq \sqrt{\frac{\Delta_0(D + C)}{T}} + \frac{\Delta_0^{3/2}}{2\sqrt{D+C}}\frac{1}{T^{3/2}} 
	\end{align}
	where $\hat{\vw}_T = \frac{1}{T}\sum_{t=0}^{T-1} \ov{w}_t$, $C$ is defined in \eq{\ref{eq:partialsample}},
$D$ is given by $D = (8 + 8(E-1)^2)G^2$.
	\label{th:nasgcvxnonsmoth}
\end{theorem}

\subsubsection{Strongly Convex}
% \input{sec_nasgd_scvx_nonsmooth}
\begin{theorem}
	(Partial device participation) Suppose $F_{k}$ is $\mu$-strongly
	convex for all $k$. Let $E$ be the communication interval, and learning
	rates 
	\begin{align*}
	\alpha_{t} & =\frac{c}{\mu(E+t)}\\
	\beta_{t} & \leq\alpha_{t}
	\end{align*}
	so that $\alpha_{t}\leq2\alpha_{t+E}$, and where $c$ is small enough
	such that the following hold: 
	\begin{align*}
	\alpha_{t}^{2}+\beta_{t-1}^{2} & \leq\frac{1}{2}\\
	4\alpha_{t-1}^{2} & \leq\alpha_{t}
	\end{align*}
	for all $t\geq0$. Suppose also that $G$ is a constant satisfying
	$\mathbb{E}\|w_{0}-\alpha_{0}g_{0,k}\|^{2}=\mathbb{E}\|w_{0}-\alpha_{0}\nabla F_{k}(w_{0},\xi_{0}^{k})\|^{2}\leq G^{2}$
	for all $k$, and $\mathbb{E}\|\nabla F_{k}(w,\xi_{t}^{k})\|^{2}\leq G^{2}$
	for $w=\overline{w}_{t}$ or $w=w_{t}^{k}$ and all $t,k$.
	
	Then with partial device participation, \textbf{
		\begin{align*}
		F(\sum_{t=1}^{T}\frac{2t}{T(T+1)}\overline{w}_{t})-F^{\ast} & \leq\frac{2(B'+C)}{\mu(T+1)}
		\end{align*}
	} where
	\begin{align*}
	B' & =6G^{2}+32(E-1)^{2}G^{2}+2K^{2}\\
	C & =\frac{16}{S}E^{2}G^{2}
	\end{align*}
	and $K$ is such that 
	\begin{align*}
	\alpha_{0}B+2K\cdot G & \leq\mu K^{2}\\
	B & =6G^{2}+32(E-1)^{2}G^{2}
	\end{align*}
	and
	\begin{align*}
	K & \geq\max\{\|w_{0}-w^{\ast}\|^{2},\frac{G}{2\alpha_{0}}\}
	\end{align*}
\end{theorem}

